Quasi-Deterministic Burstiness Bound for Aggregate of Independent, Periodic Flows

Time-sensitive networks require timely and accurate monitoring of the status of the network. To achieve this, many devices send packets periodically, which are then aggregated and forwarded to the controller. Bounding the aggregate burstiness of the traffic is then crucial for effective resource management. In this paper, we are interested in bounding this aggregate burstiness for independent and periodic flows. A deterministic bound is tight only when flows are perfectly synchronized, which is highly unlikely in practice and would be overly pessimistic. We compute the probability that the aggregate burstiness exceeds some value. When all flows have the same period and packet size, we obtain a closed-form bound using the Dvoretzky-Kiefer-Wolfowitz inequality. In the heterogeneous case, we group flows and combine the bounds obtained for each group using the convolution bound. Our bounds are numerically close to simulations and thus fairly tight. The resulting aggregate burstiness estimated for a non-zero violation probability is considerably smaller than the deterministic one: it grows in $\sqrt{n\log{n}}$, instead of $n$, where $n$ is the number of flows.

==> Figures/arrivals.tex <==
\begin{tikzpicture}
		
		
		\pgfplotsset{soldot/.style={color=black,only marks,mark=*}} 				   		   		 \pgfplotsset{holdot/.style={color=black,fill=white,only marks,mark=*}}
		\pgfplotsset{ticks=none}
		% \begin{axis}[
		% xmin=-1,xmax= 10,ymin=-1,ymax=5, axis lines=center, width=1.4\textwidth,
		% height=1.2\textwidth]
  		\begin{axis}[
		xmin=-0.8,xmax= 10,ymin=-0.8,ymax=5, axis lines=center, width=0.9\textwidth,
		height=0.5\textwidth]
		
		\addplot[soldot, ultra thick] coordinates{(1,0)(3,1)(5,2)(7,3)(9,4)};
		\addplot[holdot, ultra thick] coordinates{(1,1)(3,2) (5,3) (7,4)} ;
  
            \draw[ultra thick] (axis cs:0,0) -- (axis cs:1,0);
		\draw[dotted] (axis cs:1,0) -- (axis cs:1,1);
		\draw[ultra thick] (axis cs:1,1) -- (axis cs:3,1);
		\draw[dotted] (axis cs:3,1) -- (axis cs:3,0);
            \draw[dotted] (axis cs:1,1) -- (axis cs:0,1);

		
		\draw[dotted] (axis cs:3,1) -- (axis cs:3,2);
		\draw[ultra thick] (axis cs:3,2) -- (axis cs:5,2);
		\draw[dotted] (axis cs:5,2) -- (axis cs:5,0);
		\draw[dotted] (axis cs:3,2) -- (axis cs:0,2);
		
		\draw[dotted] (axis cs:5,2) -- (axis cs:5,3);
		\draw[ultra thick] (axis cs:5,3) -- (axis cs:7,3);
		\draw[dotted] (axis cs:7,3) -- (axis cs:7,4);
		\draw[dotted] (axis cs:9,4) -- (axis cs:9,5);
		\draw[dotted] (axis cs:5,3) -- (axis cs:0,3);
		
		\draw[dotted] (axis cs:7,3) -- (axis cs:7,4);
		\draw[ultra thick] (axis cs:7,4) -- (axis cs:9,4);
		\draw[dotted] (axis cs:9,4) -- (axis cs:9,0);
		\draw[dotted] (axis cs:7,4) -- (axis cs:0,4);
		\draw[dotted] (axis cs:7,3) -- (axis cs:7,0);
		
		\draw[ultra thick,dashed] (axis cs:0,1) -- (axis cs:8,5);

  
		% \draw[dotted] (axis cs:0,0) -- (axis cs:0,1);
		% \draw[ultra thick] (axis cs:0,1) -- (axis cs:2,1);
		% \draw[dotted] (axis cs:2,1) -- (axis cs:2,0);

		
		% \draw[dotted] (axis cs:2,1) -- (axis cs:2,2);
		% \draw[ultra thick] (axis cs:2,2) -- (axis cs:4,2);
		% \draw[dotted] (axis cs:4,2) -- (axis cs:4,0);
		% \draw[dotted] (axis cs:2,2) -- (axis cs:0,2);
		
		% \draw[dotted] (axis cs:4,2) -- (axis cs:4,3);
		% \draw[ultra thick] (axis cs:4,3) -- (axis cs:6,3);
		% \draw[dotted] (axis cs:6,3) -- (axis cs:6,4);
		% \draw[dotted] (axis cs:8,4) -- (axis cs:8,5);
		% \draw[dotted] (axis cs:4,3) -- (axis cs:0,3);
		
		% \draw[dotted] (axis cs:6,3) -- (axis cs:6,4);
		% \draw[ultra thick] (axis cs:6,4) -- (axis cs:8,4);
		% \draw[dotted] (axis cs:8,4) -- (axis cs:8,0);
		% \draw[dotted] (axis cs:6,4) -- (axis cs:0,4);
		% \draw[dotted] (axis cs:6,3) -- (axis cs:6,0);
		
		% \draw[thick,dashed] (axis cs:0,1) -- (axis cs:8,5);
		
		
		\draw[thick, dashed,  ->] (axis cs:2,3) -- (axis cs:2.7,2.5) node[pos=0.1, above] {\huge $\gamma_{r_f,l_f}$};
		
		% \draw[thick,  ->] (axis cs:6,2.3) -- (axis cs:5,2.8) node[pos=0.1, below] {\Large $\nu_{p,b}$};
		
% 		\draw[dashed ->] (axis cs:6,0.5) -- (axis cs:5,0.7) node[pos=0.1, right] {\Large $\beta_{c,L}$};
		
% 		\draw[dashed ->] (axis cs:8,1.5) -- (axis cs:7,2) node[pos=0.1, right] {\text{non-convex service curve}};

		
		% %x axis
		\draw (1,-0.5) node{\large$\phi_f$};
            \draw (3,-0.5) node{\large$\phi_f + \tau_f$};
            \draw (5,-0.5) node{\large$\phi_f + 2\tau_f$};
            \draw (7,-0.5) node{\large$\phi_f + 3\tau_f$};
            \draw (9,-0.5) node{\large$\phi_f + 4\tau_f$};
		% \draw (4,-1) node{$2p$};
		% \draw (6,-1) node{$3p$};
		% \draw (8,-1) node{$4p$};

		
		% %y axis
		\draw (-.5,1) node{\large$l_f$};
             \draw (-.5,2) node{\large$2l_f$};
             \draw (-.5,3) node{\large$3l_f$};
             \draw (-.5,4) node{\large$4l_f$};
		% \draw (-1,2) node{$2b$};
		% \draw (-1,3) node{$3b$};
		% \draw (-1,4) node{$4b$};


		

\end{axis}
\end{tikzpicture}% NO EMPTY LINE HERE!!!! 

==> assumptions.tex <==
\section{Assumptions and Problem Statement} \label{sec:assump_prob}
% \hossein{
% \begin{enumerate}
%     \item Assumptions
%     \item Discussion on stationarity.
%     \item Discussion on ergodicity.
%     \item Problem Statement
% \end{enumerate}}
\subsection{Assumptions}\label{sec:assump}
We consider $n$ periodic flows of packets. Each flow $f = 1:n$  is periodic with period $\tau_f$ and sends packets  of size $l_f$; we pick a time origin and let $\phi_f$ (phase) denote the emission time of the first packet. We assume that $\phi_f$ is uniformly distributed in $[0,\tau_f]$, and that the different $\phi_f$, $f = 1:n$, are independent random variables.

% \begin{figure}[htbp]
% \centering
%     \scalebox{1}{\input{Figures/arrivals}}
% 	\caption{\sffamily \small Traffic of flow $f$: Starting from phase $\phi_f$, flow $f$ periodically sends packets of constant size $l_f$  with period $\tau_f$. The traffic is constrained by a deterministic token-bucket arrival curve $\gamma_{r_f,l_f}$ defined for $t> 0$ by $\gamma_{r_f,l_f}(t)=l_f + r_ft$ and for $t=  0$ by $\gamma_{r_f,l_f}(0)=0$; note that $r_f = \frac{l_f}{\tau_f}$.}
% 	\label{fig:periodic}
% \end{figure}


\subsection{Problem Statement} \label{sec:prob_state}
We say a flow is constrained by a token-bucket arrival curve with rate $r$ and burst $b$ if $\forall s \leq t,~ A(s,t] \leq r(t - s) + b$ where we let $A(s,t]$ denote the number of bits observed in time interval $(s,t]$. 
% the number of bits observed for this flow for any $s \leq t$ is upper bounded by $r(t-s) + b$, i.e., $\forall s \leq t,~ A(s,t] \leq r(t - s) + b$ where we let $A(s,t]$ denote the number of bits observed in time interval $(s,t]$. 
% % This definition is a deterministic constraint on the flow. 
It follows, from the assumptions, that each flow $f=1:n$ is constrained  by a token-bucket arrival curve with rate $r_f= \frac{l_f}{\tau_f}$ and burst $l_f$.
% defined by $\gamma_{r_f,l_f}(t) = r_ft+l_f$ for $t > 0$ and  $\gamma_{r_f,l_f}(t) = 0$ for $t =0$ with $r_f = \frac{l_f}{\tau_f}$. 
% Also, the aggregate traffic has a deterministic, token-bucket arrival curve $\gamma_{\rtot,\ltot}$ with $\rtot = \sum_{f = 1}^Fr_f$ and $\ltot = \sum_{f = 1}^Fl_f$. 
Also, their aggregate traffic is constrained by a token-bucket arrival curve with rate $\rtot = \sum_{f = 1}^nr_f$ and burst $\ltot = \sum_{f = 1}^nl_f$.
% , where $\ltot $ is the deterministic bound on the aggregate burstiness and is achieved when all phases are identical, i.e., when all flows are perfectly synchronized; this is highly unlikely in practice. In fact, the aggregate burstiness would likely be smaller when flows are not synchronized.
% In contrast, we assume that phases are independent, and we have no other information on them, which corresponds to the maximum entropy, thus, we assume uniform distribution.

We are interested in token-bucket arrival curves  with rate $\rtot$ and burst $b$ for the aggregate traffic that is valid with some probability; specifically, we want to find a bound on the tail probability of the aggregate burstiness.
% bound the probability that the aggregate burstinss exceeds some value $b$ with a small probability $\epsilon(b)$, which we call a bound on the tail probability of the aggregate burstiness.
To address this, we first  introduce the aggregate burstiness $\bar{B}(t)$ at time $t$ which is defined as the smallest value of the burst such that the aggregate traffic is constrained by a token-bucket arrival curve with rate $\rtot$ and burst $\bar{B}(t)$, when observing the aggregate traffic up to time $t$. The value of  $\bar{B}(t)$ is given by
% We let $B(t)$ denote the aggregate burstiness at time $t$, and is given by 
\begin{equation} \label{eq:agg_burst_t}
    \bar{B}(t) = \sup_{s \leq t} \{ A(s,t] - \rtot(t - s) \}
\end{equation}
% where $A(s,t]$ is the number of bits observed in time interval $(s,t]$ for the aggregate traffic. 
Thus, the aggregate burstiness is given by 
\begin{equation}\label{eq:agg_burst}
    B = \sup_{t \geq 0}\Bar{B}(t)
\end{equation}
and $B$ is the smallest value of the burst such that the aggregate traffic is constrained by a token-bucket arrival curve with rate $\rtot$ and burst $B$ throughout the entire network's lifetime.

 Observe that $ \P(B > b) =0$ for all $b \geq \ltot$, as $\ltot$ is a deterministic bound on the aggregate burstiness. Then, for some pre-specified value $0 \leq b < \ltot$, our problem is equivalent to finding $\epsilon(b) $ that bounds the tail probability of the aggregate burstiness $B$, i.e.,
\begin{equation} \label{eq:prob}
     \P(B > b) \leq \epsilon(b)
\end{equation}
% \begin{equation} \label{eq:prob}
%      \P(\sup_{t \geq 0}B(t) > b) = \P\lp \exists t \geq 0,~ B(t) > b\rp \leq \epsilon(b) 
% \end{equation}
% The token-bucket function with rate $\rtot$ and burst $b$ is a valid arrival curve for the aggregate with the violation probability of at most $\epsilon(b)$.
% , i.e., is valid with the probability of at least $1 - \epsilon(b)$.






% we want to bound the probability that



% \subsection{Properties}

% By A2 it follows that each flow $f$ is constrained  by a token-bucket arrival curve defined by $\gamma_{r_f,l_f}(t) = r_ft+l_f$ for $t>0$ and $\gamma_{r_f,b_f}(t)=0$ for $t= 0$ with $r_f = \frac{l_f}{\tau_f}$. Having a token-bucket arrival curve with a rate $r_f$ and a burst $b_f$ means that the number of bits observed for this flow in any time interval of duration $\tau$ cannot be more than $b_f + r_f\tau$ bits.

% We let $B(t)$ denote he aggregate burstiness $B(t)$ at time $t$, and is given by
% \begin{equation} \label{eq:agg_burst}
%     B(t) \isdef \sup_{s \leq t} \{ A(t) - A(s) - \rtot(t - s) \}
% \end{equation}
% The aggregate traffic $A$ has a deterministic, token-bucket arrival curve $\gamma_{\rtot,\ltot}$ with $\rtot = \sum_{f \in \calF}r_f$ and $\ltot = \sum_{f \in \calF}l_f$. Thus, it follows that $\ltot $ is a deterministic bound on aggregate burstiness, i.e.,
% \begin{equation} 
%     B(t) \leq  \sum_{f \in \calF}l_f = \ltot 
% \end{equation}

% In our case, arrival processes are packetized and periodic. Let us denote by $T_i$ and $L_i$ the arrival time and packet size of the $i$-th packet in the aggregate traffic. Then, for all $i \geq 1$, We have $A(T_i) = \sum_{k=1}^iL_j$. Then, \eqref{eq:agg_burst} can be rewritten as follows:
% \begin{equation} \label{eq:agg_burst_period}
%     B(t) = \sup_{i \leq j} \{ \sum_{k=i}^jL_k - \rtot(T_j - T_i) \}
% \end{equation}






==> conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}
For independent, periodic flows, we provided quasi-deterministic bounds on the aggregate burstiness, with small violation tolerance, that are considerably less than those obtained if we do not allow any probability of violation (deterministic bounds).  We obtained a closed-form expression for the homogeneous case, and for the heterogeneous case, we combined bounds obtained for homogeneous sets using the convolution bounding technique. 
% Deterministic network calculus can  then be applied  to obtain delay and backlog bounds that are valid with  probability of at least $1 - \varepsilon$. 



% We consider independent, periodic flows and are interested in bounding the burstiness of their aggregate traffic, which is crucial for effective resource management in time-sensitive networks. The deterministic bound is tight only when flows are perfectly synchronized, which is highly unlikely in practice and results in an overly pessimistic bound. We compute the probability that the aggregate burstiness exceeds some value. When all flows have the same period and packet size, we obtain a closed-form bound using the Dvoretzky–Kiefer–Wolfowitz (DKW) inequality. In the heterogeneous case, we group flows and combine the bounds obtained for each group using the convolution bound, which we derive by Abel's summation. Our bounds are numerically close to simulations and thus fairly tight. The resulting aggregate burstiness estimated for a non-zero violation probability is considerably smaller than the deterministic one; it grows in $\sqrt{n\log{n}}$, unlike the deterministic one that grows in  $n$, where $n$ is the number of flows.

==> heterogeneous.tex <==
\section{Heterogeneous Case} \label{sec:heterogen}

In this section, we consider the case where flows have different periods and packet sizes. We present two theorems; the former obtains a bound by grouping flows into  homogeneous sets and combining the bounds obtained for each set, using a convolution bounding technique, which we present in Proposition~\ref{prop:conv}. The latter, for a specific case, when flows have the same period and different packet sizes, provides an alternative bound that may be better when the number of flows per packet size is small.

% \hossein{
% \begin{enumerate}
%     \item Theorem 3: Same Period but Different Packet sizes
%     \item Theorem 4: Different Period and Packet sizes, Convolution Bound (Heterogeneous flows)
% \end{enumerate}}


\begin{proposition}[Convolution Bound]\label{prop:conv}
    Let $X_1,X_2,\ldots,X_g$ be $g \geq 2$ independent random variables with $X_i \in \Nats$ for  $i=1:g$.  Assume that $\Psi_i$ is wide-sense increasing and is a lower bound on the CDF of $X_i$, namely, $\P(X_i \leq b) \geq \Psi_i(b)$ for $b \in \Nats$ and $i=1:g$. Define $\psi_i$ by $\psi_i(0) = \Psi_i(0)$ and $\psi_i(b)=\Psi_i(b)-\Psi_i(b-1)$ for $b>0, b\in \Nats$ and $i=1:g$. 

    Then, a lower bound on the CDF of $\sum_{i=1:g}X_i$ is given by
    \begin{equation}\label{eq:convBound}
        \P (\sum_{i=1:g}X_i \leq b ) \geq \Psi_{1,2,\ldots,g}(b), \;\;\; b\in \Nats
    \end{equation}
    with  
    \begin{equation}\label{eq:psi}
        \Psi_{1,2,\ldots,g}(b) \isdef \lp\psi_1*\psi_2*\ldots*\psi_{g-1}*\Psi_{g} \rp(b), \;\;\; b\in \Nats
    \end{equation}
    In the above, the symbol $*$ denotes the discrete convolution, defined for arbitrary functions $f_1,f_2:\Nats \to \mathbb{R}$ by
    \begin{equation}\label{eq:discConv}
    (f_1* f_2)(b) = \sum_{j=0}^{b} f_1(j) f_2(b-j), \;\;\; b\in \Nats
    \end{equation}
\end{proposition}
\begin{proof}
    % We first  show the result when $g=2$, then extend it to $g > 2$. 
    We prove it by induction on $g$.
    
    \textbf{Base Case $g=2$:}
    We need to show that
    % $\P( X_1 + X_2 \leq b) \geq \Psi_{1,2}(b)$, for $b\in \Nats$, with
    \begin{equation} \label{eq:conv}
        \P( X_1 + X_2 \leq b) \geq \Psi_{1,2}(b)= (\psi_1 * \Psi_2)(b)
        % =  (\psi_2 * \Psi_1)(b)
    \end{equation}
    
    % we show that $\P( X_1 + X_2 \leq b) \geq \Psi_{1,2}(b) = (\psi_1 * \Psi_2)(b)$.
    % Consider two groups, say $1$ and $2$; we show that
    % $\P( X_1 + X_2 \leq b) \geq \Psi_{1,2}(b)$, for $b\in \Nats$, with
    % \begin{equation} \label{eq:conv}
    %     \Psi_{1,2}(b)= (\psi_1 * \Psi_2)(b) =  (\psi_2 * \Psi_1)(b)
    % \end{equation}
    
    Let $F_i(b)=\P(X_i\leq b)$, $i=1:2$. Observe that $\P(X_i = 0) = F_i(0)$ and $\P(X_i=b)=F_i(b)-F_i(b-1)$ for $b>0,b\in\Nats$. Then 
    {\footnotesize
    \begin{align}
    \P(X_1+X_2\leq b)  &=\sum_{j=0}^{b}\P(X_1+j\leq b | X_2=j)\P(X_2= j) = \sum_{j=0}^{b}\P(X_1+j\leq b )\P(X_2= j)\\
% &=&    \sum_{j=0}^{b}\P(X_1+j\leq b )\P(X_2= j)\\
&= \sum_{j=0}^{b}F_1(b-j)\P(X_2= j) \geq \sum_{j=0}^{b}\Psi_1(b - j)\P(X_2= j) 
\\
    % &\geq&\sum_{j=0}^{b}\Psi_1(b - j)\P(X_2= j) \\
    &\geq\Psi_1(b)F_2(0) + \sum_{j=1}^{b}\Psi_1(b - j)(F_2(j)-F_2(j-1)) 
    \label{eq:last}
    \end{align}}

% \begin{eqnarray}
%     &=&\sum_{j=0}^{b}\P(X_1+j\leq b | X_2=j)\P(X_2= j) = \sum_{j=0}^{b}\P(X_1+j\leq b )\P(X_2= j)\\
% % &=&    \sum_{j=0}^{b}\P(X_1+j\leq b )\P(X_2= j)\\
% &=& \sum_{j=0}^{b}F_1(b-j)\P(X_2= j) \geq \sum_{j=0}^{b}\Psi_1(b - j)\P(X_2= j) 
% \\
%     % &\geq&\sum_{j=0}^{b}\Psi_1(b - j)\P(X_2= j) \\
%     &\geq&\Psi_1(b)F_2(0) + \sum_{j=1}^{b}\Psi_1(b - j)(F_2(j)-F_2(j-1)) 
%     \label{eq:last}
% \end{eqnarray}
% \begin{eqnarray}
%     \P(X_1+X_2\leq b)&=&\sum_{j=0}^{b}\P(X_1+j\leq b | X_2=j)\P(X_2= j)\\
% &=&    \sum_{j=0}^{b}\P(X_1+j\leq b )\P(X_2= j)\\
% &=& \sum_{j=0}^{b}F_1(b-j)\P(X_2= j)
% \\
%     &\geq&\sum_{j=0}^{b}\Psi_1(b - j)\P(X_2= j) \\
%     &\geq&\Psi_1(b)F_2(0) + \sum_{j=1}^{b}\Psi_1(b - j)(F_2(j)-F_2(j-1)) 
%     \label{eq:last}
% \end{eqnarray}
% \begin{align}
% \P(X_1+X_2\leq b)&=\sum_{j=0}^{b}\P(X_1+j\leq b | X_2=j)\P(X_2= j) \nonumber \
% &=\sum_{j=0}^{b}\P(X_1+j\leq b)\P(X_2= j) \nonumber \
% &=\sum_{j=0}^{b}F_1(b-j)\P(X_2=j) \nonumber \
% &\geq\sum_{j=0}^{b}\Psi_1(b-j)\P(X_2=j) \nonumber \
% &\geq\Psi_1(b)F_2(0) + \sum_{j=1}^{b}\Psi_1(b-j)(F_2(j)-F_2(j-1)) \label{eq:last}
% \end{align}
% \begin{align}
%         &= \sum_{j=0}^{b}\P(X_1+j\leq b | X_2=j)\P(X_2= j) =    \sum_{j=0}^{b}\P(X_1+j\leq b )\P(X_2= j)\\
%         &=   \sum_{j=0}^{b}F_1(b-j)\P(X_2= j) \geq \sum_{j=0}^{b}\Psi_1(b - j)\P(X_2= j)\\
% % &=   \sum_{j=0}^{b}F_1(b-j)\P(X_2= j)
% % \\
%     & \geq \Psi_1(b)F_2(0) + \sum_{j=1}^{b}\Psi_1(b - j)(F_2(j)-F_2(j-1))
%     % \\
%     % &\geq \Psi_1(b)F_2(0) + \sum_{j=1}^{b}\Psi_1(b - j)(F_2(j)-F_2(j-1)) 
%     \label{eq:last}
% \end{align}
We use Abel's summation by parts in \eqref{eq:last} and obtain $\P(X_1+X_2\leq b) $
 \begin{align}
    % \P(X_1+X_2\leq b) 
    \P(X_1+X_2\leq b) &\geq\Psi_1(b)F_2(0) + \sum_{j=1}^{b}\Psi_1(b - j)F_2(j)- \sum_{j=1}^{b}\Psi_1(b - j)F_2(j-1)
    \\
    &=
    \Psi_1(b)F_2(0) + \sum_{j=1}^{b}\Psi_1(b - j)F_2(j)- \sum_{j=0}^{b-1}\Psi_1(b - j - 1)F_2(j)
    \\
    &=
    \sum_{j=0}^{b}\Psi_1(b - j)F_2(j)- \sum_{j=0}^{b-1}\Psi_1(b - j - 1)F_2(j)
    \\
    &=
     \Psi_1(0)F_2(b) + \sum_{j=0}^{b-1}(\Psi_1(b - j) - \Psi_1(b - j- 1))F_2(j)\\
    &=
    \psi_1(0)F_2(b) + \sum_{j=0}^{b-1}\psi_1(b - j)F_2(j) = \sum_{j=0}^{b}\psi_1(b - j)F_2(j)
    \\
    &=
     \sum_{j=0}^{b}\psi_1(b - j)F_2(j) \geq \sum_{j=0}^{b}\psi_1(b - j)\Psi_2(j)= \Psi_{1,2}(b)
\end{align}
%  \begin{eqnarray}
%     % \P(X_1+X_2\leq b) 
%     \P(X_1+X_2\leq b) &\geq&\Psi_1(b)F_2(0) + \sum_{j=1}^{b}\Psi_1(b - j)F_2(j)- \sum_{j=1}^{b}\Psi_1(b - j)F_2(j-1)
%     \\
%     &=&
%     \Psi_1(b)F_2(0) + \sum_{j=1}^{b}\Psi_1(b - j)F_2(j)- \sum_{j=0}^{b-1}\Psi_1(b - j - 1)F_2(j)
%     \\
%     &=&
%     \sum_{j=0}^{b}\Psi_1(b - j)F_2(j)- \sum_{j=0}^{b-1}\Psi_1(b - j - 1)F_2(j)
%     \\
%     &=&
%      \Psi_1(0)F_2(b) + \sum_{j=0}^{b-1}(\Psi_1(b - j) - \Psi_1(b - j- 1))F_2(j)\\
%     &=&
%     \psi_1(0)F_2(b) + \sum_{j=0}^{b-1}\psi_1(b - j)F_2(j) = \sum_{j=0}^{b}\psi_1(b - j)F_2(j)
%     \\
%     &=&
%      \sum_{j=0}^{b}\psi_1(b - j)F_2(j) \geq \sum_{j=0}^{b}\psi_1(b - j)\Psi_2(j)= \Psi_{1,2}(b)
% \end{eqnarray}
which shows the base case. 
% We now proceed to show that $(\psi_1 * \Psi_2) = (\Psi_1 * \psi_2)$
% \textbf{Step 2 (Abel's summation):}  We use Abel's summation by parts in \eqref{eq:last} and obtain
%  \begin{eqnarray}
%     \P(X_1+X_2\geq b) 
%     &\leq&\sum_{j=0}^{b}\Phi_1(b - j)F_2(j)-\sum_{j=0}^{b}\Phi_1(b - j)F_2(j+1) + F_2(b+1)
%     \\
%     &=&
%     \sum_{j=0}^{b}\Phi_1(b - j)F_2(j)-\sum_{j=1}^{b+1}\Phi_1(b - j+1)F_2(j) + F_2(b+1)
%     \\
%     &=&
%     \sum_{j=0}^{b}\Phi_1(b - j)F_2(j)-\sum_{j=0}^{b} \Phi_1(b - j+1)F_2(j)+\Phi_1(b+1) - F_2(b+1) + F_2(b+1)
%     \\
%     &=&
%     \sum_{j=0}^{b}\Phi_1(b - j)F_2(j)-\sum_{j=0}^{b} \Phi_1(b - j+1)F_2(j)+\Phi_1(b+1)\\
%     &=&
%     \sum_{j=0}^{b}(\Phi_1(b - j)-\Phi_1(b - j+1))F_2(j)+\Phi_1(b+1)
%     \\
%     &=&
%     \sum_{j=0}^{b}\varphi_1(b - j)F_2(j)+\Phi_1(b+1)\isdef \Phi_{1,2}(b)
% \end{eqnarray}
% Hence, \eqref{eq:conv} is shown.
% Observe that
%  \begin{eqnarray}
%     (\psi_1 * \Psi_2)(b)
%     &=&\sum_{j=0}^{b}\Psi_1(b - j)\Psi_2(j) - \sum_{j=1}^{b}\Psi_1(b - j)\Psi_2(j) 
%     \\
%     &=&
%     \sum_{i,j s.t. i + j = b, i,j \geq 0 }\Psi_1(i)\Psi_2(j)  +  \sum_{i,j s.t. i + j = b - 1, i,j \geq 0 }\Psi_1(i)\Psi_2(j) 
% \end{eqnarray}
% which is symmetric in indices 1,2 and thus shows that $\psi_1 * \Psi_2 = \Psi_1 * \psi_2$. Hence, \eqref{eq:conv} is shown. 

 \textbf{Induction Case:}
We now assume that the convolution bound holds for up to $k \geq 2$ variables, and we show that it also holds for $k+1$ variables. 

By the induction hypothesis, for variables $X_2, X_3, \ldots, X_{k+1}$ we have 
\begin{equation}
    \P( \sum_{i=2:(k+1)}X_i \geq b) \leq (\psi_2*\psi_3*\ldots*\Psi_{k+1})(b) = \Psi_{2,\ldots,k+1}(b),~ b \in \Nats
\end{equation}
Observe that $X_1$ and $\sum_{i=2:(k+1)}X_i$ are independent; also,  by the induction hypothesis, the convolution bound holds for two variables. Thus $\forall b \in \Nats$,
% We now apply the base case where we replace $X_2$ be $\sum_{i=2:(k+1)}X_i $ and we obtain
\begin{equation}
    \P( X_1 + \sum_{i=2:(k+1)}X_i \geq b) \leq (\psi_1 *\Psi_{2,\ldots,k+1})(b) =  (\psi_1 *(\psi_2*\psi_3*\ldots*\Psi_{k+1}))(b)
\end{equation}
The induction step is concluded by associativity of the discrete convolution.
% We now iteratively apply \eqref{eq:conv} and obtain $ \P\lp \sum_{i=1=:g}  X_i \leq b \rp \geq \lp\psi_1*\psi_2*\ldots*\psi_{g-1}*\Psi_{g} \rp(b) =  \Psi_{1,2,\ldots,g}(b)$ for $b\in \Nats$, 
% % \begin{equation} \label{eq:hs3}
% %     \Psi_{1,2,\ldots,g}(b) = \lp\psi_1*\psi_2*\ldots*\psi_{g-1}*\Psi_{g} \rp(b), \;\;\; b>0,b\in \Nats
% % \end{equation}
% which concludes the proposition.
\qed
\end{proof}


Note that $\psi_1 * \Psi_2 = \Psi_1 * \psi_2$ as $ (\psi_1 * \Psi_2)(b) =\sum_{j=0}^{b}\Psi_1(b - j)\Psi_2(j) - \sum_{j=1}^{b}\Psi_1(b - j)\Psi_2(j) = \sum_{i,j s.t. i + j = b, i,j \geq 0 }\Psi_1(i)\Psi_2(j)  +  \sum_{i,j s.t. i + j = b - 1, i,j \geq 0 }\Psi_1(i)\Psi_2(j)$ which is symmetric in indices 1,2. Thus, the convolution bound is independent of the labeling of the variables, i.e.,  $ \psi_1*\psi_2*\ldots*\psi_{g-1}*\Psi_{g} = \psi_1*\psi_2*\ldots*\psi_{g-2}*\psi_{g}*\Psi_{g-1} = \ldots =   \psi_2*\ldots*\psi_{g-1}*\psi_{g}*\Psi_{1} $. 

% in \eqref{eq:convBound}, the index of $\Psi_g$  can be swapped by the index of any $\psi_i$ for $i = 1:g-1$ without affecting the bound, i.e., $ \psi_1*\psi_2*\ldots*\psi_{g-1}*\Psi_{g} = \psi_1*\psi_2*\ldots*\psi_{g-2}*\psi_{g}*\Psi_{g-1} = \ldots =   \psi_2*\ldots*\psi_{g-1}*\psi_{g}*\Psi_{1} $. 

\textbf{Remark.} An alternative  to Proposition~\ref{prop:conv} is to use union bound rather than the convolution bound. Specifically, consider some $b$ and a collection $(b_1,b_2, \ldots, b_g)$ such that $\sum_{i=1}^gb_i = b$ and $b_i\geq 0$; then, observe that $\bigcap_{i=1}^g\lc X_i \leq b_i \rc \subseteq \lc \sum_{i=1:g}X_i \leq \sum_{i=1:g}b_i \rc$ and thus, by contraposition, $\lc \sum_{i=1:g}X_i  > b \rc \subseteq \bigcup_{i=1}^g\lc X_i > b_i \rc$. It follows that $\P( \sum_{i=1:g}X_i >  b) \leq \sum_{i=1:g}\P\lp X_i >  b\rp \leq \sum_{i=1:g}(1 - \Psi_i(b_i))$. Thus, one can compute a collection $(b_1,b_2, \ldots, b_g)$ that minimizes the right-hand side, and obtain
\begin{equation}
    \P( \sum_{i=1:g}X_i  \leq  b) \geq 1 - \lp \lp 1 - \Psi_1 \rp \otimes  \lp 1 - \Psi_2 \rp \otimes \ldots \otimes  \lp 1 - \Psi_g \rp \rp(b)
\end{equation}
% $\P\lp \sum_{i=1:g}X_i  \leq  b\rp \geq 1 - \lp (1 - \Psi_1)\otimes (1 - \Psi_2)\otimes \ldots \otimes (1 - \Psi_g) \rp(b)$ 
where $\otimes$ denotes the discrete min-plus convolution defined for two arbitrary functions $f_1,f_2: \mathbb{N} \to \mathbb{R}$ by $(f_1 \otimes f_2)(b) = \inf_{0 \leq b' \leq b}\{f_1(b') + f_2(b - b') \}$. It can be shown that the convolution bound always dominate the union bound; however, note that the union bound does not require that random variables $X_i$ be independent. In our numerical evaluations, we find that the convolution bound provides significantly
better results than the union bound. 
% 1 - (1 - \Psi_1)\oslash (1 - \Psi_2)\oslash \ldots \oslash (1 - \Psi_g)$.


% This is because  $\footnotesize (\psi_1 * \Psi_2)(b) =\sum_{j=0}^{b}\Psi_1(b - j)\Psi_2(j) - \sum_{j=1}^{b}\Psi_1(b - j)\Psi_2(j) = \sum_{i,j s.t. i + j = b, i,j \geq 0 }\Psi_1(i)\Psi_2(j)  +  \sum_{i,j s.t. i + j = b - 1, i,j \geq 0 }\Psi_1(i)\Psi_2(j)$ which symmetric in indices 1,2 and thus shows that $\psi_1 * \Psi_2 = \Psi_1 * \psi_2$. 


% Group flows in homogeneous sets and   bounds on the tail probability of the  aggregate burstiness of each group (functions $\varepsilon_i$ for each group $i$) can be obtained by  our results for the homogeneous case in Section~\ref{sec:homogen}. Theorem~\ref{thm:hetero} then provides a convolution technique to combine these bounds and bound the tail probability of the aggregate burstiness of all flows; it can be efficiently computed using discrete convolution.


\begin{theorem}[Flows with different periods and different packet-sizes] \label{thm:hetero}
Assume the assumption of Section~\ref{sec:assump}, and group flows into $g \geq 2$ homogeneous sets (i.e., flows of each group have the same packet size and period). For each group $i = 1:g$, compute a bound on the tail probability of their aggregate burstiness $B_i$ using Theorem~\ref{thm:homog_dkw}, namely function $\varepsilon_i$ such that  $ \P\lp B_i > b\rp \leq \varepsilon_i(b)$  for all $b\in \Nats$.
% $\varepsilon_i(b)$  which is a bound on the tail probability of $B_i$, the aggregate burstiness of group $i$, using Theorem~\ref{thm:homog_dkw}, namely,  $ \P\lp B_i > b\rp \leq \varepsilon_i(b)$  for all $b\in \Nats$.
Define $\Psi_i(b) = 1 - \varepsilon_i(b)$ for $b\in \Nats$ and define $\psi_i$ by $\psi_i(0) = \Psi_i(0)$ and $\psi_i(b)=\varepsilon_i(b-1)-\varepsilon_i(b)$ for $b>0, b\in \Nats$. Also, Define $\Psi_{1,2,\ldots,g}$ as in \eqref{eq:psi}.

Then, a bound on the tail probability of the aggregate burstiness of all flows $B$ is given by
\begin{equation} \label{eq:eps_hetero}
     \P\lp B > b\rp \leq 1 - \Psi_{1,2,\ldots,g}(b) \isdef \varepsilon_{1,2,\ldots,g}(b), \;\;\; b < \ltot,b\in \Nats
\end{equation}
% with $\varepsilon_{1,2,\ldots,g}(0) = 1 $ and 
% \begin{align}
% \varepsilon_{1,2,\ldots,g}(b) = 1 - \lp\psi_1*\psi_2*\ldots*\psi_{g-1}*\Psi_{g} \rp(b), \;\;\; b>0,b\in \Nats
% \end{align} 
% The symbol $*$ denotes the discrete convolution, defined in \eqref{eq:discConv}. 
% Consider $g$ homogeneous groups (i.e., flows of each group have the same packet size and period).
% Also, assume that, for $i = 1:g$, $ \P\lp B_i > b\rp \leq \varepsilon_i(b)$ for all $b\in \Nats$ where $B_i$ is the aggregate burstiness of group $i$ and $\varepsilon_i$ is wide-sense decreasing and $\varepsilon_i(0) = 1$. 
% Define $\Psi_i(b) = 1 - \varepsilon_i(b)$ for $b\in \Nats$ and define $\psi_i$ by $\psi_i(0) = 0$ and $\psi_i(b)=\varepsilon_i(b-1)-\varepsilon_i(b)$ for $b>0, b\in \Nats$. Consider some $b \in \Nats$. Then, a bound on the tail probability of the aggregate burstiness of all groups $B$ is given by
% \begin{equation} \label{eq:eps_hetero}
%      \P\lp B > b\rp \leq \varepsilon_{1,2,\ldots,g}(b)
% \end{equation}
% with $\varepsilon_{1,2,\ldots,g}(0) = 1 $ and 
% \begin{align}
% \varepsilon_{1,2,\ldots,g}(b) = 1 - \lp\psi_1*\psi_2*\ldots*\psi_{g-1}*\Psi_{g} \rp(b), \;\;\; b>0,b\in \Nats
% \end{align} 
% Also, the index of $\Psi_g$  can be swapped by the index of any $\psi_i$ for $i = 1:g-1$ without affecting the bound, i.e., $ \psi_1*\psi_2*\ldots*\psi_{g-1}*\Psi_{g} = \psi_1*\psi_2*\ldots*\psi_{g-2}*\psi_{g}*\Psi_{g-1} = \ldots =   \psi_2*\ldots*\psi_{g-1}*\psi_{g}*\Psi_{1} $.
% \begin{align}
%     \psi_1*\psi_2*\ldots*\psi_{g-1}*\Psi_{g} &= \psi_1*\ldots*\psi_{g-2}*\psi_{g}*\Psi_{g-1} = \ldots =   \psi_2*\ldots*\psi_{g-1}*\psi_{g}*\Psi_{1} 
%     % \psi_2*\ldots*\psi_{g-1}*\psi_{g}*\Psi_{1} =\psi_1*\psi_3*\ldots*\psi_{g}*\Psi_{2}=\\
%     % \ldots&=\psi_1*\psi_2*\ldots*\psi_{g-2}*\psi_{g}*\Psi_{g-1}
% \end{align} 
% \begin{align}
%      \varepsilon_{1,2,\ldots,g}(0) &= 1 \\
%      \varepsilon_{1,2,\ldots,g}(b) &= 1 - \lp\psi_1*\psi_2*\ldots*\psi_{g-1}*\Psi_{g} \rp,~b>0,b\in \Nats
% \end{align} 
% \begin{align}
%      \varepsilon_{1,2,\ldots,g}(0) &= 1 \\
%      \varepsilon_{1,2,\ldots,g}(0) &= 1 - \lp\psi_1*\psi_2*\ldots*\psi_{g-1}*\Psi_{g} \rp = 1 - \lp\psi_2*\psi_3*\ldots*\psi_{g}*\Psi_{1} \rp \\
%      &= 1 - \lp\psi_1*\psi_3*\psi_4*\ldots*\psi_{g}*\Psi_{2} \rp = \ldots =  1 - \lp\psi_1*\psi_2*\ldots*\psi_{g-2}*\Psi_{g-1} \rp \ldots
% \end{align} 
% \label{eq:eps_hetero}
%         \varepsilon_{1,2,\ldots,g}(0) = 1 
%      \varepsilon_{1,2}(b) = (E_2 * \varepsilon_1)(b) + \varepsilon_2(b+1) = (E_1 * \varepsilon_2)(b) + \varepsilon_1(b+1)
% \end{equation}
% In the above, the symbol $*$ denotes the discrete convolution, defined by 
% \begin{equation}
%     (\psi* \Psi)(b) = \sum_{j=0}^{b} \psi(j) \Psi(b-j), \;\;\; b\in \Nats
% \end{equation}
\end{theorem}
% The essence of  Theorem~\ref{thm:hetero} is as follows: First, flows should be homogeneously grouped where bounds on the tail probability of the  aggregate burstiness of each group (functions $\varepsilon_i$ for each group $i$) can be obtained by  our results for the homogeneous case in Section~\ref{sec:homogen}. It then provides a convolution technique to combine these bounds and bound the tail probability of the aggregate burstiness of all flows. 

% % applied as follows:
% % \begin{enumerate}
% %     \item Group flows such that flows in each group either the same period and packet size or have the same period but different packet size.
% %     \item Compute the bounding function $\varepsilon$ as presented in Section~\ref{sec:homogen} and Section~\ref{sec:semi-homogen}, respectively, for each group.
% %     \item Apply Theorem~\ref{thm:hetero} find a bounding function for the aggregate of all flows.
% % \end{enumerate}
% The bound of Theorem~\ref{thm:hetero} is tight; specifically, $\varepsilon_{1,2,\ldots,g}$ is the best possible bounding function if the only information on different groups is their independence and the knowledge of their bounding functions  $\varepsilon_i$, for $i =1:g$. $\varepsilon_{1,2,\ldots,g}$ can be efficiently computed using  properties of discrete convolution, namely, associativity and commutativity \cite{Oppenheim2010}.
% this is because if $\varepsilon_i$ are tight, \eqref{eq:eps_hetero} becomes equality, hence $\varepsilon_{1,2,\ldots,g}$ is also tight.

% The bound of Theorem~\ref{thm:hetero} has a closed form, and one can use all properties of discrete convolution (e.g., associativity, commutativity, distributivity, etc.) \cite{Oppenheim2010} to compute it efficiently.  Moreover, the bound is tight, i.e., $\varepsilon_{1,2,\ldots,g}$ is the best possible bounding function if the only information on different groups  is their independence and the knowledge of their bounding functions  $\varepsilon_i$, for $i =1:g$; this is because if $\varepsilon_i$ are tight, \eqref{eq:eps_hetero} becomes equality, hence $\varepsilon_{1,2,\ldots,g}$ is also tight.

% Theorem~\ref{thm:hetero} can be applied as follows:
% \begin{enumerate}
%     \item Group flows such that flows in each group either the same period and packet size or have the same period but different packet size.
%     \item Compute the bounding function $\varepsilon$ as presented in Section~\ref{sec:homogen} and Section~\ref{sec:semi-homogen}, respectively, for each group.
%     \item Apply Theorem~\ref{thm:hetero} find a bounding function for the aggregate of all flows.
% \end{enumerate}


% For flows  with the same period and packet size and/or flows with the same period but different packet sizes, we can compute the bounding function $\varepsilon$ as presented in Section~\ref{sec:homogen} and Section~\ref{sec:semi-homogen}, respectively. Then, Theorem~\ref{thm:hetero}
% Theorem~\ref{thm:hetero} enables us to group flows into such groups and find a bounding function for the aggregate of all flows. 
% The bound of Theorem~\ref{thm:hetero} has a closed form, and one can use all properties of discrete convolution (e.g., associativity, commutativity, distributivity, etc.) \cite{Oppenheim2010} to compute it efficiently.  Moreover, the bound is tight, i.e., $\varepsilon_{1,2,\ldots,g}$ is the best possible bounding function if the only information on different groups  is their independence and the knowledge of their bounding functions  $\varepsilon_i$, for $i =1:g$; this is because if $\varepsilon_i$ are tight, \eqref{eq:eps_hetero} becomes equality, hence $\varepsilon_{1,2,\ldots,g}$ is also tight.



\begin{proof} 
    % We first show the following equation
    % \begin{equation} \label{eq:hs1}
    %     \P(  B \leq b) \geq \P( \sum_{i=1:g} \lceil B_i\rceil \leq b ), \;\;\; b\in \Nats
    % \end{equation} 
    % and for $b \in \Nats$,
    % \begin{equation}
    %     \P\lp \sum_{i=1}^g\sup_{t \geq 0}B_i(t) > b\rp \leq \P\lp \sum_{i=1}^g \lceil \sup_{t \geq 0}B_i(t) \rceil > b\rp 
    % \end{equation}
    
    Let us denote by $A_i(t,s]$, for $i = 1:g$, the arrival of the aggregate of flows of group $i$ in the interval $(s,t]$. Also,  let us denote by $r_i$, for $i = 1:g$,  the aggregate arrival rate of  flows of group $i$. Observe that for all $s\leq t$, $A(s,t] = \sum_{i=1}^gA_i(t,s]$ and $\rtot = \sum_{i=1}^gr_i$. Combine this by definition of $\bar{B}(t)$ in \eqref{eq:agg_burst_t} to obtain  $\forall t \geq 0$, $\Bar{B}(t) = \sup_{s \leq t} \{ A(s,t] - \rtot(t - s) \} =  \sup_{s \leq t} \lc  \sum_{i=1}^g \lp A_i(s,t] - r_i(t - s) \rp \rc
        \leq  \sum_{i=1}^g \sup_{s \leq t} \lc   A_i(s,t] - r_i(t - s) \rc = \sum_{i=1}^g\Bar{B}_i(t) $.
    % \begin{align}
    %     \Bar{B}(t) = \sup_{s \leq t} \{ A(s,t] - \rtot(t - s) \} &=  \sup_{s \leq t} \lc  \sum_{i=1}^g \lp A_i(s,t] - r_i(t - s) \rp \rc\\
    %     &\leq  \sum_{i=1}^g \underbrace{\sup_{s \leq t} \lc   A_i(s,t] - r_i(t - s) \rc}_{\Bar{B}_i(t)}
    % \end{align}
    %     \begin{align}
    %     \Bar{B}(t) = \sup_{s \leq t} \{ A(s,t] - \rtot(t - s) \} &=  \sup_{s \leq t} \lc  \sum_{i=1}^g \lp A_i(s,t] - r_i(t - s) \rp \rc\\
    %     &\leq  \sum_{i=1}^g \underbrace{\sup_{s \leq t} \lc   A_i(s,t] - r_i(t - s) \rc}_{\Bar{B}_i(t)}
    % \end{align}
    %     B(t) = \sup_{s \leq t} \{ A(s,t] - \rtot(t - s) \} =  \sup_{s \leq t} \lc  \sum_{i=1}^g \lp A_i(s,t] - r_i(t - s) \rp \rc \leq \sum_{i=1}^g
    % \end{equation}
Hence, it follows that $B = \sup_{t \geq 0}\Bar{B}(t) \leq \sum_{i=1}^g\sup_{t \geq 0}\Bar{B}_i(t) = \sum_{i=1}^gB_i$ and as $ \sum_{i=1}^g B_i \leq  \sum_{i=1}^g\lceil B_i\rceil$, we obtain $ \P(  B \leq b) \geq \P( \sum_{i=1:g} \lceil B_i\rceil \leq b ), \;\;\; b\in \Nats$ .
% shows \eqref{eq:hs1}.

We now apply Proposition~\ref{prop:conv} with  $X_i = \lceil B_i\rceil$ and $\Psi_i$ as the theorem defines. Observe the followings for $i=1:g$: $\lceil B_i\rceil \in \Nats$ and are independent; as $\varepsilon_i$ is wide-sense decreasing, $\Psi_i$ is  wide-sense increasing;   $\psi_i(0) = \Psi_i(0)$ and $\psi_i(b)=\Psi_i(b)-\Psi_i(b-1)$ for $b>0,b\in \Nats$. Hence, Proposition~\ref{prop:conv} can be applied and we obtain $\P( \sum_{i=1:g} \lceil B_i\rceil \leq b) \geq \Psi_{1,2,\ldots,g}(b), \;\;\; b\in \Nats$.
% \begin{equation} \label{eq:hs2}
%         \P( \sum_{i=1:g} \lceil B_i\rceil \leq b) \geq \Psi_{1,2,\ldots,g}(b), \;\;\; b\in \Nats
% \end{equation} 
Combine it with the previous paragraph to conclude the theorem. \qed
% \textbf{Step 2:} Consider two groups, say $1$ and $2$; we show the following: For $b\in \Nats$,
%     $\P(\lceil B_1 \rceil+\lceil B_2\rceil \leq b) \geq \Psi_{1,2}(b)$ with
%     \begin{equation} \label{eq:conv}
%         \Psi_{1,2}(b)= (\psi_1 * \Psi_2)(b) =  (\psi_2 * \Psi_1)(b)
%     \end{equation}
% For conciseness, we replace $\lceil B_i\rceil$ by $X_i$, for $i = 1:2$, in the rest of the proof. Observe that, first, $X_i \in \Nats$  for $i=1:2$, are  two independent random variables. 
% % Let $X_1, X_2$ be two independent random variables with $X_i\in \Nats$. 
% Second, by definition, $\Psi_i$ is a bound on the CDF of $X_i$, namely, $\P(X_i\leq b)\geq \Psi_i(b)$ for all $b \in \Nats$ and $i=1:2$. Third, observe that  $\psi_i(0) = \Psi_i(0)$ and $\psi_i(b)=\Psi_i(b)-\Psi_i(b-1)$ for $b>0,b\in \Nats$.
% by definition,  $\Psi_i$ is wide-sense increasing, i.e., $\Psi_i(b)\geq \Psi_i(b-1)$ for all $b>0,b \in \Nats$ and $i=1:2$. Lastly, observe that 
% $\psi_i(0) = \Psi_i(0)$ and $\psi_i(b)=\Psi_i(b)-\Psi_i(b-1)$ for $b>0,b\in \Nats$.
% Assume that $\Psi_i$ is a bound on the CDF of $X_i$, namely, $\P(X_i\leq b)\geq \Psi_i(b)$ for all $b \in \Nats$ and $i=1:2$. Also assume that $\Psi_i$ is wide-sense increasing, i.e., $\Psi_i(b)\geq \Psi_i(b-1)$ for all $b>0,b \in \Nats$ and $i=1:2$. Define $\psi_i$ by $\psi_i(0) = \Psi_i(0)$ and $\psi_i(b)=\Psi_i(b)-\Psi_i(b-1)$ for $b>0,b\in \Nats$.
% We show the following: For $b\in \Nats$,
%     $\P(\lceil\sup_{t \geq 0}B_1(t)\rceil+\lceil\sup_{t \geq 0}B_2(t)\rceil \leq b) \geq \Psi_{1,2}(b)$ with
%     \begin{equation} \label{eq:conv}
%         \Psi_{1,2}(b)= (\psi_1 * \Psi_2)(b) =  (\psi_2 * \Psi_1)(b)
%     \end{equation}
% \textbf{Step 2.1:} Let $F_i(b)=\P(X_i\leq b)$. Observe that $\P(X_i = 0) = F_i(0)$ and $\P(X_i=b)=F_i(b)-F_i(b-1)$ for $b>0,b\in\Nats$. Then $\P(X_1+X_2\leq b) $
% \begin{eqnarray}
%     &=&\sum_{j=0}^{b}\P(X_1+j\leq b | X_2=j)\P(X_2= j) = \sum_{j=0}^{b}\P(X_1+j\leq b )\P(X_2= j)\\
% % &=&    \sum_{j=0}^{b}\P(X_1+j\leq b )\P(X_2= j)\\
% &=& \sum_{j=0}^{b}F_1(b-j)\P(X_2= j) \geq \sum_{j=0}^{b}\Psi_1(b - j)\P(X_2= j) 
% \\
%     % &\geq&\sum_{j=0}^{b}\Psi_1(b - j)\P(X_2= j) \\
%     &\geq&\Psi_1(b)F_2(0) + \sum_{j=1}^{b}\Psi_1(b - j)(F_2(j)-F_2(j-1)) 
%     \label{eq:last}
% \end{eqnarray}
% \begin{eqnarray}
%     \P(X_1+X_2\leq b)&=&\sum_{j=0}^{b}\P(X_1+j\leq b | X_2=j)\P(X_2= j)\\
% &=&    \sum_{j=0}^{b}\P(X_1+j\leq b )\P(X_2= j)\\
% &=& \sum_{j=0}^{b}F_1(b-j)\P(X_2= j)
% \\
%     &\geq&\sum_{j=0}^{b}\Psi_1(b - j)\P(X_2= j) \\
%     &\geq&\Psi_1(b)F_2(0) + \sum_{j=1}^{b}\Psi_1(b - j)(F_2(j)-F_2(j-1)) 
%     \label{eq:last}
% \end{eqnarray}
% \begin{align}
% \P(X_1+X_2\leq b)&=\sum_{j=0}^{b}\P(X_1+j\leq b | X_2=j)\P(X_2= j) \nonumber \
% &=\sum_{j=0}^{b}\P(X_1+j\leq b)\P(X_2= j) \nonumber \
% &=\sum_{j=0}^{b}F_1(b-j)\P(X_2=j) \nonumber \
% &\geq\sum_{j=0}^{b}\Psi_1(b-j)\P(X_2=j) \nonumber \
% &\geq\Psi_1(b)F_2(0) + \sum_{j=1}^{b}\Psi_1(b-j)(F_2(j)-F_2(j-1)) \label{eq:last}
% \end{align}
% \begin{align}
%         &= \sum_{j=0}^{b}\P(X_1+j\leq b | X_2=j)\P(X_2= j) =    \sum_{j=0}^{b}\P(X_1+j\leq b )\P(X_2= j)\\
%         &=   \sum_{j=0}^{b}F_1(b-j)\P(X_2= j) \geq \sum_{j=0}^{b}\Psi_1(b - j)\P(X_2= j)\\
% % &=   \sum_{j=0}^{b}F_1(b-j)\P(X_2= j)
% % \\
%     & \geq \Psi_1(b)F_2(0) + \sum_{j=1}^{b}\Psi_1(b - j)(F_2(j)-F_2(j-1))
%     % \\
%     % &\geq \Psi_1(b)F_2(0) + \sum_{j=1}^{b}\Psi_1(b - j)(F_2(j)-F_2(j-1)) 
%     \label{eq:last}
% \end{align}
% \textbf{Step 2.2:} We use Abel's summation by parts in \eqref{eq:last} and obtain $\P(X_1+X_2\leq b) $
%  \begin{eqnarray}
%     % \P(X_1+X_2\leq b) 
%     &\geq&\Psi_1(b)F_2(0) + \sum_{j=1}^{b}\Psi_1(b - j)F_2(j)- \sum_{j=1}^{b}\Psi_1(b - j)F_2(j-1)
%     \\
%     &=&
%     \Psi_1(b)F_2(0) + \sum_{j=1}^{b}\Psi_1(b - j)F_2(j)- \sum_{j=0}^{b-1}\Psi_1(b - j - 1)F_2(j)
%     \\
%     &=&
%     \sum_{j=0}^{b}\Psi_1(b - j)F_2(j)- \sum_{j=0}^{b-1}\Psi_1(b - j - 1)F_2(j)
%     \\
%     &=&
%      \Psi_1(0)F_2(b) + \sum_{j=0}^{b-1}(\Psi_1(b - j) - \Psi_1(b - j- 1))F_2(j)\\
%     &=&
%     \psi_1(0)F_2(b) + \sum_{j=0}^{b-1}\psi_1(b - j)F_2(j) = \sum_{j=0}^{b}\psi_1(b - j)F_2(j)
%     \\
%     &=&
%      \sum_{j=0}^{b}\psi_1(b - j)F_2(j) \geq \sum_{j=0}^{b}\psi_1(b - j)\Psi_2(j)= \Psi_{1,2}(b)
% \end{eqnarray}
% Hence, \eqref{eq:conv} is shown.
% \textbf{Step 2 (Abel's summation):}  We use Abel's summation by parts in \eqref{eq:last} and obtain
%  \begin{eqnarray}
%     \P(X_1+X_2\geq b) 
%     &\leq&\sum_{j=0}^{b}\Phi_1(b - j)F_2(j)-\sum_{j=0}^{b}\Phi_1(b - j)F_2(j+1) + F_2(b+1)
%     \\
%     &=&
%     \sum_{j=0}^{b}\Phi_1(b - j)F_2(j)-\sum_{j=1}^{b+1}\Phi_1(b - j+1)F_2(j) + F_2(b+1)
%     \\
%     &=&
%     \sum_{j=0}^{b}\Phi_1(b - j)F_2(j)-\sum_{j=0}^{b} \Phi_1(b - j+1)F_2(j)+\Phi_1(b+1) - F_2(b+1) + F_2(b+1)
%     \\
%     &=&
%     \sum_{j=0}^{b}\Phi_1(b - j)F_2(j)-\sum_{j=0}^{b} \Phi_1(b - j+1)F_2(j)+\Phi_1(b+1)\\
%     &=&
%     \sum_{j=0}^{b}(\Phi_1(b - j)-\Phi_1(b - j+1))F_2(j)+\Phi_1(b+1)
%     \\
%     &=&
%     \sum_{j=0}^{b}\varphi_1(b - j)F_2(j)+\Phi_1(b+1)\isdef \Phi_{1,2}(b)
% \end{eqnarray}
% Hence, \eqref{eq:conv} is shown.

% \textbf{Step 2.3:} Observe that
%  \begin{eqnarray}
%     (\psi_1 * \Psi_2)(b)
%     &=&\sum_{j=0}^{b}\Psi_1(b - j)\Psi_2(j) - \sum_{j=1}^{b}\Psi_1(b - j)\Psi_2(j) 
%     \\
%     &=&
%     \sum_{i,j s.t. i + j = b, i,j \geq 0 }\Psi_1(i)\Psi_2(j)  +  \sum_{i,j s.t. i + j = b - 1, i,j \geq 0 }\Psi_1(i)\Psi_2(j) 
% \end{eqnarray}
% which is symmetric in indices 1,2 and thus shows that $\psi_1 * \Psi_2 = \Psi_1 * \psi_2$.
% \textbf{Final Step:} We now iteratively apply Step 2 and obtain $ \P\lp \sum_{i=1}^g \lceil B_i\rceil \leq b \rp \geq \Psi_{1,2,\ldots,g}(b)$ for $b\in \Nats$ with 
% \begin{equation} \label{eq:hs3}
%     \Psi_{1,2,\ldots,g}(b) = \lp\psi_1*\psi_2*\ldots*\psi_{g-1}*\Psi_{g} \rp(b), \;\;\; b>0,b\in \Nats
% \end{equation}
% Combine this with Step 1 to conclude that 
% \begin{equation} \label{eq:hs2}
%         \P(  B \leq b) \geq \Psi_{1,2,\ldots,g}(b), \;\;\; b>0,b\in \Nats
% \end{equation} 
% which concludes the theorem.
% % with $X_i = \lceil\sup_{t \geq 0}B_i(t) \rceil$, $\Psi_i$ and $\psi_i$, for $i=1:g$ as defined in the theorem. Observe that $X_i$ are independent and $X_i \in \Nats$, $\Psi_i$ is wide-sense increasing.
\end{proof}


% \subsection{Flows with Same Period but Different Packet-size} \label{sec:semi-homogen}
% Theorem~\ref{thm:hetero} can be applied to a heterogeneous set of flows as follows: Flows should be grouped in homogeneous sets, and   bounds on the tail probability of the  aggregate burstiness of each group (functions $\varepsilon_i$ for each group $i$) can be obtained by  our results for the homogeneous case in Section~\ref{sec:homogen}. Theorem~\ref{thm:hetero} then provides a convolution technique to combine these bounds and bound the tail probability of the aggregate burstiness of all flows; it can be efficiently computed using discrete convolution.
% applied as follows:
% \begin{enumerate}
%     \item Group flows such that flows in each group either the same period and packet size or have the same period but different packet size.
%     \item Compute the bounding function $\varepsilon$ as presented in Section~\ref{sec:homogen} and Section~\ref{sec:semi-homogen}, respectively, for each group.
%     \item Apply Theorem~\ref{thm:hetero} find a bounding function for the aggregate of all flows.
% \end{enumerate}
% The bound of Theorem~\ref{thm:hetero} is tight; specifically, $\varepsilon_{1,2,\ldots,g}$ is the best possible bounding function if the only information on different groups is their independence and the knowledge of their bounding functions  $\varepsilon_i$, for $i =1:g$. $\varepsilon_{1,2,\ldots,g}$.

% As explained after Proposition~\ref{prop:conv}, an alternative to Theorem~\ref{thm:hetero} is to  combine the bounds obtained for each group using union bound, which will be dominated by  our convolution bound.  We numerically observe that our convolution bound provides significantly better bounds than the union bound (see Fig.~\ref{fig:heter}a).

% Specifically, consider some $b$ and a collection $(b_1,b_2, \ldots, b_g)$ such that $\sum_{i=1}^gb_i = b$ and $b_i>0$; then, observe that $\bigcap_{i=1}^g\lc B_i \leq b_i \rc \Rightarrow \lc B \leq \sum_{i=1:g}b_i \rc$ and thus, by contraposition, $\lc B > b \rc \Rightarrow \bigcup_{i=1}^g\lc B_i > b_i \rc$. It follows that $\P\lp B > b\rp \leq \sum_{i=1}^g\P\lp B_i > b_i\rp \leq \sum_{i=1}^g \varepsilon_i(b_i)$.
% % we have $\P\lp B > b\rp \leq \sum_{i=1}^g\P\lp B_i > b_i\rp \leq \sum_{i=1}^g \varepsilon_i(b_i)$. 
% Thus, one can compute a collection $(b_1,b_2, \ldots, b_g)$ that minimizes the right-hand side. In all examples we tested, our convolution bound dominates the union bound (see Fig.~\ref{fig:heter}a).

% \hossein{Not to be part of the main paper, rather for discussion}
% We want to show that $\forall b \in \Nats$
% \begin{equation}
%     \underbrace{1 - (\psi_1 * \Psi_2) (b)}_{\varepsilon_{1,2}(b)} \leq \underbrace{(1 - \Psi_1(k))}_{\varepsilon_1(k)} + \underbrace{(1 - \Psi_2(b - k))}_{\varepsilon_2(b-k)}, ~ k=0:b
% \end{equation}
% i.e.,
% \begin{equation}\label{eq:induc}
%     \Psi_1(k) + \Psi_2(b - k) \leq 1 + (\psi_1 * \Psi_2)(b)  = 1 + \sum_{j=0:b} \psi_1(j)  * \Psi_2(b - j), ~ k=0:b
% \end{equation}

% We prove it by induction on $b$. When $b = 1$, for both $k = 0$ and $k = 1$, \eqref{eq:induc} is satisfied as $\Psi_1, \Psi_2 \leq 1$.
% Now assume that for \eqref{eq:induc} holds for $b$ and all $k \leq b$.  We want to show that =
% \begin{equation}\label{eq:toShow}
%     \Psi_1(k) + \Psi_2(b + 1 - k) \leq  1 + \sum_{j=0:(b+1)} \psi_1(j)  * \Psi_2(b + 1 - j), ~ k = 1:(b+1)
% \end{equation}

% First, as $\Psi_2(0) = \psi_1(0) = 0 $, when $k=b+1$ \eqref{eq:toShow} is satisfied. Second,  as $\Psi_2$ is wide-sense increasing and by the induction hypothesis in \eqref{eq:induc}:
% % the we lower bound the right-hand side of \eqref{eq:toShow}:
% \begin{align}
%      1 + \sum_{j=0:(b+1)} \psi_1(j)  * \Psi_2(b + 1 - j) &\geq  1 + \sum_{j=0:b} \psi_1(j)  * \Psi_2(b + 1 - j)\\
%      &\geq  1 + \sum_{j=0:b} \psi_1(j)  * \Psi_2(b  - j)\\
%      &\geq  \Psi_1(k') + \Psi_2(b  - k'),~ k'=0:b\\
%      &\geq  \Psi_1(k'-1) + \Psi_2(b  - k'),~ k'=1:b
% \end{align}
% replace $k'$ by $k -1$ in the last inequality to obtain
% \begin{align}
%      1 + \sum_{j=0:(b+1)} \psi_1(j) \Psi_2(b + 1 - j) \geq  \Psi_1(k) + \Psi_2(b +1 - k),~ k=0:(b-1)
% \end{align}
% which shows \eqref{eq:toShow} for $k=0:(b-1)$. We now need to show \eqref{eq:toShow} for $k = b$, i.e.,
% \begin{align}
%      1 + \sum_{j=0:(b+1)} \psi_1(j) \Psi_2(b + 1 - j) \geq  \Psi_1(b) + \Psi_2(1)
% \end{align}
% As $\psi_1* \Psi_2 = \psi_2* \Psi_1 $, swap indices above  and obtain
% \begin{align}
%      1 + \sum_{j=0:(b+1)} \psi_1(j) \Psi_2(b + 1 - j) \geq  \Psi_2(k) + \Psi_1(b +1 - k),~ k=0:(b-1)
% \end{align}
% where for $k=1$, the right hand side is $\Psi_2(k) + \Psi_1(b +1 - k)$ hence  \eqref{eq:toShow} is shown for $k = b$. Therefore, \eqref{eq:toShow} is shown.

% As $\Psi_2(0) = \psi_1(0) = 0 $ it simplifies to 
% \begin{equation}\label{eq:induc}
%     \Psi_1(k) + \Psi_2(b - k) \leq  1 + \sum_{j=1:(b-1)} \psi_1(j)  * \Psi_2(b - j)
% \end{equation}

% We prove it by induction on $b$ and another on $k\leq b$. When $b = 1$, for both $k = 0$ and $k = 1$, \eqref{eq:induc} is satisfied as $\Psi_1, \Psi_2 \leq 1$.

% Now assume that for \eqref{eq:induc} hold for $b$ and all $k \leq b$. We want to show that $\forall k \leq (b+1)$
% \begin{equation}\label{eq:induc}
%     \Psi_1(k) + \Psi_2(b - k) \leq  1 + \sum_{j=1:(b)} \psi_1(j)  * \Psi_2(b + 1 - j)
% \end{equation}
% The right-hand side can be upper bounded as follows as $\Psi_2$ is wide-sense increasing and $\psi_1$ and $\Psi_2$ are non-negative:
% \begin{align}
%      1 + \sum_{j=1:b} \psi_1(j)  * \Psi_2(b + 1 - j) &\geq 1 + \sum_{j=1:b} \psi_1(j)  * \Psi_2(b  - j) \\
%      &\geq 1 + \sum_{j=1:(b-1)} \psi_1(j)  * \Psi_2(b  - j) 
% \end{align}
% Then, combining it with the induction hypothesis, we have $\forall k \leq b$
% \begin{align}
%  1 + \sum_{j=1:b} \psi_1(j)  * \Psi_2(b + 1 - j) \geq \Psi_1(k) + \Psi_2(b - k) 
% \end{align}


% In fact, the bound of Theorem~\ref{thm:hetero}, $\varepsilon_{1,2,\ldots,g}$, is  the best possible bound we can obtain, if the only known information on different groups is their independence and their bounding functions  $\varepsilon_i$, for $i =1:g$.

% Observe that for a collection $(b_1,b_2, \ldots, b_g)$ such that $\sum_{i=1}^gb_i = b$ and $b_i>0$, we have $\P\lp B > b\rp \leq \sum_{i=1}^g\P\lp B_i > b_i\rp \leq \sum_{i=1}^g \varepsilon_i(b_i)$.

% can be efficiently computed using  properties of discrete convolution, namely, associativity and commutativity \cite{Oppenheim2010}.
For a specific case, when flows have the same period and different packet sizes, we provide an alternative bound that may be better, when the number of flows per packet size is small (see Fig.~\ref{fig:heter}b).  
% We provide an alternative approach for the specific case where flows have the same period but different Packet-sizes.
% We extend the results obtained in Section~\ref{sec:homogen}, thus unlike the convolution bound of Theorem~\ref{thm:hetero}, does not require grouping of flows.
\begin{theorem}[Flows with the same period but different packet-sizes] \label{thm:semi_homog}
Assume the assumptions of Section~\ref{sec:assump}, and also assume that flows have the same period. Let $l^{(1)} \geq l^{(2)} \geq \ldots \geq l^{(n)}$ be the ordered sequence of packet sizes, arranged in non-increasing order, and consider some $0 \leq b < \ltot$. Let $\eta \isdef \min_{k=1:n-1, \sum_{j=1}^{k+1}l^{(j)} > b}\lc  \frac{k}{n-1}-\frac{\sum_{j=1}^{k+1}l^{(j)}}{\ltot} \rc$.

\begin{enumerate}
    % $\P\lp \exists t \geq 0,~ B(t) > b\rp \leq n(1 - \bar{p}(n,l,b)) = \ep(n,l,b)$ with $\bar{p}(n,l,b)$ is computed as \eqref{eq:pbThm1} when replacing $u_1, u_2, \ldots,u_{n-1}$ by $\bar{u}_1, \bar{u}_2, \ldots,\bar{u}_{n-1}$ where $\bar{u}_k = \frac{[ \sum_{j=1}^{k+1}l_{(j)} - b]^+}{\ltot}, \forall k \in \{1, \ldots, n-1 \}$.

    \item A bound on the tail probability of the aggregate burstiness of all flows $B$ is given by
% \begin{equation}\label{eq:epsdkw}
%      \P\lp \exists t \geq 0,~ B(t) > b\rp \leq n \exp \lp -2(n-1) \lp \frac{\bar{k}}{n-1}-\frac{\Lcum(\bar{k}+1)-b}{\ltot} \rp^2 \rp  = \epdkw(n,l,b)
% \end{equation}
\begin{equation}
     \P\lp B > b\rp \leq n \exp \lp -2(n-1) \lp \eta +\frac{b}{\ltot} \rp^2 \rp
     % = \epdkw(n,l,b)
\end{equation}
% where $\bar{k} = \argmin_{k\in\lc 1,2,\ldots,n-1\rc, \sum_{j=1}^{k+1}l_{(j)} > b}{ \lc  \frac{k}{n-1}-\frac{\sum_{j=1}^{k+1}l_{(j)}}{\ltot} \rc}$.

\item Consider some $0 < \varepsilon <1$ and assume that $n \geq 2$; define 
\begin{equation}
    b(n,l^{(1)},\ldots ,l^{(n)}, \varepsilon) \isdef \ltot \lceil \sqrt{\frac{\log n - \log \varepsilon}{2(n-1)}}  - \eta  \rceil 
\end{equation}
Then, $b(n,l^{(1)},\ldots ,l^{(n)}, \varepsilon)$ is a quasi-deterministic burstiness bound for the aggregate with the violation probability of at most $\varepsilon$, i.e., $\P\lp B > b(n,l^{(1)},\ldots ,l^{(n)}, \varepsilon)\rp \leq \varepsilon$.

\item Compute $\bar{p}(n,l^{(1)},\ldots ,l^{(n)},b)$ as \eqref{eq:pbThm1} by replacing $u_1, u_2, \ldots,u_{n-1}$ by $\bar{u}_1, \bar{u}_2, \ldots,\bar{u}_{n-1}$ where $\bar{u}_k = \frac{[ \sum_{j=1}^{k+1}l^{(j)} - b]^+}{\ltot},~ k =1:n-1$. Then, a bound on the tail probability of the aggregate burstiness of all groups $B$ is given by
    \begin{equation}
        \P\lp B > b\rp \leq n(1 - \bar{p}(n,l^{(1)},\ldots ,l^{(n)},b)) 
        % = \epe(n,\Vec{l},b)
        % = \ep(n,l,b)
    \end{equation}
\end{enumerate}
% \textbf{Item 1):} $\P\lp \exists t \geq 0,~ B(t) > b\rp \leq n(1 - \bar{p}(n,l,b)) = \ep(n,l,b)$
% % \begin{equation} \label{eq:epsThm1}
% %      \P\lp \exists t \geq 0,~ B(t) > b\rp \leq n(1 - \bar{p}(n,l,b)) = \ep(n,l,b) 
% % \end{equation}
% with $\bar{p}(n,l,b)$ is computed as \eqref{eq:pbThm1} when replacing $u_1, u_2, \ldots,u_{n-1}$ by $\bar{u}_1, \bar{u}_2, \ldots,\bar{u}_{n-1}$ where $\bar{u}_k = \frac{[ \sum_{j=1}^{k+1}l_{(j)} - b]^+}{\ltot}, \forall k \in \{1, \ldots, n-1 \}$.
% % \begin{align}
% %     % \label{eq:pbThm1}
% %     % p(n,l,b) & = (n-1)!\int_{y_{n-1} = u_{n-1}}^{1} \int_{y_{n-2} = u_{n-2}}^{y_{n-1}} \ldots \int_{y_{i} = u_{i}}^{y_{i+1}} \ldots \int_{y_{1} = u_{1}}^{y_{2}} 1   \,dy_1 \ldots \,dy_{n-1} \\
% %     \label{eq:ukThm3}
% %     % p(b) & = (n-1)!\int_{y_{n-1} = u_{n-1}}^{1} \int_{y_{n-2} = u_{n-2}}^{y_{n-1}} \ldots \int_{y_{i} = u_{k}}^{y_{k+1}} \ldots \int_{y_{1} = u_{1}}^{y_{2}}    \,dy_1 \ldots \,dy_{n-1}
% %      \bar{u}_k &= \frac{[ \sum_{j=1}^{k+1}l_{(j)} - b]^+}{\ltot}, \forall k \in \{1, \ldots, n-1 \}
% % \end{align}
% % $B(t)$ is defined in \eqref{eq:agg_burst}, and in \eqref{eq:ukThm1}, we use the notation $[x]^+=\max\{x,0\}$ and $\ltot = nl$.

% \textbf{Item 2):} If $b \geq \ltot \lp \sqrt{\frac{\log 2}{2(n-1)}}  - \frac{\bar{k}}{n-1} + \frac{\sum_{j=1}^{\bar{k}+1}l_{(j)}}{\ltot}  \rp$, then, 
% % \begin{equation}\label{eq:epsdkw}
% %      \P\lp \exists t \geq 0,~ B(t) > b\rp \leq n \exp \lp -2(n-1) \lp \frac{\bar{k}}{n-1}-\frac{\Lcum(\bar{k}+1)-b}{\ltot} \rp^2 \rp  = \epdkw(n,l,b)
% % \end{equation}
% \begin{equation}\label{eq:epsdkw}
%      \P\lp \exists t \geq 0,~ B(t) > b\rp \leq n \exp \lp -2(n-1) \lp \frac{\bar{k}}{n-1}-\frac{\sum_{j=1}^{k+1}l_{(j)}-b}{\ltot} \rp^2 \rp  = \epdkw(n,l,b)
% \end{equation}
% where $\bar{k} = \argmin_{k\in\lc 1,2,\ldots,n-1\rc, \sum_{j=1}^{k+1}l_{(j)} > b}{ \lc  \frac{k}{n-1}-\frac{\sum_{j=1}^{k+1}l_{(j)}}{\ltot} \rc}$.
% % \begin{align}
% %     \label{eq:kbar}
% %     \bar{k} = \argmin_{k\in\lc 1,2,\ldots,n-1\rc, \sum_{j=1}^{k+1}l_{(j)} > b}{ \lc  \frac{k}{n-1}-\frac{\sum_{j=1}^{k+1}l_{(j)}}{\ltot} \rc}
% %     % k^* &= \min_{ k \in \lc 1,2,\ldots, n-1\rc}\lc  \sum_{j=1}^{\bar{k}+1}l_{(j)} > b \rc
% % \end{align}

% \textbf{Item 3):} Consider some $\varepsilon > 0$, and compute $b(n,l, \varepsilon)$ as follow:
% \begin{equation}
%     b(n,l, \varepsilon) = \ltot \lp \sqrt{\frac{\log n - \log \varepsilon}{2(n-1)}}  - \frac{\bar{k}}{n-1} + \frac{\sum_{j=1}^{\bar{k}+1}l_{(j)}}{\ltot}  \rp 
% \end{equation}
% where $\bar{k}$ is defined in Item 2). Then, $b(n,l, \varepsilon)$ is a quasi-deterministic burstiness bound for the aggregate with the violation probability of at most $\varepsilon$, i.e., $\P\lp \exists t \geq 0,~ B(t) > b(n,l, \varepsilon)\rp \leq \varepsilon$.
\end{theorem}



% \begin{theorem}[Flows with Same Period but Different Packet-size] \label{thm:semi_homog}
% Assume the assumptions of Section~\ref{sec:assump}, and also assume that flows have the same period, i.e., for every flow $f$, $\tau_f = \tau$ for some $\tau > 0$. Let $l_{(1)} \geq l_{(2)} \geq \ldots \geq l_{(n)}$ be the ordered sequence of packet-sizes and consider some $b$. Then,
% Item 1):
% \begin{equation} \label{eq:epsThm1}
%      \P\lp \exists t \geq 0,~ B(t) > b\rp \leq n(1 - \bar{p}(n,l,b)) = \ep(n,l,b) 
% \end{equation}
% with $\bar{p}(n,l,b)$ is computed as \eqref{eq:pbThm1} when replacing $u_1, u_2, \ldots,u_{n-1}$ by $\bar{u}_1, \bar{u}_2, \ldots,\bar{u}_{n-1}$ where
% \begin{align}
%     % \label{eq:pbThm1}
%     % p(n,l,b) & = (n-1)!\int_{y_{n-1} = u_{n-1}}^{1} \int_{y_{n-2} = u_{n-2}}^{y_{n-1}} \ldots \int_{y_{i} = u_{i}}^{y_{i+1}} \ldots \int_{y_{1} = u_{1}}^{y_{2}} 1   \,dy_1 \ldots \,dy_{n-1} \\
%     \label{eq:ukThm3}
%     % p(b) & = (n-1)!\int_{y_{n-1} = u_{n-1}}^{1} \int_{y_{n-2} = u_{n-2}}^{y_{n-1}} \ldots \int_{y_{i} = u_{k}}^{y_{k+1}} \ldots \int_{y_{1} = u_{1}}^{y_{2}}    \,dy_1 \ldots \,dy_{n-1}
%      \bar{u}_k &= \frac{[ \sum_{j=1}^{k+1}l_{(j)} - b]^+}{\ltot}, \forall k \in \{1, \ldots, n-1 \}
% \end{align}
% % $B(t)$ is defined in \eqref{eq:agg_burst}, and in \eqref{eq:ukThm1}, we use the notation $[x]^+=\max\{x,0\}$ and $\ltot = nl$.


% \end{theorem}

% \begin{theorem}[Closed-Form, DKW Bound] \label{thm:semi_homog_dkw}
% Assume the assumptions of Theorem~\ref{thm:semi_homog}. Also, consider some $b$ such that $b \geq \ltot \lp \sqrt{\frac{\log 2}{2(n-1)}}  - \frac{\bar{k}}{n-1} + \frac{\sum_{j=1}^{\bar{k}+1}l_{(j)}}{\ltot}  \rp$. Then, 
% % \begin{equation}\label{eq:epsdkw}
% %      \P\lp \exists t \geq 0,~ B(t) > b\rp \leq n \exp \lp -2(n-1) \lp \frac{\bar{k}}{n-1}-\frac{\Lcum(\bar{k}+1)-b}{\ltot} \rp^2 \rp  = \epdkw(n,l,b)
% % \end{equation}
% \begin{equation}\label{eq:epsdkw}
%      \P\lp \exists t \geq 0,~ B(t) > b\rp \leq n \exp \lp -2(n-1) \lp \frac{\bar{k}}{n-1}-\frac{\sum_{j=1}^{k+1}l_{(j)}-b}{\ltot} \rp^2 \rp  = \epdkw(n,l,b)
% \end{equation}
% where
% \begin{align}
%     \label{eq:kbar}
%     \bar{k} = \argmin_{k\in\lc 1,2,\ldots,n-1\rc, \sum_{j=1}^{k+1}l_{(j)} > b}{ \lc  \frac{k}{n-1}-\frac{\sum_{j=1}^{k+1}l_{(j)}}{\ltot} \rc}
%     % k^* &= \min_{ k \in \lc 1,2,\ldots, n-1\rc}\lc  \sum_{j=1}^{\bar{k}+1}l_{(j)} > b \rc
% \end{align}
% % \begin{align}
% %     \label{eq:kbar}
% %     \bar{k} = \argmin_{k\in\lc k^*,...,n-1\rc}{ \lc  \frac{k}{n-1}-\frac{\sum_{j=1}^{\bar{k}+1}l_{(j)}}{\ltot} \rc } \mand k^* = \min_{ k \in \lc 1,2,\ldots, n-1\rc}\lc  \sum_{j=1}^{\bar{k}+1}l_{(j)} > b \rc
% %     % k^* &= \min_{ k \in \lc 1,2,\ldots, n-1\rc}\lc  \sum_{j=1}^{\bar{k}+1}l_{(j)} > b \rc
% % \end{align}
% Also,  $\epdkw(n,l,b) \geq \ep(n,l,b)$ where $\ep(n,l,b)$ is the bound of Theorem~\ref{thm:homog}.
% \end{theorem}

% \begin{corollary}[Estimated Quasi-Deterministic Burstiness in Closed-form] \label{cor:semi_homog_burst}
% Assume the assumptions of Theorem~\ref{thm:semi_homog}. Consider some $\varepsilon > 0$, and compute $b(n,l, \varepsilon)$ as follow:
% \begin{equation}
%     b(n,l, \varepsilon) = \ltot \lp \sqrt{\frac{\log n - \log \varepsilon}{2(n-1)}}  - \frac{\bar{k}}{n-1} + \frac{\sum_{j=1}^{\bar{k}+1}l_{(j)}}{\ltot}  \rp 
% \end{equation}
% where $bar{k}$ is defined in \eqref{eq:kbar}. Then, $b(n,l, \varepsilon)$ is a quasi-deterministic burstiness bound for the aggregate with the violation probability of at most $\varepsilon$, i.e., $\P\lp \exists t \geq 0,~ B(t) > b(n,l, \varepsilon)\rp \leq \varepsilon$.
% % \begin{equation}
% %      \P\lp \exists t \geq 0,~ B(t) > b_F^\epsilon\rp \leq \epsilon
% % \end{equation}
% \end{corollary}

 % Theorem~\ref{thm:semi_homog} is the extension of the results presented in Theorem~\ref{thm:homog}, Theorem~\ref{thm:homog_dkw}, and Corollary~\ref{cor:homog_burst} when flows different packet-sizes; Indeed,  
 When all flows have the same packet-sizes $l$ and $b \in \Nats$, Theorem~\ref{thm:semi_homog} provides exactly the same bounds as  provided in Theorem~\ref{thm:homog_dkw}, Corollary~\ref{cor:homog_burst}, and Theorem~\ref{thm:homog}
 of Section~\ref{sec:homogen}. Also, Algorithm~\ref{alg:thm1} can be used to compute the bound of item 3) with the following changes: First, at line $1$, replace the value of $m \gets \argmax_{ k=1:n-1}{ \sum_{j=1}^{k+1}l^{(j)} \leq b}$. Second, at line $4$, replace $u_k$ by $\bar{u}_k$.
 
 \begin{proof}
 The proof follows similar steps as in the proof of Theorems~\ref{thm:homog_dkw}~and~\ref{thm:homog} with the following change in Proposition~\ref{prop:main}: We replace the definition of $H_{i,j}$ in \eqref{eq:Hij}  with $H_{i,j} = \sum_{k=1}^{j - i +1}l^{(k)}  - \ltot(T_j - T_i)$. This is obtained by upper bonding $ A(T_i, T_j]$ by $\sum_{k=1}^{j - i +1}l^{(k)}$, as in the time interval $(T_i, T_j]$, $(j-i + 1)$ packets have arrived in the aggregate traffic.
 %   % because in Step 1) of the proof of Lemma~\ref{lem:main} we use the fact that in the time interval $(T_i, T_j]$, $(j-i + 1)$ packets have arrived in the aggregate traffic, and thus $A(T_i, T_j]$ can be upper bounded $\sum_{k=1}^{j - i +1}l_{(k)}$ and the rest of the proof follows the same steps.
 % Event $E$ becomes $ E = \bigcup_{k=\bar{k}}^{n-1} 
 %   \lc U_{(k)} < \frac{\sum_{j=1}^{k+1}l^{(j)}-b}{\ltot}\rc$. This is obtained by upper bpnding $ A(T_i, T_j]$ by $\sum_{k=1}^{j - i +1}l^{(k)}$, as in the time interval $(T_i, T_j]$, $(j-i + 1)$ packets have arrived in the aggregate traffic; then it follows that
 %   % because in Step 1) of the proof of Lemma~\ref{lem:main} we use the fact that in the time interval $(T_i, T_j]$, $(j-i + 1)$ packets have arrived in the aggregate traffic, and thus $A(T_i, T_j]$ can be upper bounded $\sum_{k=1}^{j - i +1}l_{(k)}$;
 %   we replace $H_{i,j}$ in \eqref{eq:Hij}  with $\bar{H}_{i,j} = \sum_{k=1}^{j - i +1}l_{(k)}  - \ltot(T_j - T_i)$, and the rest of the proof follows the same steps.
   % of size $l$ have arrived in the aggregate traffic, and hence $A(T_i, T_j] = (j - i + 1)l$. However, when packets are of different sizes, while  in the time interval, $(T_i, T_j]$  $(j-i + 1)$ packets have arrived, we do not know their sizes. However, we can upper bound $A(T_i, T_j]$ by assuming the worst-case packet arrivals, i.e., in the decreasing order of the sizes; specifically, we replace $H_{i,j}$ in \eqref{eq:Hij}  with $\bar{H}_{i,j} = \sum_{k=1}^{j - i +1}l_{(k)}  - \ltot(T_j - T_i)$. Hence, event $E$ becomes $ E = \bigcup_{k=\bar{k}}^{n-1} 
   % \lc U_{(k)} < \frac{\sum_{j=1}^{k+1}l_{(j)}-b}{\ltot}\rc$. 
   \qed
 \end{proof}

 
% \textbf{Step 3:} We now apply Step 2, \eqref{eq:conv}, with $\Psi_i$ and $\psi_i$ as defined in the theorem.

% The bound can be applied iteratively to the sum of $n$ independent random variables. 

==> homogeneous.tex <==
% \section{Homogeneous Flows: Same Period and Same Packet-size} 
\section{Homogeneous Case} \label{sec:homogen}
% \section{Homogeneous Case: Flows with the Same Period and Same Packet-size} \label{sec:homogen}


In this section, we consider the case where flows have  the same packet size and same period. We present two theorems; the former gives a closed form, unlike the latter, which might be slightly more accurate when the number of flows is small.  Both theorems are derived from  Proposition~\ref{prop:main}, the proof of which uses Lemma~\ref{lem:uniform}, which we present next.

% Recall that the aggregate burstiness $B$ satisfies $B \leq \ltot$ as $\ltot$ is a deterministic bound on the aggregate burstiness (see Section~\ref{sec:assump_prob}); hence, for any $b \geq \ltot$, we have $\P (B > \ltot) = 0$.  

% which serves as the basis for the results we obtain in this section.
% : We derive our main result, Theorem~\ref{thm:homog_dkw}, by following Lemma~\ref{lem:main} and using Dvoretzky–Kiefer–Wolfowitz (DKW) inequality.  Our second result, Theorem~\ref{thm:homog}, follows Lemma~\ref{lem:main} and uses order statistics  to bound the tail probability of the aggregate burstiness. 
% When the number of flows is small, Theorem~\ref{thm:homog} provides a better bound than Theorem~\ref{thm:homog_dkw},  but when the number of flows is large, the bound of Theorem~\ref{thm:homog_dkw} is as tight. 

% Our first and main result, Theorem~\ref{thm:homog_dkw}, follows Lemma~\ref{lem:main} and uses Dvoretzky–Kiefer–Wolfowitz (DKW) inequality to obtain a closed-form expression to bound the tail probability of the aggregate burstiness. Our second result, Theorem~\ref{thm:homog}, follows Lemma~\ref{lem:main} and uses order statistics  to bound the tail probability of the aggregate burstiness. When the number of flows is small, Theorem~\ref{thm:homog} provides a better bound than Theorem~\ref{thm:homog_dkw},  but when the number of flows is large, the bound of Theorem~\ref{thm:homog_dkw} is as tight. 

\begin{lemma}\label{lem:uniform}
        Let $U_1, ..., U_{n}$ be a sequence of $n$ independent and identically distributed (iid) standard uniform random variables, and $U_{(1)} \leq U_{(2)} \leq ,..., \leq U_{(n)}$ be the corresponding order statistic, arranged in non-decreasing order.
        Consider some integer $i \leq n$ and  
        define $W_j$ for $j=1:(n-1)$ by
        \begin{equation}
            W_j = \begin{cases}
                     U_{(j+i)} - U_{(i)} &\text{for } j=1:(n-i)\\
                     1 + U_{(j - n + i)} - U_{(i)} &\text{for } j=(n-i+1):(n-1)
                \end{cases}
        \end{equation}        
        % as follow: $j=1:(n-i),~ W_j = U_{(j+i)} - U_{(i)}$ and $ j=(n-i+1):(n-1),~ W_j = 1 + U_{(j - (n-i))} - U_{(i)}$. 
        Then, the joint distribution of $W_1, \ldots,W_{n-1}$ is the same as the joint distribution of $U_{(1)},...,U_{(n-1)}$.
    \end{lemma}
    \begin{proof}
    The lemma is equivalent to proving that for any collection of  bounded, measurable functions $g_1, g_2, \ldots,g_{n-1}$,
    \begin{equation} \label{eq:orderUniform1}
        \E\lp g_1(W_1)\ldots g_{n-1}((W_{n-1}) \rp = \E\lp g_1(U_{(1)})\ldots g_{n-1}((U_{(n-1)}) \rp
    \end{equation}
    Note that the density function of the joint distribution of $U_{(1)},...,U_{(n-1)}$ is \cite{gentle2009computational}
    % \cite[Equation 1.145]{gentle2009computational}
        \begin{equation}\label{eq:orderUniform}
       f_{U_{(1)},...,U_{(n-1)}}\lp y_{1},...,y_{n-1} \rp  = (n-1)!\ind{0 \leq y_{1}\leq y_2 \leq  \ldots \leq y_{n-1} \leq 1}
    \end{equation}
    % \begin{equation}
    %     f_{U_{(1)},...,U_{(n-1)}}\lp y_{1},...,y_{n-1} \rp  = (n-1)!\prod_{k=1}^{n-1}f_{U}(y_{k})\ind{y_{1}\leq y_2 \leq  \ldots \leq y_{n-1}}
    % \end{equation}
    % where $f_U$ is the probability density function of a standard uniform; as $y_{k} \in [0,1]$, $f_{U}(y_{k}) = 1$ for $k = 1:n-1$
    % % $k \in \{1,\ldots,n-1\}$
    % . Hence,
    % \begin{equation}\label{eq:orderUniform}
    %    f_{U_{(1)},...,U_{(n-1)}}\lp y_{1},...,y_{n-1} \rp  = (n-1)!\ind{y_{1}\leq y_2 \leq  \ldots \leq y_{n-1}}
    % \end{equation}
    Thus,  \eqref{eq:orderUniform1} becomes
    % , $ E\lp g_1(W_1),\ldots,g_{n-1}((W_{n-1}) \rp =$
    % \footnotesize  $ \E\lp g_1(W_1),\ldots,g_{n-1}((W_{n-1}) \rp = $
    {\footnotesize
    \begin{equation} \label{eq:lemU}
         \E\lp g_1(W_1)\ldots g_{n-1}((W_{n-1}) \rp = (n-1)!\int_{0 \leq y_1  \leq \ldots \leq y_{n-1} \leq 1}g_1(y_1) \ldots g_{n-1}(y_{n-1})  \,dy_1 \ldots \,dy_{n-1} 
    \end{equation}}
    We now proceed to show \eqref{eq:lemU}. Observe that  {\footnotesize$ E\lp g_1(W_1),\ldots,g_{n-1}((W_{n-1}) \rp =$
    % \begin{equation}
    %   E\lp g_1(U_{(i+1)} - U_{(i)}),\ldots,g_{n-i}(U_{(n)} - U_{(i)}), g_{n-i+1}(1 + U_{(1)} - U_{(i)}), \ldots, g_{n-1}(1 + U_{(i-1)} - U_{(i)}) \rp 
    % \end{equation}
    \begin{align} 
        &\E\lp g_1(U_{(i+1)} - U_{(i)})\ldots g_{n-i}(U_{(n)} - U_{(i)}) g_{n-i+1}(1 + U_{(1)} - U_{(i)}) \ldots g_{n-1}(1 + U_{(i-1)} - U_{(i)}) \rp \nonumber\\
        & =\int_{u_i=0}^1((n-1)!\int_{0 \leq u_1 \leq \ldots\leq u_{n} \leq 1} g_1(u_{i+1} - u_i)\ldots g_{n-i}(u_{n} - u_i) g_{n-i+1}(1 + u_{1} - u_i)\nonumber\\
        &\quad  \quad \quad \quad \quad  \ldots g_{n-1}(1 + u_{i-1} - u_i)du_1 \ldots du_{i-1} du_{i+1} \ldots du_{n}) du_i
        % =(n-1)!\int_{0 \leq y_1 \leq \ldots \leq y_{n-1} \leq 1} g_1(y_1), \ldots,\nonumber \\
        % &\quad  \quad \quad \quad \quad g_{n-i}(y_{n-i}) \\
        % &=(n-1)!\int_{0 \leq y_1 \leq \ldots \leq y_{n-1} \leq 1} g_1(y_1),\ldots,g_{n-i}(y_{n-i}),g_{n-i+1}(y_{n-i+1}), \ldots, g_{n-1}(y_{n-1})dy_1,\ldots,dy_{n-1}
    \end{align}
    }
    We change variables $u_1,\ldots,u_{i-1},u_{i+1},\ldots u_{n-1}$ with $ y_1 , y_2,\ldots,y_{n-1} $ where for $j=1:(n-i)$, $y_j =  u_{j+i} - u_i$ and  for $j=(n-i+1):(n-1)$, $1 + u_{j - n + i} - u_i$.  Observe the followings: First, $y_1 = u_{i+1} - u_{i} \geq 0$. Second, for $j = 1:(n-i-1)$,  $y_{j+1} = u_{j+i + 1} - u_{i}  \geq u_{j+i} - u_{i} = y_{j}$. Third, $y_{n-i+1} = 1 + u_{1} - u_{i}  \geq u_{n} - u_{i} = y_{n-i}$. Lastly, $y_{n-1} \leq 1 $. Hence, we have $0 \leq y_1 \leq \ldots \leq y_{n-1} \leq 1$. Also, observe that $dy_1=du_1,\ldots,dy_{i-1}=du_{i-1},dy_i = du_{i+1},\ldots dy_{n-1} = du_{n}$. Thus, $ \E\lp g_1(W_1),\ldots,g_{n-1}((W_{n-1}) \rp =${\footnotesize 
        \begin{align}
        & =\int_{u_i=0}^1 \lp (n-1)!\int_{0 \leq y_1 \leq \ldots\leq y_{n-1} \leq 1} g_1(y_1)g_2(y_2)\ldots g_{n-1}(y_{n-1})dy_1\ldots y_{n-1} \rp du_i\\
        & =(n-1)!\int_{0 \leq y_1 \leq \ldots\leq y_{n-1} \leq 1} g_1(y_1)g_2(y_2)\ldots g_{n-1}(y_{n-1})dy_1\ldots y_{n-1} 
        % =(n-1)!\int_{0 \leq y_1 \leq \ldots \leq y_{n-1} \leq 1} g_1(y_1), \ldots,\nonumber \\
        % &\quad  \quad \quad \quad \quad g_{n-i}(y_{n-i}) \\
        % &=(n-1)!\int_{0 \leq y_1 \leq \ldots \leq y_{n-1} \leq 1} g_1(y_1),\ldots,g_{n-i}(y_{n-i}),g_{n-i+1}(y_{n-i+1}), \ldots, g_{n-1}(y_{n-1})dy_1,\ldots,dy_{n-1}
    \end{align}}
    which shows \eqref{eq:lemU}, and therefore the lemma is concluded. \qed
\end{proof}

Recall that the aggregate burstiness $B$ satisfies $B \leq \ltot$ as $\ltot$ is a deterministic bound on the aggregate burstiness (see Section~\ref{sec:assump_prob}); hence, for any $b \geq \ltot$, we have $\P (B > \ltot) = 0$.  
\begin{proposition}\label{prop:main}
Assume the assumptions of Section~\ref{sec:assump}, and also assume that flows have the same period and same packet size, i.e., for every flow $f = 1:n$, $\tau_f = \tau$ and $l_f = l$ for some $l, \tau > 0$. Consider some $0 \leq b < \ltot = nl$. Let $U_1, ..., U_{n-1}$ be a sequence of $n-1$ independent and identically distributed (iid) standard uniform random variables, and $U_{(1)},...,U_{(n-1)}$ be the corresponding order statistic, arranged in non-decreasing order. Then,
    \begin{align} \label{eq:BiT}
        % \forall i \in \{1,\ldots,n\}, 
        \P \lp B > b\rp \leq n\P\lp E \rp 
        % \lc B_i \leq b \rc = \bigcap_{k = 1}^{n-1} \lc U_{(k)} \geq \frac{ \lb (k + 1)l - b \rb^+}{\ltot} \rc, \;\;\; i = 1:n
    \end{align}
    with
    \begin{equation}
    E \isdef \bigcup_{k=\lfloor\frac{b}{l}\rfloor}^{n-1} 
   \lc U_{(k)} < \frac{(k+1)l-b}{\ltot}\rc
   % E = \bigcup_{k=\lfloor \bar{b}\rfloor}^{n-1} 
   % \lc U_{(k)} < \frac{(k+1)l-b}{\ltot}\rc
   % = \bigcup_{k=\lfloor b\rfloor}^{n-1} 
   % \lc U_{(k)} < \frac{(k+1)-\Bar{b}}{n}\rc 
\end{equation}
\end{proposition}
 % Lemma~\ref{lem:main} provides a preliminary to obtain the bound of interest: It introduces  the event $E$ such that an upper bound of $\P(E)$ is an upper bound on the tail probability of the aggregate burstiness. 
 % . Specifically, it provides the event $E$ such that upper-bounding $\P(E)$ gives an upper bound on the tail probability of the aggregate burstiness. 
 % As we show in the following theorems, bounds
 % , which is easier to solve, and its solution applies to the problem of interest. Specifically, it provides the event $E$ such that upper-bounding $\P(E)$ gives an upper bound on the tail probability of the aggregate burstiness. 
 % In Theorem~\ref{thm:homog_dkw}, we provide a closed-form expression that upper-bounds $\P(E)$ using DKW inequality and  is tight when the number of flows $n$ is large. In Theorem~\ref{thm:homog}, we use order statistics and exactly compute $\P(E)$, thus providing bounds less than or equal to that of Theorem~\ref{thm:homog_dkw}. However, it is  of interest when the number of flows is small, as Theorem~\ref{thm:homog_dkw} is easier to compute and is as tight when the number of flows is large.
 
 % but it comes with computation complexity, and hence is of interest when the number of flows is small.
 % In our main result, Theorem~\ref{thm:homog_dkw}, we provide a closed-form expression that upper-bounds $\P(E)$ using DKW inequality; this bound is as tight as that of Theorem~\ref{thm:homog}, when the number of flows is large. 


\begin{proof}
   Take the period $\tau$ as time unit so that $\tau = 1$ and $\rtot = \ltot$.
   % in the rest of the proof.
    % Without loss of generality, we assume that period $\tau = 1$, hence $\rtot = \ltot$ in the rest of the proof:
    Let $T_j,~ j\geq 1$ be the arrival time of the $j$-th packet in the aggregate. 
    % We show the following equation:
    %  \begin{equation} \label{eq:s2}
    %     B  = \max_{i=1:n}  B_i
    % \end{equation}
    %     with 
    % \begin{align}
    % \label{eq:bi}
    %      % \forall i \in \{1,\ldots,n\}, ~ 
    %      B_i &\isdef \max_{j = i:(i+n-1)} H_{i,j}, \;\;\; i = 1:n\\
    %      \label{eq:Hij}
    %     \forall j \geq i, H_{i,j} &\isdef (j - i + 1)l - \ltot(T_j - T_i)
    % \end{align}
    %     \forall i \in \{1,2,\ldots, n\}, ~ B_i = \max_{j = i:(i+n-1)} \lc (j - i + 1)l - \ltot(T_j - T_i) \rc
    %     \forall j \geq i, H_{i,j} = (j - i + 1)l - \ltot(T_j - T_i)
    % \end{equation}
    % We now prove Step 1: 
    As $\forall s \leq t, A(s, t]$ is constant between the arrival times of packets, observe that $B$ and $\bar{B}(t)$, defined in \eqref{eq:agg_burst} and \eqref{eq:agg_burst_t}, can be rewritten as 
    $B = \max_{1 \leq j}\bar{B}(T_j)$ and $\bar{B}(T_j) = \max_{i=1:j} \lc A(T_i, T_j] - \ltot(T_j - T_i) \rc$. Also,  observe that $A(T_i, T_j] = (j - i + 1)l$ and thus $\bar{B}(T_j)$ can be rewritten $\bar{B}(T_j)= \max_{i=1:j} H_{i,j}$ with $H_{i,j}   = \max_{i=1:j} \lc (j - i + 1)l - \ltot(T_j - T_i) \rc,~ j\leq i$; combine this with $B = \max_{1 \leq j}\bar{B}(T_j)$ and obtain 
      \begin{equation} \label{eq:s1}
        B = \max_{1 \leq j} \max_{i=1:j } H_{i,j} 
    \end{equation}
    As the period of every flow is equal to $1$, we have $T_{j + n} = T_j + 1$ for $j\geq 1$; also, recall that $\ltot = nl$. Then, it follows that $H_{i,j+n} = H_{i,j}$ for $i\leq j$ and $H_{i+n,j} = H_{i,j}$ if $i + n\leq j$. Combine this with \eqref{eq:s1} and obtain
    \begin{equation} \label{eq:p1s1}
       B =  \max_{1 \leq j} \max_{i=1:j } H_{i,j} =  \max_{i=1:n} \underbrace{\max_{j = i:(i+n-1)} H_{i,j}}_{B_i}
    \end{equation}
    % which concludes Step 1.
    % As flows are packetized, points of interest are the arrival times of packets, and thus $\max_{t\geq 0}B(t) = \max_{1 \leq j}B(T_j)$ and $B(T_j) = \max_{i=1:j} \lc A(T_i, T_j] - \ltot(T_j - T_i) \rc$. Also, observe that $A(T_i, T_j] = (j - i + 1)l$ as in time interval $(T_i, T_j]$, $(j-i + 1)$ packets of size $l$ have arrived for the aggregate traffic. Hence
    % \begin{equation} \label{eq:s1}
    %     B = \max_{1 \leq j} \max_{i=1:j } H_{i,j} 
    % \end{equation}
    % As flows are periodic with a period equal to $1$, we have $T_{j + n} = T_j + 1$ for $j\geq 1$; also, recall that $\ltot = nl$. Then, it follows that $H_{i,j+n} = H_{i,j}$ for $i\leq j$ and $H_{i+n,j} = H_{i,j}$ if $i + n\leq j$. Hence,
    % \begin{equation}
    %     \underbrace{\max_{1 \leq j} \max_{i=1:j } H_{i,j}}_{B} =  \max_{i=1:n} \underbrace{\max_{j = i:(i+n-1)} H_{i,j}}_{B_i}
    % \end{equation}
    % which concludes \eqref{eq:s2}.
    
    % Let $U_1, ..., U_{n-1}$ be a sequence of $n-1$ independent and identically distributed (iid) standard uniform random variables, and $U_{(1)},...,U_{(n-1)}$ be the corresponding order statistic. 
    We now prove the following:
    \begin{align} \label{eq:BiT}
        % \forall i \in \{1,\ldots,n\}, 
         \P \lp B_i > b \rp  = \P(E), \;\;\; i = 1:n
    \end{align}
    % \begin{align} \label{eq:BiT}
    %     % \forall i \in \{1,\ldots,n\}, 
    %     \lc B_i \leq b \rc = \bigcap_{k = 1}^{n-1} \lc U_{(k)} \geq \frac{ \lb (k + 1)l - b \rb^+}{\ltot} \rc, \;\;\; i = 1:n
    % \end{align}
     Fix $i \leq n$. Observe that $\lc B_i > b \rc = \bigcup_{j = i}^{i + n -1} \lc (T_j - T_i) < \frac{(j - i + 1)l - b}{\ltot} \rc$.
     % $\lc B_i > b \rc $ can be rewritten as follows: 
    %   \begin{align} \label{eq:s21}
    %     \lc B_i > b \rc = \bigcup_{j = i}^{i + n -1} \lc (T_j - T_i) < \frac{(j - i + 1)l - b}{\ltot} \rc
    % \end{align}
     Let us denote $\phi_{(1)} \leq \phi_{(2)} \leq \ldots \leq \phi_{(n)}$ the ordered sequence of phases. As $i \leq n$, it follows that $T_i = \phi_{(i)}$. Second, observe that $\forall j=(i+1):(i+n-1)$, $T_j - T_i = T_j - \phi_{(i)} = \lp \phi_{(j)} - \phi_{(i)}\rp 1_{ j \leq n } +   \lp 1 + \phi_{(j - n)} - \phi_{(i)}\rp 1_{ j > n } $
    % \begin{equation} \label{eq:T}
    %     T_j - T_i = T_j - \phi_{(i)} = \lp \phi_{(j)} - \phi_{(i)}\rp 1_{ j \leq n } +   \lp 1 + \phi_{(j - n)} - \phi_{(i)}\rp 1_{ j > n } 
    % \end{equation}
    Apply Lemma~\ref{lem:uniform} to $\phi_1,\ldots,\phi_n$; it follows that the sequence $T_{i+1} - T_i,\ldots, T_{i+n-1} - T_i$ has the same joint distribution as $U_{(1)},...,U_{(n-1)}$, which shows \eqref{eq:BiT}.   %with $\phi_1,\ldots,\phi_n$ be $U_1, \ldots, U_n$, $T_{i+1} - T_i,\ldots, T_{i+n-1} - T_i$ be $W_1, \ldots,W_{n-1}$ and conclude Step 2.
    % \jylb{this proves step 2, the rest is verbose} and observe that 
    % \begin{align}
    %     \P\lp \bigcup_{j = i}^{i + n -1} \lc (T_j - T_i) < \frac{(j - i + 1)l - b}{\ltot} \rc \rp = \P \lp \bigcup_{k = 1}^{n-1} \lc U_{(k)} < \frac{(k + 1)l - b}{\ltot} \rc \rp
    % \end{align}
    % Combine it with \eqref{eq:s21} and obtain
    %     \begin{align} \label{eq:BiPhi}
    %     \P\lp       B_i > b \rp = \P \lp \bigcup_{k = 1}^{n-1} \lc U_{(k)} < \frac{(k + 1)l - b}{\ltot} \rc \rp
    % \end{align}
    % % As phases $\phi$ are independently and  uniformly distributed in $[0,1]$, it follows that, given $\phi_{(i)}$, the right-hand side of \eqref{eq:T} are $n-1$ iid standard uniform random variables that are ordered, hence we replace them by $U_{(1)},...,U_{(n-1)}$; combining this with \eqref{eq:s21} we have
    % % \begin{align} \label{eq:BiPhi}
    % %     \lc B_i > b \giventhat \phi_{(i)}\rc = \bigcup_{k = 1}^{n-1} \lc U_{(k)} < \frac{(k + 1)l - b}{\ltot} \rc
    % % \end{align}
    % % As $\phi_{(i)}$ is a standard uniform random variable, we have $ \P\lp B_i > b \rp = \P\lp B_i > b \giventhat \phi_{(i)}\rp \P\lp\phi_{(i)}\rp =  \P\lp B_i > b \giventhat \phi_{(i)}\rp$; also, 
    % As $U_{(k)} \geq 0$ for $k = 1:n-1$ and $\frac{(k + 1)l - b}{\ltot}  < 0$ for $k=1: \lfloor \frac{b}{l} \rfloor - 1$ we obtain \eqref{eq:BiT}, and hence, Step 2 is concluded. 
    % % % $k \in \{1,\ldots,n-1\}$
    % % . Combine these with \eqref{eq:BiPhi} to conclude \eqref{eq:BiT}. 

    Combine \eqref{eq:p1s1} and \eqref{eq:BiT}: 
    % It follows that
    \begin{equation} \label{eq:s41}
       \lc B > b \rc  = \bigcup_{i=1}^n \lc B_i > b \rc \Rightarrow \P \lp B > b \rp  \leq \sum_{i=1}^n \underbrace{\P \lp B_i > b \rp}_{\P(E)} = n\P(E)
    \end{equation} 
    Therefore, the proposition is concluded.   
    \qed
    % Combining it with Step 2, 
    % % \begin{equation} \label{eq:s41}
    % %    \P \lp B > b \rp  = \bigcup_{i=1}^n \P \lp B_i > b \rp 
    % % \end{equation}
    % % Combining Step 2 and Step 3, we have 
    % \begin{equation}\label{eq:s42}
    %    % \forall i \in \{1,\ldots,n\}, 
    %    \P \lp B_i > b \rp  = 1 -  p(n,l,b), \;\;\; i = 1:n
    % \end{equation}
    % Combining \eqref{eq:s41} and \eqref{eq:s42} we have 
    % \begin{equation} \label{eq:s43}
    %    \P \lp B > b \rp  = n\P \lp B_i > b \rp =  n\lp 1 -  p(n,l,b)\rp 
    % \end{equation}
    % which concludes  the theorem. 
    % \textbf{Step 3 (Order Statistics)}:  We show that following:
    % \begin{equation} \label{eq:order}
    %     \P \lp \bigcap_{k = 1}^{n-1} \lc U_{(k)} \geq \frac{\lb (k + 1)l - b \rb^+}{\ltot} \rc \rp = p(n,l,b)
    % \end{equation}
    % The density function of the distribution of $U_{(1)},...,U_{(n-1)}$ is \cite[Equation 1.145]{gentle2009computational}
    % \begin{equation}
    %     f_{U_{(1)},...,U_{(n-1)}}\lp y_{1},...,y_{n-1} \rp  = (n-1)!\prod_{k=1}^{n-1}f_{U}(y_{k})\ind{y_{1}\leq y_2 \leq  \ldots \leq y_{n-1}}
    % \end{equation}
    % where $f_U$ is the probability density function of a standard uniform; as $y_{k} \in [0,1]$, $f_{U}(y_{k}) = 1$ for $k = 1:n-1$
    % % $k \in \{1,\ldots,n-1\}$
    % . Hence,
    % \begin{equation}
    %     f_{U_{(1)},...,U_{(n-1)}}\lp y_{1},...,y_{n-1} \rp  = (n-1)!\ind{y_{1}\leq y_2 \leq  \ldots \leq y_{n-1}}
    % \end{equation}
    % The probability of the left-hand side of \eqref{eq:order} is equal to the probability that  $k = 1:n-1, U_{(k)} \geq \frac{(k + 1)l - b}{\ltot} = u_k$, hence $ \P \lp \bigcap_{k = 1}^{n-1} \lc U_{(k)} \geq \frac{\lb (k + 1)l - b \rb^+}{\ltot} \rc \rp = $
    % \begin{align}
    %     &\int_{y_{n-1} = u_{n-1}}^{1} \ldots \int_{y_{i} = u_{i}}^{1} \ldots \int_{y_{1} = u_{1}}^{1} f_{U_{(1)},...,U_{(n-1)}}\lp y_{1},...,y_{n-1} \rp    \,dy_1 \ldots \,dy_{n-1} \\
    %     &=\int_{y_{n-1} = u_{n-1}}^{1} \ldots \int_{y_{i} = u_{i}}^{1} \ldots \int_{y_{1} = u_{1}}^{1} (n-1)!\ind{y_{1}\leq y_2 \leq  \ldots \leq y_{n-1}}   \,dy_1 \ldots \,dy_{n-1} \\
    %     &=(n-1)!\int_{y_{n-1} = u_{n-1}}^{1}  \ldots \int_{y_{i} = u_{i}}^{y_{i+1}} \ldots \int_{y_{1} = u_{1}}^{y_{2}} 1   \,dy_1 \ldots \,dy_{n-1} = p(n,l,b) 
    %     % \\
    %     % &= p(n,l,b)
    % \end{align}
    % \textbf{Final Step (Union Bound)}: We proceed to prove the theorem. By Step 1, 
    % % It follows that
    % \begin{equation} \label{eq:s41}
    %    \lc B > b \rc  = \bigcup_{i=1}^n \lc B_i > b \rc \Rightarrow \P \lp B > b \rp  = \sum_{i=1}^n \P \lp B_i > b \rp
    % \end{equation}
    % % \begin{equation} \label{eq:s41}
    % %    \P \lp B > b \rp  = \bigcup_{i=1}^n \P \lp B_i > b \rp 
    % % \end{equation}
    % Combining Step 2 and Step 3, we have 
    % \begin{equation}\label{eq:s42}
    %    % \forall i \in \{1,\ldots,n\}, 
    %    \P \lp B_i > b \rp  = 1 -  p(n,l,b), \;\;\; i = 1:n
    % \end{equation}
    % Combining \eqref{eq:s41} and \eqref{eq:s42} we have 
    % \begin{equation} \label{eq:s43}
    %    \P \lp B > b \rp  = n\P \lp B_i > b \rp =  n\lp 1 -  p(n,l,b)\rp 
    % \end{equation}
    % which concludes  the theorem. 
\end{proof}
% We now present our main result.
% by upper bounding of $\P(E)$ hence the tail probability of the aggregate burstiness.
% Lemma~\ref{lem:main} introduces  the event $E$ such that an upper bound of $\P(E)$ is an upper bound on the tail probability of the aggregate burstiness.  In Theorem~\ref{thm:homog_dkw}, we provide a closed-form expression that upper-bounds $\P(E)$ hence the tail probability of the aggregate burstiness. 
\begin{theorem}[Flows with the same period and  packet-size, DKW bound] \label{thm:homog_dkw}
Assume the assumptions of Section~\ref{sec:assump}, and also assume that flows have the same period and same packet size, i.e., for every flow $f=1:n$, $\tau_f = \tau$ and $l_f = l$ for some $l, \tau > 0$. Also, consider some $ b < \ltot = nl$. Then, a bound on the tail probability of the aggregate burstiness $B$ is given by 
\begin{equation}\label{eq:epsdkw}
     \P\lp B > b\rp \leq n\exp{\lp-2(n-1)\lp \frac{\lfloor\frac{b}{l} \rfloor}{n-1} - \frac{1}{n}\rp^2 \rp} \isdef \epdkw(n,l,b)
\end{equation}
% In the above, $B$ is the aggregate burstiness defined in \eqref{eq:agg_burst}.
% Also,  $\epdkw(n,l,b) \geq \ep(n,l,b)$ where $\ep(n,l,b)$ is the bound of Theorem~\ref{thm:homog}.
\end{theorem}
\begin{proof}
    Observe that when $ \lfloor\frac{b}{l} \rfloor < 1-\frac1n +\sqrt{\frac{(n-1)\log 2}{2}}$, we have $\epdkw(n,l,b)\geq \frac n 2$, hence \eqref{eq:epsdkw} holds when $n\geq 2$. For $n=1$, \eqref{eq:epsdkw} holds because the right-hand side is $1$. Therefore we now proceed to prove \eqref{eq:epsdkw} when $n\geq 2$ and  $ \lfloor\frac{b}{l} \rfloor \geq  1-\frac1n +\sqrt{\frac{(n-1)\log 2}{2}}$.
    
       \textbf{Step 1:} Recall that $U_{1},...,U_{n-1}$ is a sequence of $n-1$ 
      iid standard uniform random variables and $U_{(1)},...,U_{(n-1)}$ is the corresponding order statistics, arranged in non-decreasing order.  For $\varepsilon > 0$, define $E'(\varepsilon)$ by
        \begin{equation} \label{eq:Eprime}
             E'(\varepsilon) \isdef \bigcup_{k=1}^{n-1} 
            \lc U_{(k)} < \frac{k}{n-1}-\varepsilon\rc  
        \end{equation}
We now show that
  \begin{equation} 
     \P\lp E'(\varepsilon)\rp \leq e^{-2(n-1)\varepsilon^2} \mif \varepsilon \geq \sqrt{\frac{\log 2}{2(n-1)}} 
     \label{eq:s1DKW}
 \end{equation} 
% \begin{equation} 
%      \P\lp E'(\varepsilon)\rp \leq e^{-2(n-1)\varepsilon^2} \mif \varepsilon \geq \varepsilon_0 \melse    \P\lp E'(\varepsilon)\rp \leq \frac{1}{2}
%      \label{eq:s1DKW}
%  \end{equation} 
 %   \begin{equation} 
 %     \P\lp E'(\varepsilon)\rp \leq e^{-2(n-1)\varepsilon^2} \ind{\epsilon \geq \epsilon_0} + \frac{1}{2}\ind{\epsilon < \epsilon_0} 
 %     % \mif \varepsilon \geq \sqrt{\frac{\log 2}{2(n-1)}} \melse    \P\lp E'(\varepsilon)\rp \leq \frac{1}{2}
 %     % \label{eq:s1DKW}
 % \end{equation} 
%       We show the following equation:
%   \begin{equation} 
%      \P(E')\leq e^{-2(n-1)\varepsilon^2} \mif \varepsilon \geq \sqrt{\frac{\log 2}{2(n-1)}}
%      \label{eq:s1DKW}
%  \end{equation} 
%  with 
%   \begin{equation} \label{eq:Eprime}
%    E' = \bigcup_{k=1}^{n-1} 
%    \lc U_{(k)} < \frac{k}{n-1}-\varepsilon\rc  
% \end{equation}
Let $F_{n-1}$ be the (random) empirical cumulative distribution function of $U_1,...,U_{n-1}$, defined  $\forall x \in [0,1]$ by
\begin{equation}
     F_{n-1}(x)=\frac{1}{n-1}\sum_{i=1}^{n-1}\ind{U_{(i)}\leq x}
 \end{equation} 
The Dvoretzky–Kiefer–Wolfowitz inequality \cite{massart1990tight} states that
\begin{equation}
     \P(\sup_{x\in[0,~1]} (F_{n-1}(x)-x)>\varepsilon  )\leq e^{-2(n-1)\varepsilon^2} \mif \varepsilon \geq \sqrt{\frac{\log 2}{2(n-1)}}
     \label{eq-wpjgrt}
 \end{equation} 
 We can apply this to find the bound of interest. First, we prove that
 \begin{equation} \label{hgqewd}
     (\sup_{x\in[0,~1]} (F_{n-1}(x)-x)>\varepsilon)
     \Leftrightarrow
     (\exists k\in \lc 1,..., n-1\rc, U_{(k)}<\frac{k}{n-1}-\varepsilon)
 \end{equation}
 
Proof of  $\Leftarrow$: By the right-hand side, it follows that $\frac{k}{n-1} - U_{(k)} > \varepsilon$ for some $k$. Also, observe that $F_{n-1}\lp U_{(k)}\rp  = \frac{k}{n-1}$. Hence, $F_{n-1}\lp x\rp - x>\varepsilon$ for $x = U_{(k)}$, and thus the left-hand side is shown.

Proof of $\Rightarrow$: Observe that   for $k = 1:(n-2)$ and $U_{(k)} \leq x < U_{(k+1)}$, $F_{n-1}\lp x\rp = F_{n-1}\lp U_{(k)}\rp = \frac{k}{n-1}$. Also, observe that $x > U_{(n-1)}$, $F_{n-1}\lp x\rp = 1$ and $x < U_{(1)}$, $F_{n-1}\lp x\rp = 0$. 
Hence, 
\begin{equation}
    F_{n-1}(x) - x =  \begin{cases} 
         -x & \text{if } 0 \leq x < U_{(1)}\\
         \frac{k}{n-1} - x & \text{if } U_{(k)} \leq x < U_{(k+1)} \text{for $k =1:(n-2)$} \\
            1 - x & \text{if }   U_{(n-1)} \leq x \leq  1
    \end{cases}
\end{equation}
Thus, $F_{n-1}(x) - x \leq 0 \leq \epsilon$ when $0 \leq x < U_{(1)}$  and $F_{n-1}(x) - x$ is decreasing for $U_{(n)} \leq x \leq  1$ and for $ U_{(k)} \leq x < U_{(k+1)}$ with $k =1:(n-2)$. Hence, the supremum in the left-hand side of \eqref{hgqewd} is obtained for some $x =  U_{(k)}$, i.e., $\sup_{x\in[0,~1]} (F_{n-1}(x)-x) = \sup_{k\in\{ 1,\ldots,n-1\}} (F_{n-1}(U_{(k)})-U_{(k)}) = \sup_{k\in\{ 1,\ldots,n-1\}} (\frac{k}{n-1}-U_{(k)})$, which implies the right-hand side.




% it implies that $\exists k \in \{ 1,\ldots,n-1\}$ the supremum is obtained for some $x =  U_{(k)}$, i.e., 


% First, observe that for $k = 1:(n-2)$ and $U_{(k)} \leq x < U_{(k+1)}$, $F_{n-1}\lp x\rp = F_{n-1}\lp U_{(k)}\rp = \frac{k}{n-1}$. Second, observe that $x > U_{(n-1)}$, $F_{n-1}\lp x\rp = 1$ and $x < U_{(1)}$, $F_{n-1}\lp x\rp = 0$. Third, observe


% , and as $F_{n-1}\lp U_{(k)}\rp =  \frac{k}{n-1} - U_{(k)}$, we have  $\varepsilon<F_{n-1}\lp U_{(k)}\rp - U_{(k)}$. Also,  as $0 \leq U_{(k)} \leq 1$,  we have 
 
%  This is obtained by observing that if the inequality $F_{n-1}(x)-x>\varepsilon$ occurs for some $x$, then it must occur for $x=U_{(k)}$ for some $k$.
  Hence, \eqref{hgqewd} is shown; combine it with  \eqref{eq-wpjgrt} to show \eqref{eq:s1DKW}, and conclude Step~1.


 \textbf{Step 2:} We now proceed to show that if 
  \begin{equation} \label{eq:eps}
    \varepsilon = \frac{\lfloor \frac{b}{l} \rfloor}{n-1}-\frac{1}{n}
\end{equation}
then, $E\subseteq E'(\varepsilon)$, where  event $E$ is defined in Proposition~\ref{prop:main}.

Fix $k \in \lfloor \frac{b}{l}\rfloor:(n-1)$. As $k \geq \lfloor \frac{b}{l}\rfloor$ and $\frac{1}{n-1} + \frac{1}{n} > 0$, we have $\frac{k}{n-1} - \frac{k}{n} \geq \frac{\lfloor \frac{b}{l}\rfloor}{n-1} - \frac{\lfloor \frac{b}{l}\rfloor}{n} $; also, as $ \frac{b}{l} \geq \lfloor \frac{b}{l}\rfloor$, we have  $\frac{k}{n-1} - \frac{k}{n} \geq \frac{\lfloor \frac{b}{l}\rfloor}{n-1} - \frac{\frac{b}{l}}{n} $; then, add $\frac{1}{n}$ to the both side of the inequality and obtain  $\frac{k}{n-1} - \frac{k}{n} + \frac{1}{n} \geq \frac{\lfloor \frac{b}{l}\rfloor}{n-1} - \frac{\frac{b}{l}}{n} + \frac{1}{n} $, which can be rewritten as $\frac{k}{n-1} - \underbrace{(\frac{\lfloor \frac{b}{l}\rfloor}{n-1} - \frac{1}{n} )}_{\varepsilon} \geq \frac{k+1 + \frac{b}{l}}{n}$.
% \begin{equation}
%     \frac{k}{n-1} - \underbrace{(\frac{\lfloor \frac{b}{l}\rfloor}{n-1} - \frac{1}{n} )}_{\varepsilon} \geq \frac{k+1 + \frac{b}{l}}{n}
% \end{equation}
Then, it follows that $U_{(k)}<\frac{(k+1)l-b}{\ltot}$ implies $U_{(k)} < \frac{k}{n-1}-\varepsilon$ for all $k=\lfloor \frac{b}{l}\rfloor:(n-1)$, and thus $E\subseteq E'(\varepsilon)$. 
% , which concludes Step 2.
% as the above inequality holds for $k \in \lfloor \frac{b}{l}\rfloor:(n-1)$, it follows that 
 
% %  that the largest possible $\varepsilon$ such that $E\subseteq E'$ is 
% %  \begin{equation} \label{eq:eps}
% %     \varepsilon = \frac{\lfloor \bar{b}\rfloor}{n-1}-\frac{1}{n}
% % \end{equation}
% \jylb{this is contorted. Please make a straightforward sequence of implications.}
% \hossein{To prove that $E\subseteq E'(\varepsilon)$, we need to show that if $U_{(k)}<\frac{(k+1)l-b}{\ltot}$ then $U_{(k)} < \frac{k}{n-1}-\varepsilon$ for all $k=\lfloor \frac{b}{l}\rfloor:(n-1)$; this is equivalent to proving that $\frac{k+1-\frac{b}{l}}{n}\leq \frac{k}{n-1}-\varepsilon$ for all $k=\lfloor \frac{b}{l}\rfloor:(n-1)$, i.e., $\varepsilon \leq \min_{k=\lfloor \frac{b}{l}\rfloor:(n-1)} \lc \frac{k}{n-1}-\frac{k+1-\frac{b}{l}}{n} \rc $. Observe that the minimum of the right-hand side is obtained for $k=\lfloor \frac{b}{l} \rfloor$, and thus  $\varepsilon \leq \frac{\lfloor \frac{b}{l} \rfloor}{n-1}-\frac{\lfloor \frac{b}{l} \rfloor+1-\frac{b}{l}}{n}$; as $\frac{b}{l} \geq \lfloor \frac{b}{l} \rfloor$, we must have $\varepsilon \leq \frac{\lfloor \frac{b}{l} \rfloor}{n-1}-\frac{1}{n} $ which is true for the value of $\varepsilon$ in \eqref{eq:eps}, and hence Step 2 is concluded.}

% Observe that $E\subseteq E'(\varepsilon)$ is implied if $\forall k \in\lc\lfloor \frac{b}{l} \rfloor,...,n-1\rc$, $\frac{k+1-\frac{b}{l}}{n}\leq \frac{k}{n-1}-\varepsilon$ which can be rewritten as $\varepsilon \leq \frac{k}{n-1}-\frac{k+1-\frac{b}{l}}{n}$; as the minimum over $k$ of the right-hand side is obtained for $k=\lfloor \frac{b}{l} \rfloor$, we must have $\varepsilon \leq \frac{\lfloor \frac{b}{l} \rfloor}{n-1}-\frac{\lfloor \frac{b}{l} \rfloor+1-\frac{b}{l}}{n}$, which is true for the value of $\varepsilon $ given in \eqref{eq:eps}, and hence Step 2 is concluded.


% \begin{equation}
%     \frac{k+1-\frac{b}{l}}{n}\leq \frac{k}{n-1}-\varepsilon = \frac{k}{n-1} - \frac{\lfloor \frac{b}{l} \rfloor}{n-1}-\frac{1}{n},\;\;\;\forall k \in\lc\lfloor \frac{b}{l} \rfloor,...,n-1\rc
% \end{equation}
% which can be rewritten as follows
% \begin{equation}
%     \frac{\lfloor \frac{b}{l} \rfloor}{n-1} - \frac{\frac{b}{l}}{n} \leq   \frac{k}{n-1} - \frac{k}{n} ,\;\;\;\forall k \in\lc\lfloor \frac{b}{l} \rfloor,...,n-1\rc
% \end{equation}
% The minimum over $k$ of the right-handside is obtained for $k=\lfloor \bar{b}\rfloor$ and as $ \frac{b}{l} \geq \lfloor \frac{b}{l} \rfloor$, hence the equation above is shown, and Step 2 is concluded.

% then $E\subseteq E'$. We are looking for $\varepsilon$ that satisfies 
% \begin{equation}
%     \varepsilon\leq \frac{k}{n-1}-\frac{k+1-\bar{b}}{n},\;\;\;\forall k \in\lc\lfloor \bar{b}\rfloor,...,n-1\rc
% \label{eq-dfksjn}
% \end{equation}
% The minimum over $k$ of the right-handside is obtained for $k=\lfloor \bar{b}\rfloor$, therefore \eqref{eq-dfksjn} is equivalent to 
% \begin{equation}
%     \varepsilon\leq \frac{\lfloor \bar{b}\rfloor}{n-1}-\frac{\lfloor \bar{b}\rfloor+1-\bar{b}}{n}
% \end{equation}
% and as $\bar{b}-\lfloor \bar{b}\rfloor\geq 0$, conclude Step 2.

\textbf{Final Step:}
By Step 2, we have $ \P(E) \leq \P(E'(\varepsilon))$. Also,  observe that $ \lfloor\frac{b}{l} \rfloor\geq 1-\frac1n +\sqrt{\frac{(n-1)\log 2}{2}}$ implies $\varepsilon \geq \sqrt{\frac{\log 2}{2(n-1)}}$. Thus, combine it with Step 1 to obtain $\P(E)\leq \P(E'(\varepsilon)) \leq  \exp{\lp-2(n-1) \lp\frac{\lfloor \frac{b}{l} \rfloor}{n-1}-\frac{1}{n}\rp^2\rp}$. Combine it with Proposition~\ref{prop:main} to conclude the theorem. \qed
% \begin{equation} \label{eq:e}
%     \P(E)\leq \P(E'(\varepsilon)) \leq  \exp{\lp-2(n-1) \lp\frac{\lfloor \frac{b}{l} \rfloor}{n-1}-\frac{1}{n}\rp^2\rp}
% \end{equation}
% Combine \eqref{eq:e} with Proposition~\ref{prop:main} to conclude the theorem. \qed

% \hossein{By Step 2, we have $ \P(E) \leq \P(E'(\varepsilon))$. Combine it with Step 1 to obtain
% \begin{equation} \label{eq:e}
%     \P(E) \leq  \exp{\lp-2(n-1) \lp\frac{\lfloor \frac{b}{l} \rfloor}{n-1}-\frac{1}{n}\rp^2\rp}
% \end{equation}
% provided that $\varepsilon = \frac{\lfloor \frac{b}{l} \rfloor}{n-1}-\frac{1}{n} \geq \sqrt{\frac{\log 2}{2(n-1)}}$, i.e., provided that
% \begin{equation}
%     % \lp \frac{\lfloor b\rfloor}{n-1}-\frac{1}{n}\rp^2\geq \frac{\log 2}{n-1}
%     \lfloor \frac{b}{l} \rfloor \geq 1-\frac1n +\sqrt{\frac{\log 2}{2}}\sqrt{n-1}
%      \label{eq-ghefq}
% \end{equation}
% Combine \eqref{eq:e} with Proposition~\ref{prop:main} to conclude the theorem. \qed}

% For the value of $\varepsilon $ obtained at Step 2, we have $E\subseteq E'(\varepsilon)$ and thus, combine \eqref{eq:s1DKW},  \eqref{eq:eps}, and Proposition~\ref{prop:main} to obtain

% \begin{equation}
%     \P\lp B > b\rp \leq n\P(E) \leq n\P(E') \leq n \exp{\lp-2(n-1) \lp\frac{\lfloor \frac{b}{l} \rfloor}{n-1}-\frac{1}{n}\rp^2\rp}
%     \label{eq-jhwdef}
% \end{equation}
% provided that $\varepsilon \geq \sqrt{\frac{\log 2}{2(n-1)}}$, i.e., provided that
% \begin{equation}
%     % \lp \frac{\lfloor b\rfloor}{n-1}-\frac{1}{n}\rp^2\geq \frac{\log 2}{n-1}
%     \lfloor \frac{b}{l} \rfloor \geq 1-\frac1n +\sqrt{\frac{\log 2}{2}}\sqrt{n-1}
%      \label{eq-ghefq}
% \end{equation}
% which concludes the theorem. \qed
\end{proof}
% \begin{proof}
%     Observe that when $ \lfloor\frac{b}{l} \rfloor < 1-\frac1n +\sqrt{\frac{(n-1)\log 2}{2}}$, we have $\epdkw(n,l,b)\geq \frac n 2$, hence \eqref{eq:epsdkw} holds when $n\geq 2$. For $n=1$, \eqref{eq:epsdkw} holds because the right-hand side is $1$. Therefore we now proceed to prove \eqref{eq:epsdkw} when $n\geq 2$ and  $ \lfloor\frac{b}{l} \rfloor \geq  1-\frac1n +\sqrt{\frac{(n-1)\log 2}{2}}$.
    
%        \textbf{Step 1:} Recall that $U_{1},...,U_{n-1}$ is a sequence of $n-1$ 
%       iid standard uniform random variables and $U_{(1)},...,U_{(n-1)}$ is the corresponding order statistics, arranged in non-decreasing order.  For $\varepsilon > 0$, define $E'(\varepsilon)$ by
%         \begin{equation} \label{eq:Eprime}
%              E'(\varepsilon) \isdef \bigcup_{k=1}^{n-1} 
%             \lc U_{(k)} < \frac{k}{n-1}-\varepsilon\rc  
%         \end{equation}
% We now show that
%   \begin{equation} 
%      \P\lp E'(\varepsilon)\rp \leq e^{-2(n-1)\varepsilon^2} \mif \varepsilon \geq \sqrt{\frac{\log 2}{2(n-1)}} 
%      \label{eq:s1DKW}
%  \end{equation} 
% % \begin{equation} 
% %      \P\lp E'(\varepsilon)\rp \leq e^{-2(n-1)\varepsilon^2} \mif \varepsilon \geq \varepsilon_0 \melse    \P\lp E'(\varepsilon)\rp \leq \frac{1}{2}
% %      \label{eq:s1DKW}
% %  \end{equation} 
%  %   \begin{equation} 
%  %     \P\lp E'(\varepsilon)\rp \leq e^{-2(n-1)\varepsilon^2} \ind{\epsilon \geq \epsilon_0} + \frac{1}{2}\ind{\epsilon < \epsilon_0} 
%  %     % \mif \varepsilon \geq \sqrt{\frac{\log 2}{2(n-1)}} \melse    \P\lp E'(\varepsilon)\rp \leq \frac{1}{2}
%  %     % \label{eq:s1DKW}
%  % \end{equation} 
% %       We show the following equation:
% %   \begin{equation} 
% %      \P(E')\leq e^{-2(n-1)\varepsilon^2} \mif \varepsilon \geq \sqrt{\frac{\log 2}{2(n-1)}}
% %      \label{eq:s1DKW}
% %  \end{equation} 
% %  with 
% %   \begin{equation} \label{eq:Eprime}
% %    E' = \bigcup_{k=1}^{n-1} 
% %    \lc U_{(k)} < \frac{k}{n-1}-\varepsilon\rc  
% % \end{equation}
% Let $F_{n-1}$ be the (random) empirical cumulative distribution function of $U_1,...,U_{n-1}$, defined  $\forall x \in [0,1]$ by
% \begin{equation}
%      F_{n-1}(x)=\frac{1}{n-1}\sum_{i=1}^{n-1}\ind{U_{(i)}\leq x}
%  \end{equation} 
% The Dvoretzky–Kiefer–Wolfowitz inequality \cite{massart1990tight} states that
% \begin{equation}
%      \P\lp \sup_{x\in[0,~1]} (F_{n-1}(x)-x)>\varepsilon  \rp\leq e^{-2(n-1)\varepsilon^2} \mif \varepsilon \geq \sqrt{\frac{\log 2}{2(n-1)}}
%      \label{eq-wpjgrt}
%  \end{equation} 
%  We can apply this to find the bound of interest. First, we prove that
%  \begin{equation} \label{hgqewd}
%      \lp\sup_{x\in[0,~1]} (F_{n-1}(x)-x)>\varepsilon\rp 
%      \Leftrightarrow
%      \lp\exists k\in \lc 1,..., n-1\rc, U_{(k)}<\frac{k}{n-1}-\varepsilon\rp
%  \end{equation}
 
% Proof of  $\Leftarrow$: By the right-hand side, it follows that $\frac{k}{n-1} - U_{(k)} > \varepsilon$ for some $k$. Also, observe that $F_{n-1}\lp U_{(k)}\rp  = \frac{k}{n-1}$. Hence, $F_{n-1}\lp x\rp - x>\varepsilon$ for $x = U_{(k)}$, and thus the left-hand side is shown.

% Proof of $\Rightarrow$: Observe that   for $k = 1:(n-2)$ and $U_{(k)} \leq x < U_{(k+1)}$, $F_{n-1}\lp x\rp = F_{n-1}\lp U_{(k)}\rp = \frac{k}{n-1}$. Also, observe that $x > U_{(n-1)}$, $F_{n-1}\lp x\rp = 1$ and $x < U_{(1)}$, $F_{n-1}\lp x\rp = 0$. 
% Hence, 
% \begin{equation}
%     F_{n-1}(x) - x =  \begin{cases} 
%          -x & \text{if } 0 \leq x < U_{(1)}\\
%          \frac{k}{n-1} - x & \text{if } U_{(k)} \leq x < U_{(k+1)} \text{for $k =1:(n-2)$} \\
%             1 - x & \text{if }   U_{(n-1)} \leq x \leq  1
%     \end{cases}
% \end{equation}
% Thus, $F_{n-1}(x) - x \leq 0 \leq \epsilon$ when $0 \leq x < U_{(1)}$  and $F_{n-1}(x) - x$ is decreasing for $U_{(n)} \leq x \leq  1$ and for $ U_{(k)} \leq x < U_{(k+1)}$ with $k =1:(n-2)$. Hence, the supremum in the left-hand side of \eqref{hgqewd} is obtained for some $x =  U_{(k)}$, i.e., $\sup_{x\in[0,~1]} (F_{n-1}(x)-x) = \sup_{k\in\{ 1,\ldots,n-1\}} (F_{n-1}(U_{(k)})-U_{(k)}) = \sup_{k\in\{ 1,\ldots,n-1\}} (\frac{k}{n-1}-U_{(k)})$, which implies the right-hand side.




% % it implies that $\exists k \in \{ 1,\ldots,n-1\}$ the supremum is obtained for some $x =  U_{(k)}$, i.e., 


% % First, observe that for $k = 1:(n-2)$ and $U_{(k)} \leq x < U_{(k+1)}$, $F_{n-1}\lp x\rp = F_{n-1}\lp U_{(k)}\rp = \frac{k}{n-1}$. Second, observe that $x > U_{(n-1)}$, $F_{n-1}\lp x\rp = 1$ and $x < U_{(1)}$, $F_{n-1}\lp x\rp = 0$. Third, observe


% % , and as $F_{n-1}\lp U_{(k)}\rp =  \frac{k}{n-1} - U_{(k)}$, we have  $\varepsilon<F_{n-1}\lp U_{(k)}\rp - U_{(k)}$. Also,  as $0 \leq U_{(k)} \leq 1$,  we have 
 
% %  This is obtained by observing that if the inequality $F_{n-1}(x)-x>\varepsilon$ occurs for some $x$, then it must occur for $x=U_{(k)}$ for some $k$.
 
%  Hence, \eqref{hgqewd} is shown; now combine it with  \eqref{eq-wpjgrt} to show \eqref{eq:s1DKW}, which concludes Step 1.


%  \textbf{Step 2:} We now proceed to show that if 
%   \begin{equation} \label{eq:eps}
%     \varepsilon = \frac{\lfloor \frac{b}{l} \rfloor}{n-1}-\frac{1}{n}
% \end{equation}
% then, $E\subseteq E'(\varepsilon)$, where  event $E$ is defined in Proposition~\ref{prop:main}.

% Fix $k \in \lfloor \frac{b}{l}\rfloor:(n-1)$. As $k \geq \lfloor \frac{b}{l}\rfloor$ and $\frac{1}{n-1} + \frac{1}{n} > 0$, we have $\frac{k}{n-1} - \frac{k}{n} \geq \frac{\lfloor \frac{b}{l}\rfloor}{n-1} - \frac{\lfloor \frac{b}{l}\rfloor}{n} $; also, as $ \frac{b}{l} \geq \lfloor \frac{b}{l}\rfloor$, we have  $\frac{k}{n-1} - \frac{k}{n} \geq \frac{\lfloor \frac{b}{l}\rfloor}{n-1} - \frac{\frac{b}{l}}{n} $; then, add $\frac{1}{n}$ to the both side of the inequality and obtain  $\frac{k}{n-1} - \frac{k}{n} + \frac{1}{n} \geq \frac{\lfloor \frac{b}{l}\rfloor}{n-1} - \frac{\frac{b}{l}}{n} + \frac{1}{n} $, which can be rewritten as $\frac{k}{n-1} - \underbrace{(\frac{\lfloor \frac{b}{l}\rfloor}{n-1} - \frac{1}{n} )}_{\varepsilon} \geq \frac{k+1 + \frac{b}{l}}{n}$.
% % \begin{equation}
% %     \frac{k}{n-1} - \underbrace{(\frac{\lfloor \frac{b}{l}\rfloor}{n-1} - \frac{1}{n} )}_{\varepsilon} \geq \frac{k+1 + \frac{b}{l}}{n}
% % \end{equation}
% Then, it follows that $U_{(k)}<\frac{(k+1)l-b}{\ltot}$ implies $U_{(k)} < \frac{k}{n-1}-\varepsilon$ for all $k=\lfloor \frac{b}{l}\rfloor:(n-1)$, and thus $E\subseteq E'(\varepsilon)$. 
% % , which concludes Step 2.
% % as the above inequality holds for $k \in \lfloor \frac{b}{l}\rfloor:(n-1)$, it follows that 
 
% % %  that the largest possible $\varepsilon$ such that $E\subseteq E'$ is 
% % %  \begin{equation} \label{eq:eps}
% % %     \varepsilon = \frac{\lfloor \bar{b}\rfloor}{n-1}-\frac{1}{n}
% % % \end{equation}
% % \jylb{this is contorted. Please make a straightforward sequence of implications.}
% % \hossein{To prove that $E\subseteq E'(\varepsilon)$, we need to show that if $U_{(k)}<\frac{(k+1)l-b}{\ltot}$ then $U_{(k)} < \frac{k}{n-1}-\varepsilon$ for all $k=\lfloor \frac{b}{l}\rfloor:(n-1)$; this is equivalent to proving that $\frac{k+1-\frac{b}{l}}{n}\leq \frac{k}{n-1}-\varepsilon$ for all $k=\lfloor \frac{b}{l}\rfloor:(n-1)$, i.e., $\varepsilon \leq \min_{k=\lfloor \frac{b}{l}\rfloor:(n-1)} \lc \frac{k}{n-1}-\frac{k+1-\frac{b}{l}}{n} \rc $. Observe that the minimum of the right-hand side is obtained for $k=\lfloor \frac{b}{l} \rfloor$, and thus  $\varepsilon \leq \frac{\lfloor \frac{b}{l} \rfloor}{n-1}-\frac{\lfloor \frac{b}{l} \rfloor+1-\frac{b}{l}}{n}$; as $\frac{b}{l} \geq \lfloor \frac{b}{l} \rfloor$, we must have $\varepsilon \leq \frac{\lfloor \frac{b}{l} \rfloor}{n-1}-\frac{1}{n} $ which is true for the value of $\varepsilon$ in \eqref{eq:eps}, and hence Step 2 is concluded.}

% % Observe that $E\subseteq E'(\varepsilon)$ is implied if $\forall k \in\lc\lfloor \frac{b}{l} \rfloor,...,n-1\rc$, $\frac{k+1-\frac{b}{l}}{n}\leq \frac{k}{n-1}-\varepsilon$ which can be rewritten as $\varepsilon \leq \frac{k}{n-1}-\frac{k+1-\frac{b}{l}}{n}$; as the minimum over $k$ of the right-hand side is obtained for $k=\lfloor \frac{b}{l} \rfloor$, we must have $\varepsilon \leq \frac{\lfloor \frac{b}{l} \rfloor}{n-1}-\frac{\lfloor \frac{b}{l} \rfloor+1-\frac{b}{l}}{n}$, which is true for the value of $\varepsilon $ given in \eqref{eq:eps}, and hence Step 2 is concluded.


% % \begin{equation}
% %     \frac{k+1-\frac{b}{l}}{n}\leq \frac{k}{n-1}-\varepsilon = \frac{k}{n-1} - \frac{\lfloor \frac{b}{l} \rfloor}{n-1}-\frac{1}{n},\;\;\;\forall k \in\lc\lfloor \frac{b}{l} \rfloor,...,n-1\rc
% % \end{equation}
% % which can be rewritten as follows
% % \begin{equation}
% %     \frac{\lfloor \frac{b}{l} \rfloor}{n-1} - \frac{\frac{b}{l}}{n} \leq   \frac{k}{n-1} - \frac{k}{n} ,\;\;\;\forall k \in\lc\lfloor \frac{b}{l} \rfloor,...,n-1\rc
% % \end{equation}
% % The minimum over $k$ of the right-handside is obtained for $k=\lfloor \bar{b}\rfloor$ and as $ \frac{b}{l} \geq \lfloor \frac{b}{l} \rfloor$, hence the equation above is shown, and Step 2 is concluded.

% % then $E\subseteq E'$. We are looking for $\varepsilon$ that satisfies 
% % \begin{equation}
% %     \varepsilon\leq \frac{k}{n-1}-\frac{k+1-\bar{b}}{n},\;\;\;\forall k \in\lc\lfloor \bar{b}\rfloor,...,n-1\rc
% % \label{eq-dfksjn}
% % \end{equation}
% % The minimum over $k$ of the right-handside is obtained for $k=\lfloor \bar{b}\rfloor$, therefore \eqref{eq-dfksjn} is equivalent to 
% % \begin{equation}
% %     \varepsilon\leq \frac{\lfloor \bar{b}\rfloor}{n-1}-\frac{\lfloor \bar{b}\rfloor+1-\bar{b}}{n}
% % \end{equation}
% % and as $\bar{b}-\lfloor \bar{b}\rfloor\geq 0$, conclude Step 2.

% \textbf{Final Step:}
% By Step 2, we have $ \P(E) \leq \P(E'(\varepsilon))$. Also,  observe that $ \lfloor\frac{b}{l} \rfloor\geq 1-\frac1n +\sqrt{\frac{(n-1)\log 2}{2}}$ implies $\varepsilon \geq \sqrt{\frac{\log 2}{2(n-1)}}$. Thus, combine it with Step 1 to obtain 
% \begin{equation} \label{eq:e}
%     \P(E)\leq \P(E'(\varepsilon)) \leq  \exp{\lp-2(n-1) \lp\frac{\lfloor \frac{b}{l} \rfloor}{n-1}-\frac{1}{n}\rp^2\rp}
% \end{equation}
% Combine \eqref{eq:e} with Proposition~\ref{prop:main} to conclude the theorem. \qed

% % \hossein{By Step 2, we have $ \P(E) \leq \P(E'(\varepsilon))$. Combine it with Step 1 to obtain
% % \begin{equation} \label{eq:e}
% %     \P(E) \leq  \exp{\lp-2(n-1) \lp\frac{\lfloor \frac{b}{l} \rfloor}{n-1}-\frac{1}{n}\rp^2\rp}
% % \end{equation}
% % provided that $\varepsilon = \frac{\lfloor \frac{b}{l} \rfloor}{n-1}-\frac{1}{n} \geq \sqrt{\frac{\log 2}{2(n-1)}}$, i.e., provided that
% % \begin{equation}
% %     % \lp \frac{\lfloor b\rfloor}{n-1}-\frac{1}{n}\rp^2\geq \frac{\log 2}{n-1}
% %     \lfloor \frac{b}{l} \rfloor \geq 1-\frac1n +\sqrt{\frac{\log 2}{2}}\sqrt{n-1}
% %      \label{eq-ghefq}
% % \end{equation}
% % Combine \eqref{eq:e} with Proposition~\ref{prop:main} to conclude the theorem. \qed}

% % For the value of $\varepsilon $ obtained at Step 2, we have $E\subseteq E'(\varepsilon)$ and thus, combine \eqref{eq:s1DKW},  \eqref{eq:eps}, and Proposition~\ref{prop:main} to obtain

% % \begin{equation}
% %     \P\lp B > b\rp \leq n\P(E) \leq n\P(E') \leq n \exp{\lp-2(n-1) \lp\frac{\lfloor \frac{b}{l} \rfloor}{n-1}-\frac{1}{n}\rp^2\rp}
% %     \label{eq-jhwdef}
% % \end{equation}
% % provided that $\varepsilon \geq \sqrt{\frac{\log 2}{2(n-1)}}$, i.e., provided that
% % \begin{equation}
% %     % \lp \frac{\lfloor b\rfloor}{n-1}-\frac{1}{n}\rp^2\geq \frac{\log 2}{n-1}
% %     \lfloor \frac{b}{l} \rfloor \geq 1-\frac1n +\sqrt{\frac{\log 2}{2}}\sqrt{n-1}
% %      \label{eq-ghefq}
% % \end{equation}
% % which concludes the theorem. \qed
% \end{proof}

% Theorem~\ref{thm:homog_dkw} gives a closed-form upper-bound to Theorem~\ref{thm:homog}, and moreover, is obtained using Dvoretzky–Kiefer–Wolfowitz (DKW) inequality which is known to be tight when the number of flows $n$ is large \cite{dkw}. Hence, Theorem~\ref{thm:homog_dkw} has all the properties explained after Theorem~\ref{thm:homog}. We also numerically confirm its tightness (see Fig.~ ??). 

% Note that it is obvious that $\epdkw(n,l,b) = 0$ for $b \geq \ltot = nl$ 
% \jylb{How about the condition on b ? Is it constraining or not ?}
% \hossein{Note that the theorem does not provide a bound when $b$ is smaller than a certain value. However, bounds on the tail probability of the aggregate burstiness for such small values are not interesting as it is very likely that the aggregate burstiness would exceed them. Later, in Theorem~\ref{thm:homog}, we compute  bounds for such small values and numerically observe that they are mostly equal to one (see Fig.~\ref{fig:homog}(a)).}

Note that the bound of Theorem~\ref{thm:homog_dkw} is only less than one and is non-trivial when $  \lfloor\frac{b}{l} \rfloor \geq 1-\frac1n +\sqrt{\frac{(n-1)\log 2}{2}}$.

The following corollary provides a closed-form formulation for the minimum value for the aggregate burstiness with a violation probability of at most $\varepsilon$.  It is obtained by setting the right-hand side of \eqref{eq:epsdkw} in Theorem~\ref{thm:homog_dkw} to $\varepsilon$.
% \hossein{It is obtained by Theorem~\ref{thm:homog_dkw}, and by finding the smallest value of $b$ such that $\epdkw(n,l,b) \leq \varepsilon$.}

%  It is obtained by setting the right-hand side of \eqref{eq:epsdkw} in Theorem~\ref{thm:homog_dkw} to $\varepsilon$.

% \jylb{how about the condition on epsilon ? why does it disappear ?}
\begin{corollary}[Quasi-deterministic burstiness bound] \label{cor:homog_burst}
Assume the assumptions of Theorem~\ref{thm:homog_dkw} and assume that $n\geq 2$. Consider some $0 < \varepsilon < 1$, and define 
\begin{equation}
    b(n,l, \varepsilon) \isdef l\lceil 1 -\frac1n+\sqrt{\frac{(n-1)(\log n-\log\varepsilon)}{2}}\rceil
\end{equation}
Then, $b(n,l, \varepsilon)$ is a quasi-deterministic burstiness bound for the aggregate with the violation probability of at most $\varepsilon$, i.e., $\P\lp B > b\lp n,l, \varepsilon \rp \rp \leq \varepsilon$.
% \begin{equation}
%      \P\lp \exists t \geq 0,~ B(t) > b_F^\epsilon\rp \leq \epsilon
% \end{equation}
\end{corollary}
% \begin{proof}
%     Observe that $\frac{b(n,l, \varepsilon)}{l} = \lfloor\frac{b(n,l, \varepsilon)}{l} \rfloor\geq 1-\frac1n +\sqrt{\frac{(n-1)\log 2}{2}}$ as $\frac{b(n,l, \varepsilon)}{l} $ is an integer and $0 < \varepsilon < 1$. Then, apply Theorem~\ref{thm:homog_dkw} with $b(n,l, \varepsilon)$ and observe that $\epdkw\lp n ,b(n,l, \varepsilon), l  \rp  \leq \varepsilon$.\qed
% \end{proof}

% Corollary~\ref{cor:homog_burst} is obtained by setting the right-hand side of \eqref{eq:epsdkw} in Theorem~\ref{thm:homog_dkw} to $\varepsilon$, i.e., by finding the smallest $b$ such that $\epdkw(n,l,b) \leq \varepsilon$. 
Observe that $b(n, l,\varepsilon)$ grows in $\sqrt{n\log{n}}$ as opposed to the deterministic bound ($\ltot = nl$) that grows in $n$ (see Fig.~\ref{fig:homog}b).
% , i.e., the ratio $\frac{b(n, l,\varepsilon)}{\ltot}$ is in the order of $\sqrt{\frac{\log{n}}{n}}$ (see Fig.~\ref{fig:num}b).
% We also numerically confirm that, given a non-zero violation probability, $b(n, l,\epsilon)$ is tight compared to the burstiness obtained by Theorem~\ref{thm:homog} (see Fig. ??). 
% We now present a refinement to Theorem~\ref{thm:homog_dkw} that  provides slightly  better bounds when the number of flows is small. 

Proposition~\ref{prop:main} introduces the event $E$ such that an upper bound of $\P(E)$ is used to derive an upper bound on the tail probability of the aggregate burstiness.   Theorem~\ref{thm:homog_dkw} is derived from the DKW upper bound of  $\P(E)$, which is tight when the number of flows $n$ is large. In Theorem~\ref{thm:homog}, we replace this closed-form upper bound by the exact value of $\P(E)$; thus, it provides a slightly better bound when the number of flows is small but at the expense of not having a closed-form expression.

% We now present a refinement to Theorem~\ref{thm:homog_dkw} that  provides slightly  better bounds when the number of flows is small.   Lemma~\ref{lem:main} introduces the event $E$ such that an upper bound of $\P(E)$ provides an upper bound on the tail probability of the aggregate burstiness.   Theorem~\ref{thm:homog_dkw} gives a closed-form expression that gives an upper bound to $\P(E)$ using the DKW inequality and  is tight when the number of flows $n$ is large. Theorem~\ref{thm:homog}  exactly computes $\P(E)$; thus, it provides a slightly better bound when the number of flows is small but at the expense of not having a closed-form expression.
 % providing bounds less than or equal to that of Theorem~\ref{thm:homog_dkw}. However,  provides a slightly better bound when the number of flows is small, but at the expense of not having a closed-form expression.

\begin{theorem}[Refinement of Theorem~\ref{thm:homog_dkw} for small groups] \label{thm:homog}
Assume the assumptions of Theorem~\ref{thm:homog_dkw}, and consider some $b \geq 0$. Then, a bound on the tail probability of the aggregate burstiness $B$ is given by

% of Section~\ref{sec:assump}, and also assume that flows have the same period and same packet size, i.e., for every flow $f$, $\tau_f = \tau$ and $l_f = l$ for some $l, \tau > 0$. Consider some $b$. Then, 
\begin{equation} \label{eq:epsThm1}
     \P\lp  B > b\rp \leq n(1 - p(n,l,b)) \isdef \ep(n,l,b) 
\end{equation}
with 
\begin{align}
    \label{eq:pbThm1}
    p(n,l,b) & = (n-1)!\int_{y_{n-1} = u_{n-1}}^{1} \int_{y_{n-2} = u_{n-2}}^{y_{n-1}} \ldots \int_{y_{i} = u_{i}}^{y_{i+1}} \ldots \int_{y_{1} = u_{1}}^{y_{2}} 1   \,dy_1 \ldots \,dy_{n-1} \\
    \label{eq:ukThm1}
    % p(b) & = (n-1)!\int_{y_{n-1} = u_{n-1}}^{1} \int_{y_{n-2} = u_{n-2}}^{y_{n-1}} \ldots \int_{y_{i} = u_{k}}^{y_{k+1}} \ldots \int_{y_{1} = u_{1}}^{y_{2}}    \,dy_1 \ldots \,dy_{n-1}
     u_k &= \frac{[ (k+1)l - b]^+}{\ltot}, \;\;\; k=1:n-1
     % , \forall k \in \{1, \ldots, n-1 \}
\end{align}
 Also,  $\epdkw(n,l,b) \geq \ep(n,l,b)$ where $\epdkw(n,l,b)$ is the bound of Theorem~\ref{thm:homog_dkw}. In \eqref{eq:ukThm1}, $[x]^+=\max\{x,0\}$.
\end{theorem}

Note that the computation of the bound of Theorem~\ref{thm:homog} requires computing $p(n,l,b)$ in \eqref{eq:pbThm1},  which is a series of polynomials integration, and finding a general close-form formula might be challenging. However, it is easy to give an iterative computation as we give in Algorithm~\ref{alg:thm1}. 

% We iteratively compute the bound of Theorem~\ref{thm:homog} in Algorithm~\ref{alg:thm1}. 
 
% Note that $p(n,l,b)$ in \eqref{eq:pbThm1} is a series of polynomials integration, and finding a general close-form formula might be challenging. We iteratively compute the bound of Theorem~\ref{thm:homog} in Algorithm~\ref{alg:thm1}. \jylb{This last sentence is not well written. \eqref{eq:pbThm1} is the same as ``the bound of Theorem~\ref{thm:homog}" but this is not obvious. Also there is no link with the previous sentence. }

 
 % However, we compute the bound of Theorem~\ref{thm:homog} iteratively in Algorithm~\ref{alg:thm1}. 

\begin{algorithm}[H]
	\small 
    \SetKwInOut{IV}{Local Variables}
     \SetKwInOut{Input}{Inputs}
     \SetKwInOut{Output}{Output}
    \Input{number of flows $n$, packet-size $l$, and burst $b$.}
    \Output{$\ep$ such that $\P(B > b) \leq \ep$.}
    % , a bound on the tail probability of the aggregate burstiness, i.e., $\P(B > b) \leq \ep$.}
    % \KwResult{$\ep$, a bound on the tail probability of the aggregate burstiness, i.e., $\P(B > b) \leq \ep$}
    \IV{integer $m$, $u_k$ for $k =\lfloor \frac{b}{l}\rfloor:n-1$, and collections $\lp q_1^m, \ldots, q_m^m \rp$ for $m=\lfloor\frac{b}{l} \rfloor-1:n-1$.}
% 	 \KwResult{$\lp \beta, d, \zcut,b\rp$: Collection of per-node strict service curve, per-node delay bounds,  bounds on propagated burstiness of flows at cuts, and  aggregate burst bound at the output of every node and every edge for all classes}

    % $\forall k \in \{\lfloor b \rfloor - 1, \ldots, n-1 \}$, $u_k \gets$ as in \eqref{eq:ukThm1}\;
    % $\bar{b} \gets \frac{b}{l}$\;
    $m \gets \lfloor \frac{b}{l} \rfloor - 1$\;
    $\lp q_1^m, \ldots, q_m^m \rp \gets \lp 0, 0, \ldots,0, 1 \rp$\;
    \For{$m \leftarrow \lfloor\frac{b}{l}  \rfloor - 1$ to $n-2$}{
        $u_{m+1} \gets$ Compute as in \eqref{eq:ukThm1} with $k = m+1$\;
         $q_0^{m+1} \gets -\sum_{j=0}^m \frac{(m+1)q_j^m}{j+1}u_{m+1}^{j+1} \mand q_{m+1}^{m+1} \gets 1 $\;
        \lFor{$i \leftarrow 1$ to $m$}{
                $q_i^{m+1} \gets \frac{(m+1)q_i^m}{i+1} $
    % $\lp q_1^{m+1}, \ldots, q_{m+1}^{m+1} \rp \gets \Pi\lp \lp q_1^m, \ldots, q_m^m \rp , u_{m+1} \rp$\;
    }
            % $q_{m+1}^{m+1} \gets 1 $\;
    }
    $\ep \gets  n\sum_{i=0}^{n-2} q_i^{n-1}$\;
    \textbf{return} $\ep$
    \caption{ \small Computation of Theorem~\ref{thm:homog}: $\ep\lp n,l,b\rp$}
	\label{alg:thm1}
\end{algorithm}


\begin{proof}
    %  We first show the following equation where recall that event $E$ is defined in Proposition~\ref{prop:main}:
    % \begin{equation} \label{eq:order}
    %     \P \lp E \rp = 1 - p(n,l,b)
    % \end{equation}
    Let $\Bar{E}$ be the complementary event of $E$ (see Proposition~\ref{prop:main}); observe that $\Bar{E} = \bigcap_{k = 1}^{n-1} \lc U_{(k)} \geq \frac{\lb (k + 1)l - b \rb^+}{\ltot} \rc$.
    % \begin{equation}
    %     \Bar{E} = \bigcap_{k = 1}^{n-1} \lc U_{(k)} \geq \frac{\lb (k + 1)l - b \rb^+}{\ltot} \rc
    % \end{equation}
    Recall that $f_{U_{(1)},...,U_{(n-1)}}$, the density function of the joint distribution of $U_{(1)},...,U_{(n-1)}$, is  given in \eqref{eq:orderUniform}.
    % \cite[Equation 1.145]{gentle2009computational}
    % \begin{equation}
    %     f_{U_{(1)},...,U_{(n-1)}}\lp y_{1},...,y_{n-1} \rp  = (n-1)!\prod_{k=1}^{n-1}f_{U}(y_{k})\ind{y_{1}\leq y_2 \leq  \ldots \leq y_{n-1}}
    % \end{equation}
    % where $f_U$ is the probability density function of a standard uniform; as $y_{k} \in [0,1]$, $f_{U}(y_{k}) = 1$ for $k = 1:n-1$
    % % $k \in \{1,\ldots,n-1\}$
    % . Hence,
    % \begin{equation}
    %     f_{U_{(1)},...,U_{(n-1)}}\lp y_{1},...,y_{n-1} \rp  = (n-1)!\ind{y_{1}\leq y_2 \leq  \ldots \leq y_{n-1}}
    % \end{equation}
    $\P \lp \Bar{E} \rp $ is equal to the probability that  $k = 1:n-1, U_{(k)} \geq \frac{(k + 1)l - b}{\ltot} = u_k$, hence 
    % $\P \lp \Bar{E} \rp $
    % $ \P \lp \bigcap_{k = 1}^{n-1} \lc U_{(k)} \geq \frac{\lb (k + 1)l - b \rb^+}{\ltot} \rc \rp = $
    {\footnotesize 
    \begin{align}
       \P \lp \Bar{E} \rp &=  \int_{y_{n-1} = u_{n-1}}^{1} \ldots \int_{y_{i} = u_{i}}^{1} \ldots \int_{y_{1} = u_{1}}^{1} f_{U_{(1)},...,U_{(n-1)}}\lp y_{1},...,y_{n-1} \rp    \,dy_1 \ldots \,dy_{n-1} \\
        &=\int_{y_{n-1} = u_{n-1}}^{1} \ldots \int_{y_{i} = u_{i}}^{1} \ldots \int_{y_{1} = u_{1}}^{1} (n-1)!\ind{0 \leq y_{1}\leq y_2 \leq  \ldots \leq y_{n-1} \leq 1}   \,dy_1 \ldots \,dy_{n-1} \\
        &=(n-1)!\int_{y_{n-1} = u_{n-1}}^{1}  \ldots \int_{y_{i} = u_{i}}^{y_{i+1}} \ldots \int_{y_{1} = u_{1}}^{y_{2}} 1   \,dy_1 \ldots \,dy_{n-1} = p(n,l,b) 
        % \\
        % &= p(n,l,b)
    \end{align}
    }
    Lastly, combine it with  $\P \lp \Bar{E} \rp = 1 - \P \lp E \rp$ and Proposition~\ref{prop:main}. \qed
    % \textbf{Final Step (Union Bound)}: We proceed to prove the theorem. By Step 1, 
    % % It follows that
    % \begin{equation} \label{eq:s41}
    %    \lc B > b \rc  = \bigcup_{i=1}^n \lc B_i > b \rc \Rightarrow \P \lp B > b \rp  = \sum_{i=1}^n \P \lp B_i > b \rp
    % \end{equation}
    % % \begin{equation} \label{eq:s41}
    % %    \P \lp B > b \rp  = \bigcup_{i=1}^n \P \lp B_i > b \rp 
    % % \end{equation}
    % Combining Step 2 and Step 3, we have 
    % \begin{equation}\label{eq:s42}
    %    % \forall i \in \{1,\ldots,n\}, 
    %    \P \lp B_i > b \rp  = 1 -  p(n,l,b), \;\;\; i = 1:n
    % \end{equation}
    % Combining \eqref{eq:s41} and \eqref{eq:s42} we have 
    % \begin{equation} \label{eq:s43}
    %    \P \lp B > b \rp  = n\P \lp B_i > b \rp =  n\lp 1 -  p(n,l,b)\rp 
    % \end{equation}
    % which concludes  the theorem. \qed
\end{proof}

% \section{Homogeneous Case: Flows with the Same Period and Same Packet-size} \label{sec:homogen}
% % We first present our results, with the complete proof, for homogeneous flows in Section~\ref{sec:homogen}. 
% % We then extend them to the case where flows have different packet sizes in Section~\ref{sec:semi-homogen}. 
% % \hossein{
% % \begin{enumerate}
% %     \item Theorem 1: Exact formula
% %     \item Recursive algorithm for computation of the exact formulation
% %     \item Theorem 2: DKW bound 
% % \end{enumerate}}

% % We assume that flows have the same period and same packet size, i.e., for each flow $f$, $\tau_f = \tau$ and $l_f = l$.


% % \subsection{Burstiness Bound by Order Statistics and Union Bound}
% % \subsection{Homogeneous Flows: Same Period and Same Packet-size}


% \begin{theorem}[Flows with Same Period and Packet-size] \label{thm:homog}
% Assume the assumptions of Section~\ref{sec:assump}, and also assume that flows have the same period and same packet size, i.e., for every flow $f$, $\tau_f = \tau$ and $l_f = l$ for some $l, \tau > 0$. Consider some $b$. Then, 
% \begin{equation} \label{eq:epsThm1}
%      \P\lp  B > b\rp \leq n(1 - p(n,l,b)) = \ep(n,l,b) 
% \end{equation}
% with 
% \begin{align}
%     \label{eq:pbThm1}
%     p(n,l,b) & = (n-1)!\int_{y_{n-1} = u_{n-1}}^{1} \int_{y_{n-2} = u_{n-2}}^{y_{n-1}} \ldots \int_{y_{i} = u_{i}}^{y_{i+1}} \ldots \int_{y_{1} = u_{1}}^{y_{2}} 1   \,dy_1 \ldots \,dy_{n-1} \\
%     \label{eq:ukThm1}
%     % p(b) & = (n-1)!\int_{y_{n-1} = u_{n-1}}^{1} \int_{y_{n-2} = u_{n-2}}^{y_{n-1}} \ldots \int_{y_{i} = u_{k}}^{y_{k+1}} \ldots \int_{y_{1} = u_{1}}^{y_{2}}    \,dy_1 \ldots \,dy_{n-1}
%      u_k &= \frac{[ (k+1)l - b]^+}{\ltot}, \;\;\; k=1:n-1
%      % , \forall k \in \{1, \ldots, n-1 \}
% \end{align}
% In \eqref{eq:ukThm1}, $[x]^+=\max\{x,0\}$ and $\ltot = nl$.
% \end{theorem}

%  Note that $p(n,l,b)$ in \eqref{eq:pbThm1} is a series of polynomials integration, thus, finding a general close-form formula might be challenging. However, we compute the bound of Theorem~\ref{thm:homog} iteratively. 
 
%  % Note that $p(n,l,b)$ in \eqref{eq:pbThm1} is a series of polynomials integration, thus giving a general close-form formula might be challenging. Here, we explain how to compute it iteratively in Algorithm~\ref{alg:thm1}.
% % (see Appendix for the correctness of the algorithm).
% \begin{algorithm}[htbp]
	
%     \SetKwInOut{IV}{Local Variables}
%     % \SetKwInOut{Input}{Inputs}
%     % \Input{$\lp n,l,b\rp$}
%     % \KwResult{$\ep$}
%     \IV{integer $m$,\\
%     $\forall k \in \{\lfloor b \rfloor, \ldots, n-1 \}$, $u_k$,\\
%     Sequences $\lp q_1^m, \ldots, q_m^m \rp$ for $m\in \{\lfloor b \rfloor - 1, \ldots, n-1 \}$.}
% % 	 \KwResult{$\lp \beta, d, \zcut,b\rp$: Collection of per-node strict service curve, per-node delay bounds,  bounds on propagated burstiness of flows at cuts, and  aggregate burst bound at the output of every node and every edge for all classes}

%     % $\forall k \in \{\lfloor b \rfloor - 1, \ldots, n-1 \}$, $u_k \gets$ as in \eqref{eq:ukThm1}\;
%     $m \gets \lfloor b \rfloor - 1$\;
%     $\lp q_1^m, \ldots, q_m^m \rp \gets \lp 0, 0, \ldots,0, 1 \rp$\;
%     \For{$m \leftarrow \lfloor b \rfloor - 1$ to $n-2$}{
%         $u_{m+1} \gets$ Compute as in \eqref{eq:ukThm1} with $k = m+1$\;
%          $q_0^{m+1} \gets -\sum_{j=0}^m \frac{(m+1)q_j^m}{j+1}u_{m+1}^{j+1} \mand q_{m+1}^{m+1} \gets 1 $\;
%         \lFor{$i \leftarrow 1$ to $m$}{
%                 $q_i^{m+1} \gets \frac{(m+1)q_i^m}{i+1} $
%     % $\lp q_1^{m+1}, \ldots, q_{m+1}^{m+1} \rp \gets \Pi\lp \lp q_1^m, \ldots, q_m^m \rp , u_{m+1} \rp$\;
%     }
%             % $q_{m+1}^{m+1} \gets 1 $\;
%     }
%     $\ep \gets  n\sum_{i=0}^{n-2} q_i^{n-1}$\;
%     \textbf{return} $\ep$
%     \caption{Computation of Theorem~\ref{thm:homog}: $\ep\lp n,l,b\rp$}
% 	\label{alg:thm1}
% \end{algorithm}
% % Note that all computations of Algorithm~\ref{alg:thm1} can be done using infinite precision arithmetic (with rational numbers), e.g., using symbolic numbers in MATLAB. Although working with symbolic numbers in MATLAB can be costly, we managed to compute the bound of Theorem~\ref{thm:homog} for large $n$ (e.g., $n = 3000$) in a feasible time on a $2.6$ GHz $6$-Core Intel Core i$7$ computer. To mitigate the run-time and memory complexity, in the following theorem, we provide a closed-form expression that upper bounds the bound of Theorem~\ref{thm:homog} and is tight when the number of flows $n$ is large.

%  % Theorem~\ref{thm:homog} provides a token-bucket arrival curve with the rate $\rtot$ and burst $b$ for the aggregate traffic with violation probability of at most $\ep(n,l,b)$;   as explained in Section~\ref{sec:realted_works},  this is of type $\sbbThree$ hence quasi-deterministic. Note that the violation probability $\ep(n,l,b)$ is independent of the period $\tau$ and only depends on packet size $l$, $b$, and the number of flows $n$. 
 
%  % Observe that the bounding function $\ep(n,l,b)$ is wide-sense decreasing in $b$ (i.e., $\ep(n,l,b+1) \leq \ep(n,l,b)$) and  for $b \geq n,~\ep(n,l,b) = 0$. Thus, given a non-zero violation $\varepsilon$, we can find the smallest value $b$ such that $\ep(n,l,b) \leq \varepsilon$, i.e., An estimated quasi-deterministic  burstiness bound that is valid with violation probability of at most $\varepsilon$. We now present the proof and then explain how to concretely compute the bound of Theorem~\ref{thm:homog}.
 

% \begin{proof}
%     % Let $\Bar{B} = \max_{t\geq 0}B(t)$, which is the maximum burstiness throughout the network's lifetime. Then, we want to prove the following:
%     % \begin{equation} \label{eq:t1}
%     %     \P \lp \Bar{B} > b \rp \leq n\lp 1 - p(n,l,b)\rp
%     % \end{equation}
%     The proof consists of several steps. Without loss of generality, we assume that period $\tau = 1$, hence $\rtot = \ltot$ in the rest of the proof:

%     \textbf{Step 1 (Packetized, Periodic flows):} We let $T_j$, for $j \geq 1$, denote the arrival time of the $j$-th packet in the aggregate traffic. We show the following:

%      \begin{equation} \label{eq:s2}
%         B  = \max_{i=1:n}  B_i
%     \end{equation}
%         with 
%     \begin{align}
%     \label{eq:bi}
%          % \forall i \in \{1,\ldots,n\}, ~ 
%          B_i &= \max_{j = i:(i+n-1)} H_{i,j}, \;\;\; i = 1:n\\
%          \label{eq:Hij}
%         \forall j \geq i, H_{i,j} &= (j - i + 1)l - \ltot(T_j - T_i)
%     \end{align}
%     %     \forall i \in \{1,2,\ldots, n\}, ~ B_i = \max_{j = i:(i+n-1)} \lc (j - i + 1)l - \ltot(T_j - T_i) \rc

%     %     \forall j \geq i, H_{i,j} = (j - i + 1)l - \ltot(T_j - T_i)
%     % \end{equation}
%     As flows are packetized, points of interest are the arrival times of packets, and thus $\max_{t\geq 0}B(t) = \max_{1 \leq j}B(T_j)$ and $B(T_j) = \max_{i=1:j} \lc A(T_i, T_j] - \ltot(T_j - T_i) \rc$. Also, observe that $A(T_i, T_j] = (j - i + 1)l$ as in time interval $(T_i, T_j]$, $(j-i + 1)$ packets of size $l$ are arrived in the aggregate traffic. Hence
%     \begin{equation} \label{eq:s1}
%         B = \max_{1 \leq j} \max_{i=1:j } H_{i,j} 
%     \end{equation}
%     As flows are periodic with a period equal to $1$, we have $T_{j + n} = T_j + 1$ for $j\geq 1$; also, recall that $\ltot = nl$. Then, it follows that $H_{i,j+n} = H_{i,j}$ for $i\leq j$ and $H_{i+n,j} = H_{i,j}$ if $i + n\leq j$. Hence,
%     \begin{equation}
%         \underbrace{\max_{1 \leq j} \max_{i=1:j } H_{i,j}}_{B} =  \max_{i=1:n} \underbrace{\max_{j = i:(i+n-1)} H_{i,j}}_{B_i}
%     \end{equation}
%     which concludes \eqref{eq:s2}.

%     \textbf{Step 2 (iid Phases)}:  Let $U_1, ..., U_{n-1}$ be a sequence of $n-1$ independent and identically distributed (iid) standard uniform random variables, and $U_{(1)},...,U_{(n-1)}$ be the corresponding order statistic. We prove the following:
%     \begin{align} \label{eq:BiT}
%         % \forall i \in \{1,\ldots,n\}, 
%         \lc B_i \leq b \rc = \bigcap_{k = 1}^{n-1} \lc U_{(k)} \geq \frac{ \lb (k + 1)l - b \rb^+}{\ltot} \rc, \;\;\; i = 1:n
%     \end{align}


%      Fix $i$. Observe that $\lc B_i \leq b \rc $ can be rewritten as follows: 
%       \begin{align} \label{eq:s21}
%         \lc B_i \leq b \rc = \bigcap_{j = i}^{i + n -1} \lc (T_j - T_i) \geq \frac{(j - i + 1)l - b}{\ltot} \rc
%     \end{align}

%      Let us denote $\phi_{(1)} \leq \phi_{(2)} \leq \ldots \leq \phi_{(n)}$ the ordered sequence of phases. As $i \leq n$, it follows that $T_i = \phi_{(i)}$. Second, observe that 
%     \begin{equation} \label{eq:T}
%         \forall j \neq i, T_j - T_i = T_j - \phi_{(i)} = \lp \phi_{(j)} - \phi_{(i)}\rp 1_{ \phi_{(j)}  \geq  \phi_{(i)} } +   \lp 1 + \phi_{(j)} - \phi_{(i)}\rp 1_{ \phi_{(j)}  <  \phi_{(i)} } 
%     \end{equation}
%     As phases $\phi$ are independently and  uniformly distributed in $[0,1]$, it follows that, given $\phi_{(i)}$, the right-hand side of \eqref{eq:T} are $n-1$ iid standard uniform random variables that are ordered, hence we replace them by $U_{(1)},...,U_{(n-1)}$; combining this with \eqref{eq:s21} we have
%     \begin{align} \label{eq:BiPhi}
%         \lc B_i \leq b \giventhat \phi_{(i)}\rc = \bigcap_{k = 1}^{n-1} \lc U_{(k)} \geq \frac{(k + 1)l - b}{\ltot} \rc
%     \end{align}
%     As $\phi_{(i)}$ is a standard uniform random variable, we have $ \P\lp B_i \leq b \rp = \P\lp B_i \leq b \giventhat \phi_{(i)}\rp \P\lp\phi_{(i)}\rp =  \P\lp B_i \leq b \giventhat \phi_{(i)}\rp$; also, $U_{(k)} \geq 0$ for $k = 1:n-1$
%     % $k \in \{1,\ldots,n-1\}$
%     . Combine these with \eqref{eq:BiPhi} to conclude \eqref{eq:BiT}.

%     \textbf{Step 3 (Order Statistics)}:  We show that following:
%     \begin{equation} \label{eq:order}
%         \P \lp \bigcap_{k = 1}^{n-1} \lc U_{(k)} \geq \frac{\lb (k + 1)l - b \rb^+}{\ltot} \rc \rp = p(n,l,b)
%     \end{equation}
%     The density function of the distribution of $U_{(1)},...,U_{(n-1)}$ is \cite[Equation 1.145]{gentle2009computational}
%     \begin{equation}
%         f_{U_{(1)},...,U_{(n-1)}}\lp y_{1},...,y_{n-1} \rp  = (n-1)!\prod_{k=1}^{n-1}f_{U}(y_{k})\ind{y_{1}\leq y_2 \leq  \ldots \leq y_{n-1}}
%     \end{equation}
%     where $f_U$ is the probability density function of a standard uniform; as $y_{k} \in [0,1]$, $f_{U}(y_{k}) = 1$ for $k = 1:n-1$
%     % $k \in \{1,\ldots,n-1\}$
%     . Hence,
%     \begin{equation}
%         f_{U_{(1)},...,U_{(n-1)}}\lp y_{1},...,y_{n-1} \rp  = (n-1)!\ind{y_{1}\leq y_2 \leq  \ldots \leq y_{n-1}}
%     \end{equation}
%     The probability of the left-hand side of \eqref{eq:order} is equal to the probability that  $k = 1:n-1, U_{(k)} \geq \frac{(k + 1)l - b}{\ltot} = u_k$, hence $ \P \lp \bigcap_{k = 1}^{n-1} \lc U_{(k)} \geq \frac{\lb (k + 1)l - b \rb^+}{\ltot} \rc \rp = $
%     \begin{align}
%         &\int_{y_{n-1} = u_{n-1}}^{1} \ldots \int_{y_{i} = u_{i}}^{1} \ldots \int_{y_{1} = u_{1}}^{1} f_{U_{(1)},...,U_{(n-1)}}\lp y_{1},...,y_{n-1} \rp    \,dy_1 \ldots \,dy_{n-1} \\
%         &=\int_{y_{n-1} = u_{n-1}}^{1} \ldots \int_{y_{i} = u_{i}}^{1} \ldots \int_{y_{1} = u_{1}}^{1} (n-1)!\ind{y_{1}\leq y_2 \leq  \ldots \leq y_{n-1}}   \,dy_1 \ldots \,dy_{n-1} \\
%         &=(n-1)!\int_{y_{n-1} = u_{n-1}}^{1}  \ldots \int_{y_{i} = u_{i}}^{y_{i+1}} \ldots \int_{y_{1} = u_{1}}^{y_{2}} 1   \,dy_1 \ldots \,dy_{n-1} = p(n,l,b) 
%         % \\
%         % &= p(n,l,b)
%     \end{align}

%     \textbf{Final Step (Union Bound)}: We proceed to prove the theorem. By Step 1, 
%     % It follows that
%     \begin{equation} \label{eq:s41}
%        \lc B > b \rc  = \bigcup_{i=1}^n \lc B_i > b \rc \Rightarrow \P \lp B > b \rp  = \sum_{i=1}^n \P \lp B_i > b \rp
%     \end{equation}
%     % \begin{equation} \label{eq:s41}
%     %    \P \lp B > b \rp  = \bigcup_{i=1}^n \P \lp B_i > b \rp 
%     % \end{equation}
%     Combining Step 2 and Step 3, we have 
%     \begin{equation}\label{eq:s42}
%        % \forall i \in \{1,\ldots,n\}, 
%        \P \lp B_i > b \rp  = 1 -  p(n,l,b), \;\;\; i = 1:n
%     \end{equation}
%     Combining \eqref{eq:s41} and \eqref{eq:s42} we have 
%     \begin{equation} \label{eq:s43}
%        \P \lp B > b \rp  = n\P \lp B_i > b \rp =  n\lp 1 -  p(n,l,b)\rp 
%     \end{equation}
%     which concludes  the theorem. \qed
% \end{proof}


% % Define the mapping $\Pi: \lp \lp q_1^m, \ldots, q_m^m \rp , u_{m+1} \rp   \mapsto \lp q_1^{m+1}, \ldots, q_{m+1}^{m+1} \rp $  for $ m \in \{ \lfloor b \rfloor - 1, \lfloor b \rfloor, \ldots, n-2\}$ as follows:
% % \begin{equation}
% %     q_i^{m+1} =  \begin{cases} 
% %          -\sum_{j=0}^m \frac{(m+1)q_j^m}{j+1}u_{m+1}^{j+1}& \text{if } i  =0\\
        
% %         \frac{(m+1)q_i^m}{i+1} & \text{if } 1 \leq i \leq m \\
% %          1 & \text{if } i = m+1 \\
% %     \end{cases}
% % \end{equation}

% % First, compared to simulations, the bound of Theorem~\ref{thm:homog} is fairly tight (see nig. ??). Second, for a small, non-zero violation probability, say $10^{-7}$), we obtain a considerably smaller quasi-deterministic burstiness bound $b$ compared to the deterministic one, $\ltot$ (see Fig. ??). Thus, if we apply deterministic network calculus using $\gamma_{\rtot,b}$ rather than $\gamma_{\rtot,\ltot}$ as an arrival curve for the aggregate flow, we obtain bounds that are significantly smaller than the deterministic bound (almost $\frac{b}{\ltot}$ times smaller); moreover, they are very unlikely to be violated with the violation probability of at most $\ep(F,b)$.
% % Note that $\ep(F,b)$ is independent of the value of the period $\tau$ and packet size $l$ and only depends on $b$ and the number of flows $F$. As shown numerically in Section~\ref{sec:num}, compared to simulations, the bound of Theorem~\ref{thm:homog} is fairly tight.
% % $sup_{t \geq 0}B(t)$, where $B(t)$ is the aggregate burstiness at time $t$. First, flows are packetized hence $sup_{t \geq 0}B(t)$ can be reduced to only values of $B(t)$ at arrival times of packets: Let us denote by  $T_i$ the arrival time of the $i$-th packet in the aggregate traffic; thus, $sup_{t \geq 0}B(t) = sup_{i \geq 1}B(T_i)$. Second, as flows are periodic, we have $T_{i+F} = T_i + \tau$, and thus $sup_{i \geq 1}B(T_i) = \sup_{i=1:2F}B(T_i)$.
% % \hossein{To be put in the appendix}
% % We now explain how to concretely compute the bound of Theorem~\ref{thm:homog}: Observe that $p(F,b)$ in \eqref{eq:pbThm1} is a series of polynomials integration, and thus giving a general close-form formula for it might be challenging. Here, we explain how to compute it efficiently and iteratively. Define $Q_m = \sum_{i = 0}^mq_i^mx^i$, a polynomial of degree $m$ for $m \in \{ 0,1, \ldots,n-1\}$, as follows:
% % \begin{equation}
% %     Q_0(x) = 1 \mand Q_{m+1}(x) = (m+1)\int_{y = u_{m+1}}^x Q_{m}(y)\,dy~ \textrm{for}~ 0 \leq m \leq n-2 
% % \end{equation}
% % Observe that $Q_m(y_{m+1}) = m!\int_{y_{m} = u_{m}}^{y_{m+1}} \ldots \int_{y_{1} = u_{1}}^{y_{2}} 1   \,dy_1 \ldots \,dy_{m} $ and $p(F,b) = Q_{n-1}(1)$. As  $u_m = 0$ for $1 \leq m < \lfloor b \rfloor$ and by the construction of $Q$, it follows that
% % \begin{equation}
% %     \begin{cases}
% %         &\text{If}~ 0 \leq m < \lfloor b \rfloor ,~ q_i^m =  \begin{cases} 
% %                                                                  1 & \text{if } i = m \\
% %                                                                   0 & \text{otherwise}                              \end{cases}
% %         \\
% %         &\text{Else if}~ \lfloor b \rfloor - 1 \leq m \leq n-2,~ q_i^{m+1} =\begin{cases} 
% %                                                                                     -\sum_{j=0}^m \frac{(m+1)q_j^m}{j+1}u_{m+1}^{j+1}& \text{if } i  =0\\
        
% %                                                                                   \frac{(m+1)q_i^m}{i+1} & \text{if } 1 \leq i \leq m \\
% %                                                                                   1 & \text{if } i = m+1 \\
% %                                                                                                           \end{cases}
% %     \end{cases}
% % \end{equation}
% % Hence, for $1 \leq m < \lfloor b \rfloor$, $Q_m(x) = x^m$, and for $\lfloor b \rfloor - 1\leq m \leq n-2$, we have a mapping that derive coefficients of the polynomial $Q_{m+1}(x)$  given coefficients of the polynomial $Q_{m}(x)$  and $u_{m+1}$, i.e., given $ \lp  \lp q_0^{m},q_1^{m}, \ldots,q_{m}^{m} \rp , u_{m+1} \rp$ computes $\lp q_0^{m+1},q_1^{m+1}, \ldots,q_{m+1}^{m+1} \rp $. As mentioned above, $p(F,b) = Q_{n-1}(1) = \sum_{i=0}^{n-1} q_i^{n-1}$ and as $q_{n-1}^{n-1} = 1$, we have
% % \begin{equation}
% %     1 - p(F,b) = 1 - Q_{n-1}(1) = \sum_{i=0}^{n-2} q_i^{n-1}
% % \end{equation}
% % which is the value of interest in \eqref{eq:epsThm1}.
% % Note that all computations can be done using infinite precision arithmetic (with rational numbers), e.g., using symbolic numbers in MATLAB. Although working with symbolic numbers in MATLAB can be costly, we managed to compute the bound of Theorem~\ref{thm:homog} for large $F$ (e.g., $F = 3000$) in a feasible time on a $2.6$ GHz $6$-Core Intel Core i$7$ computer. To mitigate the run-time and memory complexity, in the following theorem, we provide a closed-form expression that upper bounds the bound of Theorem~\ref{thm:homog}.
% % Let $P_m(x) = \sum_{i = 0}^ma_i^mx^i$. It follows that
% % \begin{equation}
% %     \begin{cases}
% %         &\text{if}~ 0 \leq m < \lfloor b \rfloor ,~ a_i^m =  \begin{cases} 
% %                                                                  \frac{1}{m!} & \text{if } i = m \\
% %                                                                   0 & \text{otherwise}                              \end{cases}
% %         \\
% %         &\text{Else if}~ \lfloor b \rfloor - 1 \leq m \leq n-2,~ a_i^{m+1} =\begin{cases} 
% %                                                                                     -\sum_{j=0}^m \frac{a_j^m}{j+1}u_{m+1}^{j+1}& \text{if } i  =0\\
        
% %                                                                                   \frac{a_i^m}{i+1} & \text{if } 1 \leq i \leq m \\
% %                                                                                   \frac{1}{(m+1)!} & \text{if } i = m+1 \\
% %                                                                                                           \end{cases}
% %     \end{cases}
% % \end{equation}
% % Hence, when for $1 \leq m \leq \lfloor b \rfloor$ (as $u_m = 0$) $P_m(x) = \frac{1}{m!}x^m$, and for $\lfloor b \rfloor - 1 \leq m \leq n-2$, we have a mapping that derive coefficients of the polynomial $P_{m+1}(x)$ (resp. $Q_{m+1}(x)$) given coefficients of the polynomial $P_{m}(x)$ (resp. $Q_{m}(x)$) and $u_{m+1}$, i.e., given $ \lp  \lp a_0^{m},a_1^{m}, \ldots,a_{m}^{m} \rp , u_{m+1} \rp$ computes $\lp a_0^{m+1},a_1^{m+1}, \ldots,a_{m+1}^{m+1} \rp $.
% % Let us denote by $T_i$ and $L_i$ the arrival time and packet size of the $i$-th packet in the aggregate traffic. As flows are packetized for all $i \geq 1$, at time $T_i$, $\sum_{k=1}^iL_j$ bits are arrived in the aggregate traffic. Then, the aggregate burstiness $B(t)$ in \eqref{eq:agg_burst} can be rewritten as follows:
% % \begin{equation} \label{eq:agg_burst_packetized}
% %     B(t) = \sup_{i \leq j} \{ \sum_{k=i}^jL_k - \rtot(T_j - T_i) \}
% % \end{equation}
% % As flows are periodic, we have $T_{i+F} = T_i + \tau$, hence it follows that 
% % \begin{equation} \label{eq:agg_burst_periodic}
% %     B(t) = \sup_{i \leq j \leq 2F} \{ \sum_{k=i}^jL_k - \rtot(T_j - T_i) \}
% % \end{equation}
% % Which is equivalent to 
% % \begin{align} \label{eq:agg_burst_periodic}
% %     B(t) &= \max_{i=1:F}B_i
% % \end{align}

% % and periodic. Let us denote by $T_i$ and $L_i$ the arrival time and packet size of the $i$-th packet in the aggregate traffic. Then, for all $i \geq 1$, We have $A(T_i) = \sum_{k=1}^iL_j$. Then, \eqref{eq:agg_burst} can be rewritten as follows:
% % \begin{equation} \label{eq:agg_burst_period}
% %     B(t) = \sup_{i \leq j} \{ \sum_{k=i}^jL_k - \rtot(T_j - T_i) \}
% % \end{equation}


% % \subsection{Computation of the Bound of Theorem~\ref{thm:homog}}

% % Observe that $p(F,b)$ in \eqref{eq:pb} is a series of polynomials integration, and thus giving a general close-form formula for it might be challenging. Here, we want to compute it iteratively. Define $P_m$ and $Q_m$, polynomials of degree $m$, as follows:
% % \begin{align}
% %     P_0(x) &= 1 \mand P_{m+1}(x) = \int_{y = u_{m+1}}^x P_{m}(y)\,dy~ \textrm{for}~ 0 \leq m \leq n-2 \\
% %     Q_m(x) &= m!P_m(x)~ \textrm{for}~ 0 \leq m \leq n-1
% % \end{align}
% % Observe that $P_m(y_{m+1}) = \int_{y_{m} = u_{m}}^{y_{m+1}} \ldots \int_{y_{1} = u_{1}}^{y_{2}} 1   \,dy_1 \ldots \,dy_{m} $ and $p(F,b) = Q_{n-1}(1)$.

% % Let $P_m(x) = \sum_{i = 0}^ma_i^mx^i$. It follows that
% % \begin{equation}
% %     \begin{cases}
% %         &\text{if}~ 0 \leq m < \lfloor b \rfloor ,~ a_i^m =  \begin{cases} 
% %                                                                  \frac{1}{m!} & \text{if } i = m \\
% %                                                                   0 & \text{otherwise}                              \end{cases}
% %         \\
% %         &\text{Else if}~ \lfloor b \rfloor - 1 \leq m \leq n-2,~ a_i^{m+1} =\begin{cases} 
% %                                                                                     -\sum_{j=0}^m \frac{a_j^m}{j+1}u_{m+1}^{j+1}& \text{if } i  =0\\
        
% %                                                                                   \frac{a_i^m}{i+1} & \text{if } 1 \leq i \leq m \\
% %                                                                                   \frac{1}{(m+1)!} & \text{if } i = m+1 \\
% %                                                                                                           \end{cases}
% %     \end{cases}
% % \end{equation}
% % Hence, when for $1 \leq m \leq \lfloor b \rfloor$ (as $u_m = 0$) $P_m(x) = x^m$, and for $\lfloor b \rfloor - 1 \leq m \leq n-2$, we have a mapping that dervie coefficients of the polynomial $P_{m+1}(x)$ (resp. $Q_{m+1}(x)$) given coefficients of the polynomial $P_{m}(x)$ (resp. $Q_{m}(x)$) and $u_{m+1}$, i.e., given $ \lp  \lp a_0^{m},a_1^{m}, \ldots,a_{m}^{m} \rp , u_{m+1} \rp$ computes $\lp a_0^{m+1},a_1^{m+1}, \ldots,a_{m+1}^{m+1} \rp $.
% % \subsection{Closed-Form, Dvoretzky–Kiefer–Wolfowitz (DKW) Bound}
% Note that all computations of Algorithm~\ref{alg:thm1} can be done using infinite precision arithmetic (with rational numbers), e.g., using symbolic numbers in MATLAB. Although working with symbolic numbers in MATLAB can be costly, we managed to compute the bound of Theorem~\ref{thm:homog} for large $n$ (e.g., $n = 3000$) in a feasible time on a $2.6$ GHz $6$-Core Intel Core i$7$ computer. To mitigate the run-time and memory complexity, in the following theorem, we provide a closed-form expression that upper bounds the bound of Theorem~\ref{thm:homog} and is tight when the number of flows $n$ is large.


% \begin{theorem}[Closed-Form, DKW Bound] \label{thm:homog_dkw}
% Assume the assumptions of Theorem~\ref{thm:homog}. Also, consider some $b$, and let $B = \frac{ b}{l}$ such that $ \lfloorB \rfloor\geq 1-\frac1n +\sqrt{\frac{(n-1)\log 2}{2}}$. Then, 
% \begin{equation}\label{eq:epsdkw}
%      \P\lp B > b\rp \leq n\exp{\lp-2(n-1)\lp \frac{\lfloor\Bar{b} \rfloor}{n-1} - \frac{1}{n}\rp^2 \rp} = \epdkw(n,l,b)
% \end{equation}
% Also,  $\epdkw(n,l,b) \geq \ep(n,l,b)$ where $\ep(n,l,b)$ is the bound of Theorem~\ref{thm:homog}.
% \end{theorem}

% Theorem~\ref{thm:homog_dkw} gives a closed-form upper-bound to Theorem~\ref{thm:homog}, and moreover, is obtained using Dvoretzky–Kiefer–Wolfowitz (DKW) inequality which is known to be tight when the number of flows $n$ is large \cite{dkw}. Hence, Theorem~\ref{thm:homog_dkw} has all the properties explained after Theorem~\ref{thm:homog}. 
% % We also numerically confirm its tightness (see Fig.~ ??).

% \begin{proof}
%     Recall that $U_1, ..., U_{n-1}$ are a sequence of $n-1$ iid standard uniform random variables and $U_{(1)},...,U_{(n-1)}$ the corresponding order statistic, and  from \eqref{eq:s43} and \eqref{eq:BiT} that   
%     \begin{equation}
%      \P\lp B> b\rp \leq n \P\lp E \rp
%     \label{eq-wegrhj}
%     \end{equation}
%     with 
% \begin{equation}
%    E = \bigcup_{k=\lfloor b\rfloor}^{n-1} 
%    \lc U_{(k)} < \frac{(k+1)l-b}{\ltot}\rc  = \bigcup_{k=\lfloor b\rfloor}^{n-1} 
%    \lc U_{(k)} < \frac{(k+1)-\Bar{b}}{n}\rc 
% \end{equation}
% % where $\Bar{b} = \frac{b}{l}$.
    

%   \textbf{Step 1 (Dvoretzky–Kiefer–Wolfowitz inequality):} We show the following:
%   \begin{equation} 
%      \P(E')\leq e^{-2(n-1)\varepsilon^2} \mif \varepsilon \geq \sqrt{\frac{\log 2}{2(n-1)}}
%      \label{eq:s1DKW}
%  \end{equation} 
%  with 
%   \begin{equation} \label{eq:Eprime}
%    E' = \bigcup_{k=1}^{n-1} 
%    \lc U_{(k)} < \frac{k}{n-1}-\varepsilon\rc  
% \end{equation}
% Let $F_{n-1}$ be the (random) empirical cumulative distribution function of $U_1,...,U_{n-1}$, defined by
% \begin{equation}
%      F_{n-1}(x)=\frac{1}{n-1}\sum_{i=1}^{n-1}\ind{U_{(i)}\leq x}
%  \end{equation} 
% The Dvoretzky–Kiefer–Wolfowitz inequality \cite{massart1990tight} states that
% \begin{equation}
%      \P\lp \sup_{x\in[0,~1]} (F_{n-1}(x)-x)>\varepsilon  \rp\leq e^{-2(n-1)\varepsilon^2} \mif \varepsilon \geq \sqrt{\frac{\log 2}{2(n-1)}}
%      \label{eq-wpjgrt}
%  \end{equation} 
%  We can apply this to find the bound of interest. First, note that 
%  \begin{equation} \label{hgqewd}
%      \lp\sup_{x\in[0,~1]} (F_{n-1}(x)-x)>\varepsilon\rp 
%      \Leftrightarrow
%      \lp\exists k\in \lc 1,..., n-1\rc, U_{(k)}<\frac{k}{n-1}-\varepsilon\rp
%  \end{equation}
%  This is obtained by observing that if the inequality $F_{n-1}(x)-x>\varepsilon$ occurs for some $x$, then it must occur for $x=U_{(k)}$ for some $k$. Combine the DKW inequality \eqref{eq-wpjgrt} and \eqref{hgqewd} to conclude \eqref{eq:s1DKW}.


%  \textbf{Step 2 (Appropriate Choice of $\varepsilon$):} We show that the largest possible $\varepsilon$ such that $E\subseteq E'$ is 
%  \begin{equation} \label{eq:eps}
%     \varepsilon = \frac{\lfloor \bar{b}\rfloor}{n-1}-\frac{1}{n}
% \end{equation}
%  We bound $E$ by $E'$ for an appropriate $\varepsilon$. Observe that if
% \begin{equation}
%     \frac{k+1-\bar{b}}{n}\leq \frac{k}{n-1}-\varepsilon,\;\;\;\forall k \in\lc\lfloor \bar{b}\rfloor,...,n-1\rc
% \end{equation}
% then $E\subseteq E'$. We are looking for $\varepsilon$ that satisfies 
% \begin{equation}
%     \varepsilon\leq \frac{k}{n-1}-\frac{k+1-\bar{b}}{n},\;\;\;\forall k \in\lc\lfloor \bar{b}\rfloor,...,n-1\rc
% \label{eq-dfksjn}
% \end{equation}
% The minimum over $k$ of the right-handside is obtained for $k=\lfloor \bar{b}\rfloor$, therefore \eqref{eq-dfksjn} is equivalent to 
% \begin{equation}
%     \varepsilon\leq \frac{\lfloor \bar{b}\rfloor}{n-1}-\frac{\lfloor \bar{b}\rfloor+1-\bar{b}}{n}
% \end{equation}
% and as $\bar{b}-\lfloor \bar{b}\rfloor\geq 0$, conclude \eqref{eq:eps}.

% \textbf{Final Step:}
% For the value of $\varepsilon $ at Step 2, we have $E\subseteq E'$ and thus, combining \eqref{eq-wegrhj}, \eqref{eq:s1DKW}, and \eqref{eq:eps} we obtain

% \begin{equation}
%     \P\lp \Bar{B} > b\rp \leq n \exp{\lp-2(n-1) \lp\frac{\lfloor \Bar{b}\rfloor}{n-1}-\frac{1}{n}\rp^2\rp}
%     \label{eq-jhwdef}
% \end{equation}
% provided that $\varepsilon \geq \sqrt{\frac{\log 2}{2(n-1)}}$, i.e., provided that
% \begin{equation}
%     % \lp \frac{\lfloor b\rfloor}{n-1}-\frac{1}{n}\rp^2\geq \frac{\log 2}{n-1}
%      \lfloor \Bar{b}\rfloor \geq 1-\frac1n +\sqrt{\frac{\log 2}{2}}\sqrt{n-1}
%      \label{eq-ghefq}
% \end{equation}
% which concludes the theorem. \qed
% \end{proof}
% % Theorem~\ref{thm:homog_dkw} gives a closed-form upper-bound to Theorem~\ref{thm:homog}, and moreover, is obtained using Dvoretzky–Kiefer–Wolfowitz (DKW) inequality which is known to be tight when the number of flows $n$ is large \cite{dkw}. Hence, Theorem~\ref{thm:homog_dkw} has all the properties explained after Theorem~\ref{thm:homog}. We also numerically confirm its tightness (see Fig.~ ??). 
% Furthermore, the following corollary provides a closed-form formulation for the minimum value for the aggregate burstiness with a violation probability of at most $\varepsilon$.

% \begin{corollary}[Estimated Quasi-Deterministic Burstiness in Closed-form] \label{cor:homog_burst}
% Assume the assumptions of Theorem~\ref{thm:homog}. Consider some $\varepsilon > 0$, and compute $b(n,l, \varepsilon)$ as follow:
% \begin{equation}
%     b(n,l, \varepsilon) = l\lp 1 -\frac1n+\sqrt{\frac{(n-1)(\log n-\log\varepsilon)}{2}}\rp
% \end{equation}
% Then, $b(n,l, \varepsilon)$ is a quasi-deterministic burstiness bound for the aggregate with the violation probability of at most $\varepsilon$, i.e., $\P\lp \exists t \geq 0,~ B(t) > b(n,l, \varepsilon)\rp \leq \varepsilon$.
% % \begin{equation}
% %      \P\lp \exists t \geq 0,~ B(t) > b_F^\epsilon\rp \leq \epsilon
% % \end{equation}
% \end{corollary}

% Corollary~\ref{cor:homog_burst} is obtained by setting the right-hand side of \eqref{eq:epsdkw} in Theorem~\ref{thm:homog_dkw} to $\varepsilon$, i.e., by finding the smallest $b$ such that $\epdkw(n,l,b) \leq \varepsilon$. $b(n, l,\varepsilon)$ is a quasi-deterministic bound, and it grows in $\sqrt{n\log{n}}$ as opposed to the deterministic bound that grows in $n$, where $n$ is the number of flows, i.e., the ratio $\frac{b(n, l,\varepsilon)}{\ltot}$ is in the order of $\sqrt{\frac{\log{n}}{n}}$ (see Fig. ??).
% % We also numerically confirm that, given a non-zero violation probability, $b(n, l,\epsilon)$ is tight compared to the burstiness obtained by Theorem~\ref{thm:homog} (see Fig. ??). 

% % \subsection{Flows with Same Period but Different Packet-size} \label{sec:semi-homogen}

% % We extend the results obtained in Section~\ref{sec:homogen} to when flows have the same Period but different packet sizes.
% % \begin{theorem}[Flows with Same Period but Different Packet-size] \label{thm:semi_homog}
% % Assume the assumptions of Section~\ref{sec:assump}, and also assume that flows have the same period, i.e., for every flow $f$, $\tau_f = \tau$ for some $\tau > 0$. Let $l_{(1)} \geq l_{(2)} \geq \ldots \geq l_{(n)}$ be the ordered sequence of packet-sizes and consider some $b$. 

% % \begin{enumerate}
% %     \item Compute $\bar{p}(n,l_{(1)}, l_{(2)},\ldots ,l_{(n)},b)$ as \eqref{eq:pbThm1} by replacing $u_1, u_2, \ldots,u_{n-1}$ by $\bar{u}_1, \bar{u}_2, \ldots,\bar{u}_{n-1}$ where $\bar{u}_k = \frac{[ \sum_{j=1}^{k+1}l_{(j)} - b]^+}{\ltot},~ k =1:n-1$. Then,
% %     \begin{equation}
% %         \P\lp \exists t \geq 0,~ B(t) > b\rp \leq n(1 - \bar{p}(n,l_{(1)}, l_{(2)},\ldots ,l_{(n)},b)) 
% %         % = \epe(n,\Vec{l},b)
% %         % = \ep(n,l,b)
% %     \end{equation}
% %     % $\P\lp \exists t \geq 0,~ B(t) > b\rp \leq n(1 - \bar{p}(n,l,b)) = \ep(n,l,b)$ with $\bar{p}(n,l,b)$ is computed as \eqref{eq:pbThm1} when replacing $u_1, u_2, \ldots,u_{n-1}$ by $\bar{u}_1, \bar{u}_2, \ldots,\bar{u}_{n-1}$ where $\bar{u}_k = \frac{[ \sum_{j=1}^{k+1}l_{(j)} - b]^+}{\ltot}, \forall k \in \{1, \ldots, n-1 \}$.

% %     \item Let $\bar{k} = \argmin_{ k=1:n-1, \sum_{j=1}^{k+1}l_{(j)} > b}{ \lc  \frac{k}{n-1}-\frac{\sum_{j=1}^{k+1}l_{(j)}}{\ltot} \rc}$ and consider some $b \geq \ltot \lp \sqrt{\frac{\log 2}{2(n-1)}}  - \frac{\bar{k}}{n-1} + \frac{\sum_{j=1}^{\bar{k}+1}l_{(j)}}{\ltot}  \rp$, then, 
% % % \begin{equation}\label{eq:epsdkw}
% % %      \P\lp \exists t \geq 0,~ B(t) > b\rp \leq n \exp \lp -2(n-1) \lp \frac{\bar{k}}{n-1}-\frac{\Lcum(\bar{k}+1)-b}{\ltot} \rp^2 \rp  = \epdkw(n,l,b)
% % % \end{equation}
% % \begin{equation}\label{eq:epsdkw}
% %      \P\lp \exists t \geq 0,~ B(t) > b\rp \leq n \exp \lp -2(n-1) \lp \frac{\bar{k}}{n-1}-\frac{\sum_{j=1}^{k+1}l_{(j)}-b}{\ltot} \rp^2 \rp
% %      % = \epdkw(n,l,b)
% % \end{equation}
% % % where $\bar{k} = \argmin_{k\in\lc 1,2,\ldots,n-1\rc, \sum_{j=1}^{k+1}l_{(j)} > b}{ \lc  \frac{k}{n-1}-\frac{\sum_{j=1}^{k+1}l_{(j)}}{\ltot} \rc}$.

% % \item Consider some $\varepsilon > 0$, and compute $b(n,l_{(1)}, l_{(2)},\ldots ,l_{(n)}, \varepsilon)$ as follow:
% % \begin{equation}
% %     b(n,l_{(1)}, l_{(2)},\ldots ,l_{(n)}, \varepsilon) = \ltot \lp \sqrt{\frac{\log n - \log \varepsilon}{2(n-1)}}  - \frac{\bar{k}}{n-1} + \frac{\sum_{j=1}^{\bar{k}+1}l_{(j)}}{\ltot}  \rp 
% % \end{equation}
% % where $\bar{k}$ is defined in Item 2). Then, $b(n,l, \varepsilon)$ is a quasi-deterministic burstiness bound for the aggregate with the violation probability of at most $\varepsilon$, i.e., $\P\lp \exists t \geq 0,~ B(t) > b(n,l_{(1)}, l_{(2)},\ldots ,l_{(n)}, \varepsilon)\rp \leq \varepsilon$.
% % \end{enumerate}
% % % \textbf{Item 1):} $\P\lp \exists t \geq 0,~ B(t) > b\rp \leq n(1 - \bar{p}(n,l,b)) = \ep(n,l,b)$
% % % % \begin{equation} \label{eq:epsThm1}
% % % %      \P\lp \exists t \geq 0,~ B(t) > b\rp \leq n(1 - \bar{p}(n,l,b)) = \ep(n,l,b) 
% % % % \end{equation}
% % % with $\bar{p}(n,l,b)$ is computed as \eqref{eq:pbThm1} when replacing $u_1, u_2, \ldots,u_{n-1}$ by $\bar{u}_1, \bar{u}_2, \ldots,\bar{u}_{n-1}$ where $\bar{u}_k = \frac{[ \sum_{j=1}^{k+1}l_{(j)} - b]^+}{\ltot}, \forall k \in \{1, \ldots, n-1 \}$.
% % % % \begin{align}
% % % %     % \label{eq:pbThm1}
% % % %     % p(n,l,b) & = (n-1)!\int_{y_{n-1} = u_{n-1}}^{1} \int_{y_{n-2} = u_{n-2}}^{y_{n-1}} \ldots \int_{y_{i} = u_{i}}^{y_{i+1}} \ldots \int_{y_{1} = u_{1}}^{y_{2}} 1   \,dy_1 \ldots \,dy_{n-1} \\
% % % %     \label{eq:ukThm3}
% % % %     % p(b) & = (n-1)!\int_{y_{n-1} = u_{n-1}}^{1} \int_{y_{n-2} = u_{n-2}}^{y_{n-1}} \ldots \int_{y_{i} = u_{k}}^{y_{k+1}} \ldots \int_{y_{1} = u_{1}}^{y_{2}}    \,dy_1 \ldots \,dy_{n-1}
% % % %      \bar{u}_k &= \frac{[ \sum_{j=1}^{k+1}l_{(j)} - b]^+}{\ltot}, \forall k \in \{1, \ldots, n-1 \}
% % % % \end{align}
% % % % $B(t)$ is defined in \eqref{eq:agg_burst}, and in \eqref{eq:ukThm1}, we use the notation $[x]^+=\max\{x,0\}$ and $\ltot = nl$.

% % % \textbf{Item 2):} If $b \geq \ltot \lp \sqrt{\frac{\log 2}{2(n-1)}}  - \frac{\bar{k}}{n-1} + \frac{\sum_{j=1}^{\bar{k}+1}l_{(j)}}{\ltot}  \rp$, then, 
% % % % \begin{equation}\label{eq:epsdkw}
% % % %      \P\lp \exists t \geq 0,~ B(t) > b\rp \leq n \exp \lp -2(n-1) \lp \frac{\bar{k}}{n-1}-\frac{\Lcum(\bar{k}+1)-b}{\ltot} \rp^2 \rp  = \epdkw(n,l,b)
% % % % \end{equation}
% % % \begin{equation}\label{eq:epsdkw}
% % %      \P\lp \exists t \geq 0,~ B(t) > b\rp \leq n \exp \lp -2(n-1) \lp \frac{\bar{k}}{n-1}-\frac{\sum_{j=1}^{k+1}l_{(j)}-b}{\ltot} \rp^2 \rp  = \epdkw(n,l,b)
% % % \end{equation}
% % % where $\bar{k} = \argmin_{k\in\lc 1,2,\ldots,n-1\rc, \sum_{j=1}^{k+1}l_{(j)} > b}{ \lc  \frac{k}{n-1}-\frac{\sum_{j=1}^{k+1}l_{(j)}}{\ltot} \rc}$.
% % % % \begin{align}
% % % %     \label{eq:kbar}
% % % %     \bar{k} = \argmin_{k\in\lc 1,2,\ldots,n-1\rc, \sum_{j=1}^{k+1}l_{(j)} > b}{ \lc  \frac{k}{n-1}-\frac{\sum_{j=1}^{k+1}l_{(j)}}{\ltot} \rc}
% % % %     % k^* &= \min_{ k \in \lc 1,2,\ldots, n-1\rc}\lc  \sum_{j=1}^{\bar{k}+1}l_{(j)} > b \rc
% % % % \end{align}

% % % \textbf{Item 3):} Consider some $\varepsilon > 0$, and compute $b(n,l, \varepsilon)$ as follow:
% % % \begin{equation}
% % %     b(n,l, \varepsilon) = \ltot \lp \sqrt{\frac{\log n - \log \varepsilon}{2(n-1)}}  - \frac{\bar{k}}{n-1} + \frac{\sum_{j=1}^{\bar{k}+1}l_{(j)}}{\ltot}  \rp 
% % % \end{equation}
% % % where $\bar{k}$ is defined in Item 2). Then, $b(n,l, \varepsilon)$ is a quasi-deterministic burstiness bound for the aggregate with the violation probability of at most $\varepsilon$, i.e., $\P\lp \exists t \geq 0,~ B(t) > b(n,l, \varepsilon)\rp \leq \varepsilon$.
% % \end{theorem}



% % % \begin{theorem}[Flows with Same Period but Different Packet-size] \label{thm:semi_homog}
% % % Assume the assumptions of Section~\ref{sec:assump}, and also assume that flows have the same period, i.e., for every flow $f$, $\tau_f = \tau$ for some $\tau > 0$. Let $l_{(1)} \geq l_{(2)} \geq \ldots \geq l_{(n)}$ be the ordered sequence of packet-sizes and consider some $b$. Then,
% % % Item 1):
% % % \begin{equation} \label{eq:epsThm1}
% % %      \P\lp \exists t \geq 0,~ B(t) > b\rp \leq n(1 - \bar{p}(n,l,b)) = \ep(n,l,b) 
% % % \end{equation}
% % % with $\bar{p}(n,l,b)$ is computed as \eqref{eq:pbThm1} when replacing $u_1, u_2, \ldots,u_{n-1}$ by $\bar{u}_1, \bar{u}_2, \ldots,\bar{u}_{n-1}$ where
% % % \begin{align}
% % %     % \label{eq:pbThm1}
% % %     % p(n,l,b) & = (n-1)!\int_{y_{n-1} = u_{n-1}}^{1} \int_{y_{n-2} = u_{n-2}}^{y_{n-1}} \ldots \int_{y_{i} = u_{i}}^{y_{i+1}} \ldots \int_{y_{1} = u_{1}}^{y_{2}} 1   \,dy_1 \ldots \,dy_{n-1} \\
% % %     \label{eq:ukThm3}
% % %     % p(b) & = (n-1)!\int_{y_{n-1} = u_{n-1}}^{1} \int_{y_{n-2} = u_{n-2}}^{y_{n-1}} \ldots \int_{y_{i} = u_{k}}^{y_{k+1}} \ldots \int_{y_{1} = u_{1}}^{y_{2}}    \,dy_1 \ldots \,dy_{n-1}
% % %      \bar{u}_k &= \frac{[ \sum_{j=1}^{k+1}l_{(j)} - b]^+}{\ltot}, \forall k \in \{1, \ldots, n-1 \}
% % % \end{align}
% % % % $B(t)$ is defined in \eqref{eq:agg_burst}, and in \eqref{eq:ukThm1}, we use the notation $[x]^+=\max\{x,0\}$ and $\ltot = nl$.


% % % \end{theorem}

% % % \begin{theorem}[Closed-Form, DKW Bound] \label{thm:semi_homog_dkw}
% % % Assume the assumptions of Theorem~\ref{thm:semi_homog}. Also, consider some $b$ such that $b \geq \ltot \lp \sqrt{\frac{\log 2}{2(n-1)}}  - \frac{\bar{k}}{n-1} + \frac{\sum_{j=1}^{\bar{k}+1}l_{(j)}}{\ltot}  \rp$. Then, 
% % % % \begin{equation}\label{eq:epsdkw}
% % % %      \P\lp \exists t \geq 0,~ B(t) > b\rp \leq n \exp \lp -2(n-1) \lp \frac{\bar{k}}{n-1}-\frac{\Lcum(\bar{k}+1)-b}{\ltot} \rp^2 \rp  = \epdkw(n,l,b)
% % % % \end{equation}
% % % \begin{equation}\label{eq:epsdkw}
% % %      \P\lp \exists t \geq 0,~ B(t) > b\rp \leq n \exp \lp -2(n-1) \lp \frac{\bar{k}}{n-1}-\frac{\sum_{j=1}^{k+1}l_{(j)}-b}{\ltot} \rp^2 \rp  = \epdkw(n,l,b)
% % % \end{equation}
% % % where
% % % \begin{align}
% % %     \label{eq:kbar}
% % %     \bar{k} = \argmin_{k\in\lc 1,2,\ldots,n-1\rc, \sum_{j=1}^{k+1}l_{(j)} > b}{ \lc  \frac{k}{n-1}-\frac{\sum_{j=1}^{k+1}l_{(j)}}{\ltot} \rc}
% % %     % k^* &= \min_{ k \in \lc 1,2,\ldots, n-1\rc}\lc  \sum_{j=1}^{\bar{k}+1}l_{(j)} > b \rc
% % % \end{align}
% % % % \begin{align}
% % % %     \label{eq:kbar}
% % % %     \bar{k} = \argmin_{k\in\lc k^*,...,n-1\rc}{ \lc  \frac{k}{n-1}-\frac{\sum_{j=1}^{\bar{k}+1}l_{(j)}}{\ltot} \rc } \mand k^* = \min_{ k \in \lc 1,2,\ldots, n-1\rc}\lc  \sum_{j=1}^{\bar{k}+1}l_{(j)} > b \rc
% % % %     % k^* &= \min_{ k \in \lc 1,2,\ldots, n-1\rc}\lc  \sum_{j=1}^{\bar{k}+1}l_{(j)} > b \rc
% % % % \end{align}
% % % Also,  $\epdkw(n,l,b) \geq \ep(n,l,b)$ where $\ep(n,l,b)$ is the bound of Theorem~\ref{thm:homog}.
% % % \end{theorem}

% % % \begin{corollary}[Estimated Quasi-Deterministic Burstiness in Closed-form] \label{cor:semi_homog_burst}
% % % Assume the assumptions of Theorem~\ref{thm:semi_homog}. Consider some $\varepsilon > 0$, and compute $b(n,l, \varepsilon)$ as follow:
% % % \begin{equation}
% % %     b(n,l, \varepsilon) = \ltot \lp \sqrt{\frac{\log n - \log \varepsilon}{2(n-1)}}  - \frac{\bar{k}}{n-1} + \frac{\sum_{j=1}^{\bar{k}+1}l_{(j)}}{\ltot}  \rp 
% % % \end{equation}
% % % where $bar{k}$ is defined in \eqref{eq:kbar}. Then, $b(n,l, \varepsilon)$ is a quasi-deterministic burstiness bound for the aggregate with the violation probability of at most $\varepsilon$, i.e., $\P\lp \exists t \geq 0,~ B(t) > b(n,l, \varepsilon)\rp \leq \varepsilon$.
% % % % \begin{equation}
% % % %      \P\lp \exists t \geq 0,~ B(t) > b_F^\epsilon\rp \leq \epsilon
% % % % \end{equation}
% % % \end{corollary}
% %  Theorem~\ref{thm:semi_homog} is the extension of the results presented in Theorem~\ref{thm:homog}, Theorem~\ref{thm:homog_dkw}, and Corollary~\ref{cor:homog_burst} when flows different packet-sizes; Indeed,  when all flows send packets of the same size $l$ and $b \in \Nats$, Theorem~\ref{thm:semi_homog} provides exactly the same result as provided in Section~\ref{sec:homogen}. Algorithm~\ref{alg:thm1} can be used to compute the bound of item 1. with the following changes: First, at line one, replace the value of $m \gets \argmax_{ k=1:n-1}{ \sum_{j=1}^{k+1}l_{(j)} \leq b}$. Second, at line $4$, replace $u_k$ by $\bar{u}_k$.
 
% %  \begin{proof}
% %  The proof also follows similar steps as in the proof of Theorems~\ref{thm:homog} and \ref{thm:homog_dkw} with the following change: In Step 1) of the proof of Theorem~\ref{thm:homog} we use the fact that in the time interval $(T_i, T_j]$, $(j-i + 1)$ packets of size $l$ have arrived in the aggregate traffic, and hence $A(T_i, T_j] = (j - i + 1)l$. However, when packets are of different sizes, while  in the time interval, $(T_i, T_j]$  $(j-i + 1)$ packets have arrived, we do not know their sizes. However, we can upper bound $A(T_i, T_j]$ by assuming the worst-case packet arrivals, i.e., in the decreasing order of the sizes; specifically, we replace $H_{i,j}$ in \eqref{eq:Hij}  with $\bar{H}_{i,j} = \sum_{k=1}^{j - i +1}l_{(k)}  - \ltot(T_j - T_i)$. \qed
% %  \end{proof}

==> introduction.tex <==
\section{Introduction} \label{sec:intro}
We consider independent, periodic flows and are interested in bounding the burstiness of their aggregate traffic.  
% Periodic flows are a common and critical type of traffic in time-sensitive networks, where bounds for the worst case are required. 
Time-sensitive networks (e.g., industrial automation, automotive, avionic, etc.) require timely and accurate monitoring of the status of the network; this makes periodic flows a common and critical type of traffic in time-sensitive networks, as many devices transmit packets periodically. These packets are aggregated and forwarded to a controller. Characterizing this aggregate traffic is crucial for effective resource management and requires bounding the aggregate burstiness. A standard approach to obtain such bounds involves finding an arrival curve  constraint with rate $r$ and burst $b$ for the aggregate traffic, which means that the number of bits observed for the aggregate in any time interval of duration $t$ cannot be more than $b + rt$ bits.
 A good arrival curve must have the lowest possible rate $r$ and the smallest possible burst $b$. In our case, as  flows periodically send packets of constant size, the long-term arrival rate of the aggregate traffic $\rtot$ is known and is the lowest possible rate for the arrival curve of the aggregate; then, the problem is to find the aggregate burstiness, which is the smallest value  $b$ such that the aggregate traffic satisfies an arrival curve  with rate $\rtot$ and burst $b$. If all flows are synchronized and  have the same phase, then the aggregate burstiness is $\ltot$, which is the sum of the packet sizes of all flows. Otherwise, the aggregate burstiness would likely be smaller. We assume that phases are random and uniformly distributed, and we are then interested in finding  the probability that the aggregate burstiness exceeds some pre-specified value, i.e., \emph{bounds on the tail probability of the aggregate burstiness}.
% A standard approach to finding  delay and backlog bounds is network calculus \cite{le_boudec_network_2001,bouillard_deterministic_2018}; 
% it often characterizes a flow using an arrival curve with rate $r$ and burst $b$, which means that the number of bits observed for this flow in any time interval of duration $t$ cannot be more than $b + rt$ bits; such a constraint is necessary for the existence of finite bounds. A good arrival curve must have the lowest possible rate $r$ and the smallest possible burstiness $b$, and we want to find these values for the aggregate traffic. In our case, as  flows periodically send packets of constant size, the long-term arrival rate of the aggregate traffic $\rtot$ is known and is the lowest possible rate for the arrival curve of the aggregate; then, the problem is to find the aggregate burstiness which is the smallest value  $b$ such that the aggregate traffic satisfies an arrival curve  with rate $\rtot$ and burst $b$. If all flows are synchronized and  have the same phases, then the aggregate burstiness is $\ltot$, which is the sum of the packet sizes of all flows. Otherwise, the aggregate burstiness would likely be smaller when flows are not synchronized. In this paper, we assume that phases are random and uniformly distributed, and we are then interested in finding  the probability that the aggregate burstiness exceeds some pre-specified value; this is what we call \emph{bound on the tail probability}  of the aggregate burstiness.
% an upper bound on the tail distribution of the aggregate burstiness when phases are random and uniformly distributed, which is the probability that the aggregate burstiness exceeds some pre-specified value. 
% the aggregate burstiness will likely be smaller if  phases are random and uniformly distributed. In such cases, we want to find a bound on the tail distribution of the aggregate burstiness, which is the probability that the aggregate burstiness exceeds some pre-specified value. 
This enables us to estimate an upper bound   for the aggregate burstiness which is valid with probability of at least $1 - \varepsilon$ throughout the entire network's lifetime, where $\varepsilon$ is   a small, non-zero violation tolerance.
Deterministic network calculus \cite{bouillard_deterministic_2018,le_boudec_network_2001} can  then be applied  to obtain delay and backlog bounds that are valid with  probability of at least $1 - \varepsilon$ (\emph{quasi-deterministic} bounds). As we show in Section~\ref{sec:homogen}, such quasi-deterministic bounds are considerably less than those obtained if we do not allow any probability of violation (deterministic bounds).
% Note that $\ltot$ corresponds to the deterministic  case with zero violation probability. As we show in Section~\ref{sec:homogen}, such quasi-deterministic bounds are considerably less than the deterministic one.
% % , and grows in $n$, where $n$ is the number of flows. However, our resulting quasi-deterministic aggregate burstiness estimated for a small, non-zero n grows in $\sqrt{n\log n}$ (see Section~\ref{sec:homogen}).
% % for the former, an obvious choice is the long-term arrival rate of the flow, and for the latter, given the rate $r$
% To characterize a flow in time-sensitive networks, we are interested in the lowest possible rate $r$ and smallest possible burstiness $b$; for the former, an obvious choice is the long-term arrival rate of the flow, and for the latter, given the rate $r$, the burstiness $b$ is the smallest value such that arrival curve constraint is satisfied. As periodic flows periodically send packets of constant size, the long-term of the aggregate traffic $\rtot$ is known, and we are then interested in finding the smallest value for the burstiness $b$ such that the aggregate traffic is constrained token-bucket arrival curve with a rate $\rtot$ and a burst $b$. 
% % With network calculus, the service offered to a flow by a system is abstracted through a service curve. Combining the service and arrival curves provides a bound on the worst-case delay and backlog.
% An arrival curve is a constraint on the amount of data a flow  can send; such a constraint is necessary for a finite delay bound. A frequently used family of arrival curves are token-bucket functions as they are tractable and have simple closed forms. Having a token-bucket arrival curve with a rate $r$ and a burst $b$ means that the number of bits observed for this flow in any time interval of duration $t$ cannot be more than $b + rt$ bits. To characterize a flow in time-sensitive networks, we are interested in the lowest possible rate $r$ and smallest possible burstiness $b$; for the former, an obvious choice is the long-term arrival rate of the flow, and for the latter, given the rate $r$, the burstiness $b$ is the smallest value such that arrival curve constraint is satisfied. As periodic flows periodically send packets of constant size, the long-term of the aggregate traffic $\rtot$ is known, and we are then interested in finding the smallest value for the burstiness $b$ such that the aggregate traffic is constrained token-bucket arrival curve with a rate $\rtot$ and a burst $b$. 
% 
% We consider independent, periodic flows and are interested in bounding the burstiness of their aggregate traffic.  Periodic flows are a common and critical type of traffic in time-sensitive networks, where bounds for the worst cases are required. Network calculus \cite{le_boudec_network_2001,bouillard_deterministic_2018} is a standard approach to finding delay and backlog bounds, and it characterizes a flow by an arrival curve.
% With network calculus, the service offered to a flow by a system is abstracted through a service curve. Combining the service and arrival curves provides a bound on the worst-case delay and backlog.
% % An arrival curve is a constraint on the amount of data a flow  can send; such a constraint is necessary for a finite delay bound. A frequently used family of arrival curves are token-bucket functions as they are tractable and have simple closed forms. Having a token-bucket arrival curve with a rate $r$ and a burst $b$ means that the number of bits observed for this flow in any time interval of duration $t$ cannot be more than $b + rt$ bits. To characterize a flow in time-sensitive networks, we are interested in the lowest possible rate $r$ and smallest possible burstiness $b$; for the former, an obvious choice is the long-term arrival rate of the flow, and for the latter, given the rate $r$, the burstiness $b$ is the smallest value such that arrival curve constraint is satisfied. As periodic flows periodically send packets of constant size, the long-term of the aggregate traffic $\rtot$ is known, and we are then interested in finding the smallest value for the burstiness $b$ such that the aggregate traffic is constrained token-bucket arrival curve with a rate $\rtot$ and a burst $b$. 
% The deterministic approach finds $\ltot$ as the aggregate burstiness, which is the sum of the packet sizes of all flows. Although this bound is always valid, it is tight only when flows are perfectly synchronized; as our flows are independent, this is highly unlikely and results in an overly pessimistic bound. In contrast, we assume that the emission times of the first packet of flows (called phases in the rest of the paper) are independent, and as we assume no other information on them, they are uniformly distributed.
% I
% n contrast, we assume that the emission times of the first packet of each flow (called phases in the paper) are independent, and we have no other information on them, which corresponds to the maximum entropy, thus, we assume uniform distribution. 
% We are interested in bounds on the worst-case delays, as it is required for time-sensitive networks.  Network calculus \cite{le_boudec_network_2001,bouillard_deterministic_2018} is a standard approach to finding delay and backlog bounds. With network calculus, the service offered to a flow by a system is abstracted through a service curve. Combining the service and arrival curves provides a bound on the worst-case delay and backlog. An arrival curve is a constraint on the amount of data a flow  can send; such a constraint is necessary for a finite delay bound. A frequently used family of arrival curves are token-bucket functions as they are tractable and have simple closed forms. Having a token-bucket arrival curve $\gamma_{r,b}$ with a rate $r$ and a burst $b$ means that the number of bits observed for this flow in any time interval of duration $t$ cannot be more than $b + rt$ bits. To characterize a flow in time-sensitive networks, we are interested in the smallest possible rate $r$ and smallest possible burstiness $b$; for the former, an obvious choice is the long-term arrival rate of the flow, and for the latter, given the rate $r$, the burstiness $b$ is the smallest value such that the flow is constrained by a token-bucket arrival curve $\gamma_{r,b}$. 
% Periodic flows are a common and critical type of traffic in time-sensitive networks, representing real-time and mission-critical applications such as industrial control systems. A periodic flow periodically sends packets of constant size; we consider some periodic and independent flows where the emission time of their first packet is uniformly distributed. We are then interested in finding a token-bucket arrival curve for the aggregate. As explained above, we take as the rate $\rtot$, the long-term rate of their aggregate, and the problem is to find the smallest value for the burstiness $b$ such that their aggregate traffic is constrained by $\gamma_{\rtot,b}$.  The deterministic approach finds $\ltot$ as the aggregate burstiness, which is the sum of the packet sizes of all flows. Although this bound is always valid throughout the network's lifetime, it  is tight only when flows are perfectly synchronized, which is highly unlikely in practice and results in an overly pessimistic bound. 
% We are then interested in token-bucket arrival curves with rate $\rtot$ and burst $b$ for the aggregate traffic such that $b$ is smaller than $\ltot$ (i.e., the deterministic burstiness) and is a valid bound on the aggregate burstiness with some probability; specifically, we want to bound the probability that the aggregate burstiness exceeds $b$ with a small probability $\varepsilon$. This enables us to apply the deterministic network calculus and obtains delay and backlog bounds, considerably less than the deterministic ones, but with violation probability of at most $1 - \varepsilon$ throughout the network's lifetime, i.e., \emph{quasi-deterministic} bounds. 

Existing  works \cite{milan_etal_backlog,chang_etal,guide_snc,sbb,stochastic_leaky_bucket_regulated_flows} do not provide quasi-deterministic bounds, rather they find the probability of delay or backlog violation at an arbitrary point in time, in stationary regime; however, in time-sensitive networks, we are interested in the probability that a delay or backlog bound is not violated during some interval (e.g., the network's lifetime), not just one arbitrary point in time. The violation probability of a delay bound being small at one arbitrary point in time, does not imply that the probability that the delay bound is never violated during a period of interest is small. In fact, there would likely be some violations. \cite[Section 4.4]{sbb} points out that quasi-deterministic bounds are always trivial when arrival processes are stationary and ergodic.  However, it has been overlooked that there is interest in some non-ergodic arrival processes, as in our case. Indeed, with our model, phases are drawn randomly but remain the same during the entire period of interest; thus, our arrival processes are not ergodic. As of today, we present the only known method that obtains quasi-deterministic bounds for independent, periodic flows.
% ; furthermore, our method applies to flows with different periods and packet sizes, i.e., heterogeneous flows.

% For the homogeneous case (i.e.,  flows with the same packet size and period), we provide a closed-form expression that bounds the tail probability of the aggregate burstiness (Theorem~\ref{thm:homog_dkw}). We obtain this bound using the Dvoretzky–Kiefer–Wolfowitz (DKW) inequality \cite{massart1990tight}. When the number of flows is large, this bound is fairly tight compared to simulations (see Fig.~\ref{fig:num}(a)). Also, it results in a closed-form expression for the quasi-deterministic burstiness estimated for a non-zero violation probability (Corollary~\ref{cor:homog_burst}); it  grows in $\sqrt{n\log{n}}$, unlike the deterministic one that grows in  $n$, where $n$ is the number of flows (see Fig.~\ref{fig:num}(b)). We also provide Theorem~\ref{thm:homog}, a refinement of Theorem~\ref{thm:homog_dkw}  that provides a slightly better bound when the number of flows is small, but at the expense of not having a closed-form expression.

% For the homogeneous case (i.e.,  flows with the same packet size and period), we provide a closed-form expression that bounds the tail probability of the aggregate burstiness (Theorem~\ref{thm:homog_dkw}). We obtain this bound using the Dvoretzky–Kiefer–Wolfowitz (DKW) inequality \cite{massart1990tight}. When the number of flows is large, this bound is fairly tight compared to simulations (see Fig.~\ref{fig:num}(a)). Also, it results in a closed-form expression for the quasi-deterministic burstiness estimated for a non-zero violation probability (Corollary~\ref{cor:homog_burst}); it  grows in $\sqrt{n\log{n}}$, unlike the deterministic one that grows in  $n$, where $n$ is the number of flows (see Fig.~\ref{fig:num}(b)). We also provide Theorem~\ref{thm:homog}, a refinement of Theorem~\ref{thm:homog_dkw}  that provides a slightly better bound when the number of flows is small, but at the expense of not having a closed-form expression.

For the homogeneous case (i.e.,  flows with the same packet size and period), we provide a closed-form expression that bounds the tail probability of the aggregate burstiness (Theorem~\ref{thm:homog_dkw}). We obtain this bound using the Dvoretzky–Kiefer–Wolfowitz (DKW) inequality \cite{massart1990tight}. When the number of flows is large, this bound is fairly tight compared to simulations. Also, it results in a closed-form expression for the quasi-deterministic burstiness estimated for a non-zero violation probability (Corollary~\ref{cor:homog_burst}); it  grows in $\sqrt{n\log{n}}$, unlike the deterministic one that grows in  $n$, where $n$ is the number of flows. We also provide Theorem~\ref{thm:homog}, a refinement of Theorem~\ref{thm:homog_dkw}  that provides a slightly better bound when the number of flows is small, but at the expense of not having a closed-form expression.

% As an alternative approach, we use order statistic and obtain in Theorem~\ref{thm:homog},  bounds less than or equal to that of Theorem~\ref{thm:homog_dkw}; however, the bound of Theorem~\ref{thm:homog} is only of interest when the number of flows is small, as Theorem~\ref{thm:homog_dkw} is easier to compute and is as tight when the number of flows is large.

% Because unlike Theorem~\ref{thm:homog_dkw}, it does not have a closed-form expression, and it comes at a high computation complexity for a large $n$; moreover, Theorem~\ref{thm:homog_dkw} becomes as tight as Theorem~\ref{thm:homog} when the number of flows grows.

% as Theorem~\ref{thm:homog_dkw} is easier to compute and is as tight when the number of flows is large.

% Because unlike Theorem~\ref{thm:homog_dkw}, it does not have a closed-form expression, and it comes at a high computation complexity for a large $n$; moreover, Theorem~\ref{thm:homog_dkw} becomes as tight as Theorem~\ref{thm:homog} when the number of flows grows.

% and is only feasible in such cases
% For the homogeneous case, when all flows have the same packet size and period, we provide a closed-form expression that bounds the tail probability of the aggregate burstiness (Theorem~\ref{thm:homog_dkw}). We obtain this bound using the Dvoretzky–Kiefer–Wolfowitz (DKW) inequality \cite{massart1990tight}, and when the number of flows is large, it is fairly tight compared to simulations (see Fig. ??). Also, it results in a closed-form expression for the quasi-deterministic burstiness estimated for a non-zero violation probability (Corollary~\ref{cor:homog_burst}); it  grows in $\sqrt{n\log{n}}$, unlike the deterministic one that grows in  $n$, where $n$ is the number of flows (see also Fig. ??). As an alternative approach for when the number of flows is small, we use order statistic and obtain in Theorem~\ref{thm:homog},  bounds less than or equal to that of Theorem~\ref{thm:homog_dkw}. 

% However, the bound of Theorem~\ref{thm:homog} is only of interest when the number of flows is small. This is because, unlike Theorem~\ref{thm:homog_dkw}, it does not have a closed-form expression and it comes at a high computation complexity and is only feasible in such cases

% This is because it comes at a high computation complexity and is only feasible in such cases, and moreover, Theorem~\ref{thm:homog_dkw} is as tight when the number of flows is large.

% does not have a closed form and comes at a high 

% ; when the number of flows is small.  When 

For the heterogeneous case (i.e., flows  with different packet sizes and periods), we obtain a bound by grouping flows into  homogeneous sets and combining the bounds obtained for each set, using a convolution bounding technique based on Abel's summation (Theorem~\ref{thm:hetero}). The obtained convolution bound can be efficiently computed using discrete convolution.
% This convolution bound  is tight, specifically, it is the best possible bound on the tail probability of the aggregate burstiness given the obtained bounds for each group. Also, it has a closed-form formulation that can be efficiently computed using  properties of discrete convolution, namely,  associativity and commutativity \cite{Oppenheim2010}.
% Moreover, this convolution bound has a closed-form formulation  and is tight; specifically, it is the best possible bound on the tail probability of the aggregate burstiness given the obtained bounds for each group.
For a specific case, when flows have the same period and different packet sizes, we provide an alternative bound that may be better, when the number of flows per packet size is small (Theorem~\ref{thm:semi_homog}).  

% we can find for the aggregate of all flows, given the obtained bound for each group.
% The convolution bounding technique is tWe use Abel's summation to obtain this convolution bound, and it is tight, i.e., it is the best possible bound we can find for the aggregate of all flows, given the obtained bound for each group.


% It comes at the cost of computation complexity and can be computed as in Algorithm~\ref{alg:thm1}, hence is of interest 


% we use order statistics and union bound to bound the probability that the aggregate burstiness exceeds some value $b$ (Theorem~\ref{thm:homog}). This enables us to compute a quasi-deterministic burstiness with a small, non-zero violation probability. Although the bound of Theorem~\ref{thm:homog} does not have a closed form, we provide a concrete algorithm to compute it iteratively (Algorithm~\ref{alg:thm1}), where all computations can be done using infinite precision arithmetic (with rational numbers), e.g., using symbolic numbers in MATLAB. However, such computations can be costly regarding run-time and memory when the number of flows is large. To mitigate this, we provide  a closed-form expression, using the Dvoretzky–Kiefer–Wolfowitz (DKW) inequality \cite{massart1990tight}, that upper bounds the bound of Theorem~\ref{thm:homog}, and is tight when the number of flows $n$ is large (Theorem~\ref{thm:homog_dkw}). Furthermore, we obtain a closed-form expression to compute a quasi-deterministic aggregate burstiness, given a non-zero violation probability (Corollary~\ref{cor:homog_burst}).   We show numerically that our bounds are fairly tight compared to simulations (see Fig. ??). Moreover, the resulting aggregate burstiness estimated for a non-zero violation probability is considerably smaller than the deterministic one; it grows in $\sqrt{n\log{n}}$, unlike the deterministic one that grows in  $n$, where $n$ is the number of flows (see Fig. ??). We extend all the results we obtained for the homogeneous flows to flows  with the same period but different packet sizes (Theorem~\ref{thm:semi_homog}). This is interesting when the number of flows per packet size is small. Otherwise, our following result might provide better bounds.

% When flows  have different packet sizes and periods (i.e., heterogeneous flows), we group flows and combine the bounds obtained for each group using convolution bound: Flows with the same period and/or same packet sizes are grouped together, where for each group, we can bound the probability that their aggregate burstiness exceeds some value  using the results we presented so far. Then, in Theorem~\ref{thm:hetero}, we use convolution bound to combine them and obtain bound on the probability that the aggregate burstiness of all flows exceeds some value. We use Abel's summation to obtain this convolution bound, and it is tight, i.e., it is the best possible bound we can find for the aggregate of all flows, given the obtained bound for each group.
% % if the only information we know is the independence of each group and the provided bounding function for them. 
% We numerically observe that the bounds obtained  when combining the bounds obtained for each group using our convolution bound rather than union bound are much better (see Fig. ??). 

We numerically show that our bounds are close to simulations. The quasi-deterministic aggregate burstiness we obtain with a small, non-zero violation tolerance is considerably smaller than the deterministic one. For the heterogeneous case, we show that our convolution bounding technique provides bounds significantly  smaller than those obtained by the union bound. 

% ; it grows in $\sqrt{n\log{n}}$, unlike the deterministic one that grows in  $n$, where $n$ is the number of flows.


% compare it to the bound obtained when combining the bounds obtained for each group using union bound, 

% Also, we numerically confirm that combining the bounds obtained for each group using convolution bound compared to union bound is significantly better.

% We show numerically that our bounds are fairly tight compared to simulations (see Fig. ??). Moreover, the resulting aggregate burstiness estimated for a non-zero violation probability is considerably smaller than the deterministic one; it grows in $\sqrt{n\log{n}}$, unlike the deterministic one that grows in  $n$, where $n$ is the number of flows (see Fig. ??).
% Today, we present the only known method that obtains quasi-deterministic bounds for independent, periodic flows with different periods and packet sizes.



% the viiteratively olation probability of a delay (resp. backlog) bound being small at one arbitrary point in time, does not imply that the probability that the delay bound (resp. backlog) is never violated during the network's lifetime is small. Rather, there would likely be some violations. \cite[Section 4.4]{sbb} points out that quasi-deterministic bounds are always trivial when arrival processes are stationary and ergodic. This is perhaps why the literature was discouraged to study such characterization. Consequently, it has been overlooked that there is interest in arrival processes that are not ergodic such as our case: The first emission times of flows are drawn randomly but remain the same for the rest of the time; thus, our arrival processes are not ergodic. Indeed, in this paper, we find quasi-deterministic arrival curves. 

% Existing  works \cite{milan_etal_backlog,chang_etal,guide_snc,sbb,stochastic_leaky_bucket_regulated_flows} do not provide quasi-deterministic bounds, rather they bound the probability that the delay (resp. backlog)  is violated at an arbitrary point in time; the violation probability of a delay (resp. backlog) bound being small at one arbitrary point in time, does not imply that the probability that the delay bound (resp. backlog) is never violated during the network's lifetime is small. Rather, there would likely be some violations. \cite[Section 4.4]{sbb} points out that quasi-deterministic bounds are always trivial when arrival processes are stationary and ergodic. This is perhaps why the literature was discouraged to study such characterization. Consequently, it has been overlooked that there is interest in arrival processes that are not ergodic such as our case: The first emission times of flows are drawn randomly but remain the same for the rest of the time; thus, our arrival processes are not ergodic. Indeed, in this paper, we find quasi-deterministic arrival curves.

% the probability of delay or backlog violation at an arbitrary point in time, in stationary regime. However, in time-sensitive networks, we are interested in the probability that a delay or backlog bound is not violated during some interval (e.g., the network's lifetime), not just one arbitrary point in time. Bounds obtained by $\sbbTwo$ do not provide such information; the violation probability of a delay bound being small at one arbitrary point in time, does not imply that the probability that the delay bound is never violated during a period of interest is small. In fact, there would likely be some violations. In contrast, when using $\sbbThree$, we can guarantee, with some probability, that delay and backlog bounds derived by deterministic network calculus are never violated  during the network's lifetime. Indeed, in this paper,  we are interested in $\sbbThree$ rather than $\sbbTwo$, as is visible in formulation \eqref{eq:prob}.






% Periodic flows are commonly used in various applications, including industrial automation, process control, and transportation systems. They are characterized by their predictable arrival times and fixed packet sizes which make them an ideal candidate for time-sensitive applications. We consider several periodic and asynchronous flows aggregated and fed to a FIFO network element, and we are interested in finding an arrival curve for the aggregate traffic, which by network calculus, can be used to obtain a delay bound. The deterministic burstiness bound for the aggregate traffic equals the sum of individual burstiness. Although this gives a valid bound and is never to be violated, it assumes perfectly synchronized flows, which is highly unlikely in practice and results in overly pessimistic bounds. Existing non-deterministic approaches bound
% the probability of buffer overflow in a network node (element), offering a service curve, fed with independent arrival processes (inputs flows) that are each constrained by arrival curves, are obtained under various assumptions.

% We focus solely on periodic flows.









==> proofs.tex <==
\section{Proofs} \label{sec:proofs}

% \subsection{Proof of Theorem~\ref{thm:homog}}
%  $\Bar{B} = sup_{t \geq 0}B(t)$, where $B(t)$ is the aggregate burstiness at time $t$. First, flows are packetized, and thus $sup_{t \geq 0}B(t)$ can be reduced to only values of $B(t)$ at arrival times of packets: Let us denote by  $T_i$ and $T_i$ be the arrival time of the $i$-th packet in the aggregate traffic; thus, $sup_{t \geq 0}B(t) = sup_{i \geq 1}B(T_i)$. Second, as flows are periodic, we have $T_{i+F} = T_i + \tau$, and thus $sup_{i \geq 1}B(T_i) = \sup_{i=1:2F}B(T_i)$.


==> related_works.tex <==
\section{Background and Related Works} \label{sec:realted_works}
% The aggregate function has a deterministic, token-bucket arrival curve $\gamma_{\rtot,\ltot}$ with $\rtot = \sum_fr_f$ and $\ltot = \sum_fl_f$. $\ltot $ is a deterministic bound that holds for any possible arrival process.
% \hossein{
% \begin{enumerate}
%     \item Different envelopes: SBB,S2BB, and S3BB, and how our definition fits.
%     \item Previous result that we want to compare: Milan et al and Amr Rizk et al.
%     \item How do we differ from previous results.
% \end{enumerate}}
% Bounds the probability of buffer overflow in a network node (element), offering a service curve, fed with independent arrival processes (inputs flows) that are each constrained by arrival curves, are obtained under various assumptions.

% Network calculus \cite{le_boudec_network_2001, Changbook,bouillard_deterministic_2018} is a  standard approach to compute delay (resp. backlog) bounds for the worst case. Specifically, with network calculus, the service offered to a flow of interest by a system is abstracted by means of a service curve. A bound on the worst-case delay (resp. backlog) is obtained by combining the service curve with an arrival curve for the flow of interest. An arrival curve is a constraint on the amount of data that the flow of interest can send; such a constraint is necessary for the existence of a finite delay bound. The exact definitions can be found in \cite[Sec. 1.2, 1.3, and 1.4]{le_boudec_network_2001}. In this paper, we focus on the arrival curves, specifically token-bucket functions that are frequently used. 

% We say a flow is constrained by a token-bucket arrival curve with rate $r$ and burst $b$ if the number of bits observed for this flow for any $s \leq t$ is upper bounded by $r(t-s) + b$, i.e., $\forall s \leq t,~ A(s,t] \leq r(t - s) + b$ where recall that $A(s,t]$ denote the number of bits observed in time interval $(s,t]$. This definition is a deterministic constraint on the flow. 

% We say a flow is constrained by a token-bucket arrival curve $\gamma_{r,b}$ (see Section~\ref{sec:assump_prob}) if the number of bits observed for this flow for any $s \leq t$ is upper bounded by $r(t-s) + b$, i.e., $\forall s \leq t,~ A(s,t] \leq r(t - s) + b$ where recall that $A(s,t]$ denote the number of bits observed in time interval $(s,t]$. This definition is a deterministic constraint on the flow. 

The definition of a deterministic constraint on the flow is defined in Section~\ref{sec:assump_prob} and always hold. Alternatively, one can define an arrival constraint that holds with some probability. Depending on how quantifiers are used, this leads to three possible definitions, called \emph{stochastically bounded burstiness}, \cite{sbb, snc_basics}, which we express here for token-bucket constraints: 
\begin{align}
    \label{eq:sbbOne}
    &\sbbOne: \forall 0 \leq s \leq t,~ \P\lp A(t,s] - r(t-s) > b\rp \leq \epsilon(b) \\
    \label{eq:sbbTwo}
    &\sbbTwo: \forall t \geq 0,~ \P ( \underbrace{\sup_{0 \leq s \leq t}\{A(t,s] - r(t-s)\}}_{\bar{B}(t)}  > b) \leq \epsilon(b) \\
    \label{eq:sbbThree}
    &\sbbThree: \P( \underbrace{\sup_{t\geq 0}\bar{B}(t)}_{B}  > b ) \leq \epsilon(b) 
    % &\sbbThree: \P( \sup_{t\geq 0}\bar{B}(t) = B  > b ) = \P( \exists t\geq 0, ~ B(t)  > b ) \leq \epsilon(b) 
\end{align}

The first definition, $\sbbOne$, requires that, for a fixed pair of measurement instant $s \leq t$, the deterministic arrival curve constraint with rate $r$ and burst $b$ is satisfied with probability at least $1 - \epsilon(b)$, and this should hold for any $s \leq t$. The second definition, $\sbbTwo$, requires that for a fixed time $t$, with probability at least $1 - \epsilon(b)$, the deterministic arrival curve with rate $r$ and burst $b$ is satisfied for the entire interval $[0, t]$, and this should hold for any $t \geq 0$.
% upper bounds the probability that at a time $t$, the burstiness $B(t)$ exceeds $b$ (see \eqref{eq:agg_burst} for the definition of $B(t)$). 
Lastly, $\sbbThree$, requires that, with probability at least $1 - \epsilon(b)$, the deterministic arrival curve with rate $r$ and burst $b$ is always satisfied.

% upper bounds  the probability that there exists a time $t$ such that the burstiness $B(t)$ exceeds $b$.

Observe that $\sbbThree$ implies $\sbbTwo$  and $\sbbTwo$  implies $\sbbOne$, hence $\sbbThree$ is the strongest. Also,  a deterministic arrival curve is a special case of $\sbbThree$ where $\epsilon(b) = 0$. This is why, for a non-zero violation probability $\epsilon(b)$, $b$ is called a \emph{quasi-deterministic} bound on the burstiness. 

$\sbbOne$ was used in \cite{sbb_one} to derive backlog bounds in a single node, but such bounds are loose, which can be attributed to the fact the definition of $\sbbOne$ is not strong enough. Other works \cite{milan_etal_backlog,chang_etal,guide_snc,sbb,stochastic_leaky_bucket_regulated_flows,kesidis_buffer} have used the stronger $\sbbTwo$ definition and obtained bounds on the probability of delay or backlog violation at an arbitrary point in time, in stationary regime. However, in time-sensitive networks, we are interested in the probability that a delay or backlog bound is not violated during some interval (e.g., the network's lifetime), not just one arbitrary point in time. Bounds obtained by $\sbbTwo$ do not provide such information; the violation probability of a delay bound being small at one arbitrary point in time, does not imply that the probability that the delay bound is never violated during a period of interest is small. In fact, there would likely be some violations. In contrast, when using $\sbbThree$, we can guarantee, with some probability, that delay and backlog bounds derived by deterministic network calculus are never violated  during the network's lifetime. Indeed, in this paper,  we are interested in $\sbbThree$ rather than $\sbbTwo$, as is visible in formulation \eqref{eq:prob}.





% As explained in Section~\ref{sec:assump_prob},  we are interested in token-bucket arrival curves of type $\sbbThree$ rather than $\sbbTwo$: In time-sensitive networks, we are interested in the probability that a delay or backlog bound is not violated during some interval (e.g., the network's lifetime), not just one arbitrary point in time. however, bounds obtained by $\sbbTwo$ do not provide such information; the violation probability of a delay bound being small at one arbitrary point in time, does not imply that the probability that the delay bound is never violated during a period of interest is small. In fact, there would likely be some violations. In contrast, we can guarantee that delay bounds derived by deterministic network calculus, when using $\sbbThree$, would never be violated with some probability during the network's lifetime.

As of today, previous works \cite{milan_etal_backlog,chang_etal,guide_snc,sbb,stochastic_leaky_bucket_regulated_flows,kesidis_buffer} are of type $\sbbTwo$: \cite[Section 4.4]{sbb} points out the fact that when arrival processes are stationary and ergodic, $\sbbThree$ is always trivial and the bounding function $\epsilon(b)$ in \eqref{eq:sbbThree} is either zero or one. This is perhaps why the literature was discouraged to study $\sbbThree$ characterizations. However, it has been overlooked that there is interest in some non-ergodic arrival processes, as in our case. Indeed, with our model, phases $\phi_f$ are drawn randomly but remain the same during the entire period of interest; thus, our arrival processes are not ergodic.

% Indeed, in this paper, we find arrival curves of type $\sbbThree$.

% the bounding function $\epsilon(b)$ of $\sbbThree$ is either zero or one; this means that there is no non-trivial  

% The fact that at one point in time, the violation probability of a delay bound is small does not imply that the probability that the delay bound is never violated during a period of interest is small; in fact that there would likely be some violations.


% and as of today, previous works are of type $\sbbTwo$: In time-sensitive networks, we are interested in the probability that a delay or backlog bound is not violated during some interval, not just one arbitrary point in time; however, bounds obtained by $\sbbTwo$ do not provide such information. The fact that at one point in time, the violation probability of a delay bound is small does not imply that the probability that the delay bound is never violated during a period of interest is small; in fact that there would likely be some violations. In contrast, 

% In time-sensitive networks, we are interested in the probability that a delay or backlog bound is not violated during some interval, not just one arbitrary point in time; however, bounds obtained by $\sbbTwo$ do not provide such information. The fact that at one point in time, the violation probability of a delay bound is small does not imply that the probability that the delay bound is never violated during a period of interest is small; in fact that there would likely be some violations. In contrast, 



% First, observe that $\sbbThree$ implies $\sbbTwo$  and $\sbbTwo$  implies $\sbbOne$, hence $\sbbThree$ is the strongest. Second, a token-bucket function $\gamma_{r,b}$ of type $\sbbThree$ is a valid arrival curve with the probability of $1 - \epsilon(b)$; indeed, a deterministic arrival curve $\gamma_{r,b}$ is of type $\sbbThree$ where $\epsilon(b) = 0$. This is why, for a non-zero violation probability $\epsilon(b)$, we call $b$ a \emph{quasi-deterministic} bound on the burstiness. Third, it follows that bounds derived by deterministic network calculus when using  $\gamma_{r,b}$ are valid with the probability of $1 - \epsilon(b)$.

% As explained in Section~\ref{sec:assump_prob},  we are interested in token-bucket arrival curves of type $\sbbThree$, and as of today, previous works are of type $\sbbTwo$: In time-sensitive networks, we are interested in the probability that a delay or backlog bound is not violated during some interval, not just one arbitrary point in time; however, bounds obtained by $\sbbTwo$ do not provide such information. The fact that at one point in time, the violation probability of a delay bound is small does not imply that the probability that the delay bound is never violated during a period of interest is small; in fact that there would likely be some violations. In contrast, 



% The second definition, $\sbbTwo$, is stronger (i.e., it implies $\sbbOne$) as it upper bounds the probability that at a time $t$, the burstiness $B(t)$, given in \eqref{eq:agg_burst}, exceeds $b$. Lastly, $\sbbThree$, the strongest (i.e., it implies $\sbbTwo$ hence $\sbbOne$), upper bounds  the probability that there exists a time $t$ such that the burstiness $B(t)$ exceeds $b$; thus, $\gamma_{r,b}$ is a valid arrival curve with the probability of $1 - \epsilon(b)$. We call $b$ a \emph{quasi-deterministic} bound on the burstiness. Note that a deterministic arrival curve $\gamma_{r,b}$ is of type $\sbbThree$ where $\epsilon(b) = 0$. Given $\gamma_{r,b}$ of type $\sbbThree$, bounds derived by deterministic network calculus are valid with the probability of $1 - \epsilon(b)$. This is why we are interested in token-bucket arrival curves of type $\sbbThree$ rather than $\sbbTwo$, and as of today, no previous work applies to our problem.

% The first definition of \emph{stochastic burstiness bound} ($\sbbOne$) upper bounds the probability that for an interval $(s,t]$, more than $\gamma_{r,b}(t-s)$ bits is observed for the flow. The second definition, $\sbbTwo$, is stronger (i.e., it implies $\sbbOne$) as it upper bounds the probability that at a time $t$, the burstiness $B(t)$, given in \eqref{eq:agg_burst}, exceeds $b$. Lastly, $\sbbThree$, the strongest (i.e., it implies $\sbbTwo$ hence $\sbbOne$), upper bounds  the probability that there exists a time $t$ such that the burstiness $B(t)$ exceeds $b$; thus, $\gamma_{r,b}$ is a valid arrival curve with the probability of $1 - \epsilon(b)$. We call $b$ a \emph{quasi-deterministic} bound on the burstiness. Note that a deterministic arrival curve $\gamma_{r,b}$ is of type $\sbbThree$ where $\epsilon(b) = 0$. Given $\gamma_{r,b}$ of type $\sbbThree$, bounds derived by deterministic network calculus are valid with the probability of $1 - \epsilon(b)$. This is why we are interested in token-bucket arrival curves of type $\sbbThree$ rather than $\sbbTwo$, and as of today, no previous work applies to our problem.


% Let us compare $\sbbTwo$ and $\sbbThree$ in our case, i.e., periodic traffic: The aggregate traffic is also periodic, with the period being the hyper-period of individual flows. $\sbbTwo$ provides a bound on the probability that the burstiness $b$  

% Note that a deterministic arrival curve $\gamma_{r,b}$ is of type $\sbbThree$ where $\epsilon(b) = 0$. Given $\gamma_{r,b}$ of type $\sbbThree$, bounds derived by deterministic network calculus are valid with the probability of $1 - \epsilon(b)$, and this is why we are interested in $\sbbThree$. Observe that $\sbbTwo$ is valid only for a one time instance; thus, when the observation window increases, it becomes weaker.

% As explained in Section~\ref{sec:assump_prob},  we are interested in token-bucket arrival curves of type $\sbbThree$, and as of today, no previous work applies to our problem. Previous works are of type $\sbbTwo$, and they compute backlog or delay bounds by assuming that aggregate traffic is fed by a network element with a known service curve \cite{milan_etal_backlog,chang_etal,guide_snc,sbb,stochastic_leaky_bucket_regulated_flows}. Specifically, assume a constant-rate server with the rate $c > \rtot$, and let $q(t)$ denote the queue length at time $t$. Then, they find $\epsilon(Q)$ such that $\forall t \geq 0,~ \P ( q(t) > Q) \leq \epsilon(Q) $, i.e., they bound the probability that the queue length (i.e., backlog) at time $t$ exceeds $Q$. Hence, their results depend on the rate of the server and are of type $\sbbTwo$. We have stronger assumptions on the flows, which enables us to obtain a strong bound on the aggregate burstiness. In Section~\ref{sec:num}, we compare an application of our bound to \cite{milan_etal_backlog, guide_snc} as other works are either presented for discrete times or dominated by \cite{milan_etal_backlog}.

% Note that  they have weaker assumptions on the flows, their results depend on the rate of the server, and are of type $\sbbTwo$. In Section~\ref{sec:num}, we compare an application of our bound to \cite{milan_etal_backlog, guide_snc} as other works are either presented for discrete times or dominated by \cite{milan_etal_backlog}. 











==> semi_homogeneous.tex <==
\section{Semi-Homogeneous Flows: Same Period and Different Packet-size} \label{sec:semi-homogen}
